Improved Approximation for Node-Disjoint Paths in Grids with Sources on the Boundary

We study the classical Node-Disjoint Paths (NDP) problem: given an undirected $n$-vertex graph G, together with a set {(s_1,t_1),...,(s_k,t_k)} of pairs of its vertices, called source-destination, or demand pairs, find a maximum-cardinality set of mutually node-disjoint paths that connect the demand pairs. The best current approximation for the problem is achieved by a simple greedy $O(\sqrt{n})$-approximation algorithm. A special case of the problem called NDP-Grid, where the underlying graph is a grid, has been studied extensively. The best current approximation algorithm for NDP-Grid achieves an $\tilde{O}(n^{1/4})$-approximation factor. On the negative side, a recent result by the authors shows that NDP is hard to approximate to within factor $2^{\Omega(\sqrt{\log n})}$, even if the underlying graph is a sub-graph of a grid, and all source vertices lie on the grid boundary. In a follow-up work, the authors further show that NDP-Grid is hard to approximate to within factor $\Omega(2^{\log^{1-\epsilon}n})$ for any constant $\epsilon$ under standard complexity assumptions, and to within factor $n^{\Omega(1/(\log\log n)^2)}$ under randomized ETH. In this paper we study NDP-Grid, where all source vertices {s_1,...,s_k} appear on the grid boundary. Our main result is an efficient randomized $2^{O(\sqrt{\log n} \cdot \log\log n)}$-approximation algorithm for this problem. We generalize this result to instances where the source vertices lie within a prescribed distance from the grid boundary. Much of the work on approximation algorithms for NDP relies on the multicommodity flow relaxation of the problem, which is known to have an $\Omega(\sqrt n)$ integrality gap, even in grid graphs. Our work departs from this paradigm, and uses a (completely different) linear program only to select the pairs to be routed, while the routing itself is computed by other methods.

==> arxiv final/coloring-squares.tex <==

%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
\label{-----------------------------sec: coloring the squares-------------------------------}
\section{Finding the Coloring of Squares and a Perfect Set of Demand Pairs}\label{sec: coloring the squares}
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
The goal of this section is to prove Theorem~\ref{thm: finding the coloring}. It would be convenient for us to reformulate the problem slightly differently. Recall that we are given a hierarchical system $\cset$ of colors, and that for all source vertices $s$ of the demand pairs in $\tmset$, their colorings are fixed: that is, each vertex $s\in S(\tmset)$ is assigned, for each level $1\leq h\leq \rho$, some level-$h$ color $c_h$. Consider now some demand pair $(s,t)\in \tmset$. For each level $1\leq h\leq \rho$, if $s$ is assigned the level-$h$ color $c_h$, then we will assign the same  level-$h$ color $c_h$ to $t$. Note that the same vertex of $G$ may serve as a destination of several demand pairs; in such a case, we view this vertex as having different copies, each of which is colored according to the coloring of the corresponding source vertex.

For now, we will ignore the set $S(\tmset)$ of the source vertices of the demand pairs in $\tmset$, and we will focus on the multi-set $U$ of the destination vertices in $T(\tmset)$. Suppose we compute some coloring $f$ of $\thset$ by $\cset$. Consider some level-$\rho$ square $Q$, and some destination vertex $t\in U\cap Q$. Suppose square $Q$ is assigned the level-$\rho$ color $c_{\rho}$. We say that $t$ \emph{agrees} with the coloring of $Q$ iff $t$ was also assigned the level-$\rho$ color $c_{\rho}$. We can now restate the problem slightly differently. We call the new problem Hierarchical Square Coloring (\HSC). 
In this problem, we are given a hierarchical system $\thset=(\qset_1,\ldots,\qset_{\rho})$ of squares, a hierarchical system $\cset$ of colors, and a multi-set $U$ of vertices that lie in $\bigcup_{Q\in \qset_{\rho}}Q$, together with an assignment of a level-$\rho$ color to each vertex in $U$. Notice that this assignment implicitly assigns, to each vertex $v\in U$, for each level $1\leq h<\rho$, a unique level-$h$ color $c_h$, which is the level-$h$ ancestor of the level-$\rho$ color assigned to $v$.
Our goal is to find a coloring $f$ of $\thset$ by $\cset$, and a subset $U'\subseteq U$ of the vertices, such that:

\begin{itemize}
\item For each vertex $t\in U'$, if $t$ belongs to a level-$\rho$ square $Q$, then the coloring of $t$ agrees with the coloring of $Q$; and
\item For each level $1\leq h\leq \rho$, for each level-$h$ color $c_h$, the total number of vertices in $U'$ whose level-$h$ color is $c_h$ is at most $d_h$.
\end{itemize}

The goal is to maximize $|U'|$.  The main result of this section is a proof of the following theorem.

\begin{theorem}\label{thm: main finding the coloring}
There is an efficient randomized algorithm, that, given as input an instance $(\thset,\hmset)$ of the \HSC problem, with high probability returns an $O(\log^4 n)$-approximate solution to it.
\end{theorem}


We first show that Theorem~\ref{thm: finding the coloring} follows from Theorem~\ref{thm: main finding the coloring}. Let $U'\subseteq U$ be the (multi)-set of the destination vertices computed by the algorithm from Theorem~\ref{thm: main finding the coloring}. As every destination vertex in $U'$ belongs to a unique demand pair in $\tmset$, set $U'$ naturally defines a subset $\tmset'\subseteq \tmset$ of demand pairs. It is immediate to verify that $|\tmset'|\geq \Omega(\opt'/\log^4 n)$. This is since the maximum-cardinality subset $\tmset''\subseteq \tmset$ of the demand pairs, for which a coloring $f'$ of $\thset$ by $\cset$ exists, with $\tmset''$ being perfect for $f'$, naturally defines a feasible solution to \HSC, of value $|\tmset''|$. The set $\tmset'$ of demand pairs has all properties of a perfect set, except that we are not guaranteed that the source and the destination vertices are all distinct. We rectify this as follows. Fix any level-$\rho$ color $c_{\rho}$. Recall that there are at most $d_{\rho}=\eta^3=2^{O(\sqrt{\log n})}$ demand pairs $(s,t)\in \tmset'$, such that the level-$\rho$ color of $s$ is $c_{\rho}$. We discard all such pairs but one from $\tmset'$. It is immediate to verify that $|\tmset'|\geq \opt'/2^{O(\sqrt{\log n})}$ still holds. We claim that all demand pairs in this final set $\tmset'$ have distinct sources and destinations. Indeed, consider any two such distinct pairs $(s,t)$, $(s',t')$. Assume first that $s=s'$. Let $c_{\rho}$ be the level-$\rho$ color of $s$. Then $\tmset'$ contains two demand pairs whose sources have the same level-$\rho$ color, a contradiction. Assume now that $s\neq s'$ but $t=t'$. Then the level-$\rho$ colors of $s$ and $s'$ must be different, and so are the level-$\rho$ colors $t$ and $t'$. However, both $t$ and $t'$ belong to the same level-$\rho$ square $Q_{\rho}$, and their color should agree with the level-$\rho$ color of $Q_{\rho}$, which is impossible.


The remainder of this section is dedicated to proving Theorem~\ref{thm: main finding the coloring}. We formulate an LP-relaxation of the problem, and then provide a randomized LP-rounding approximation algorithm for it.


For convenience, for every pair $1\leq h<h'\leq \rho$ of levels, for every level-$h$ square $Q$, we denote by $\dset_{h'}(Q)$ the set of all level-$h'$ squares that are contained in $Q$, and we think of them as level-$h'$ descendants of $Q$. Recall that for each level-$h$ color $c_h$,  we have also denoted by $\tilde \chi_{h'}(c)$ the set of all its descendant-colors that belong to level $h'$.
%--------------------------------------------------
%--------------------------------------------------
\subsection{The Linear Program}\label{subsec: the LP}
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%Consider some level $1\leq h\leq \rho$, and some level-$h$ square $Q\in \qset_h$. Recall that $Q$ is a $(\gamma_h\times \gamma_h)$-square. Therefore, in any feasible solution $V''$ for the problem, all vertices of $V''\cap V(Q)$ have the same level-$h$ color.

For every level-$\rho$ square $Q_{\rho}\in \qset_{\rho}$, and every level-$\rho$ color $c_{\rho}\in \chi_{\rho}$, we let $n(Q_{\rho},c_{\rho})$ denote the number of vertices of $U\cap V(Q_{\rho})$, whose level-$\rho$ color is $c_{\rho}$.

Our linear program has three types of variables. Fix some level $1\leq h\leq \rho$ and a level-$h$ color $c_{h}\in \chi_h$. For every level-$h$ square $Q_h\in \qset_h$, we have a variable $x(Q_h,c_h)$ indicating whether we choose color $c_h$ for square $Q_h$. We also have a global variable $Y_h(c_h)$, counting the total number of all vertices in the final solution $U'$, whose level-$h$ color is $c_h$. Finally, for every level-$\rho$ square $Q_{\rho}\in \qset_{\rho}$ and color $c_{\rho}\in \chi_{\rho}$, we have a variable $y_{\rho}(Q_{\rho},c_{\rho})$. Intuitively, if $Q_{\rho}$ is assigned the color $c_{\rho}$, then $y_{\rho}(Q_{\rho},c_{\rho})$ is the total number of vertices of $U'\cap V(Q_{\rho})$ in our solution $U'$ (note that their level-$\rho$ color must be $c_{\rho}$); otherwise, $y_{\rho}(Q_{\rho},c_{\rho})=0$. 

The objective function of the LP is:

\[\max\quad\quad\sum_{c_{\rho}\in \chi_{\rho}}Y_{\rho}(c_{\rho}).\]

We now define the constraints of the LP.
The first set of constraints requires that for each level-$\rho$ square $Q_{\rho}$, and each level-$\rho$ color $c_{\rho}$, if $Q_{\rho}$ is assigned the color $c_{\rho}$, then $y(Q_{\rho},c_{\rho})$ is bounded by $n(Q_{\rho},c_{\rho})$, and otherwise it is $0$.

\begin{equation}
y(Q_{\rho},c_{\rho})\leq n(Q_{\rho},c_{\rho})\cdot x(Q_{\rho},c_{\rho})\quad\quad \forall  c_{\rho}\in \chi_{\rho}, \forall  Q_{\rho}\in \qset_{\rho} \label{LP: bounding rho colored vertices in each square}
\end{equation}

The next set of constraints states that for each level-$\rho$ color $c_{\rho}$, the total number of vertices of $U'$ whose level-$\rho$ color is $c_{\rho}$
is equal to the summation, over all level-$\rho$ squares $Q_{\rho}$, of the number of vertices of $U'\cap V(Q)$, whose level-$\rho$ color is $c_{\rho}$.

\begin{equation}
Y_{\rho}(c_{\rho})=\sum_{Q_{\rho}\in \qset_{\rho}}y(Q_{\rho},c_{\rho}) \quad\quad \forall c_{\rho}\in \chi_{\rho}\label{LP: accounting for Yrho}
\end{equation}

The next set of constraints states that for every level $h$ and every level-$h$ color $c_h$, the total number of vertices of $U'$ whose level-$h$ color is $c_h$ is equal to the total number of vertices of $U'$ whose level-$\rho$ color is a descendant color of $c_h$. 

\begin{equation}
Y_h(c_h)=\sum_{c_{\rho}\in \tilde{\chi}_{\rho}(c_h)}Y_{\rho}(c_{\rho}) \quad\quad \forall 1\leq h< \rho, \forall c_h\in \chi_h \label{LP: Yh is sum of Yrhos}
\end{equation}

The following set of constraints ensures that for each level $h$, and each level-$h$ color $c_h$, no more than $d_h$ vertices of $U'$ whose level-$h$ color is $c_h$ are in the solution.
\begin{equation}
Y_h(c_h)\leq d_h\quad\quad \forall 1\leq h\leq \rho, \forall c_h\in \chi_h \label{LP: bound of Yh by kh}
\end{equation}

The next set of constraints ensures that every level-$1$ square is assigned some level-$1$ color.
\begin{equation}
\sum_{c_1\in \chi_1}x(Q_1,c_1)=1\quad\quad \forall Q_1\in \qset_1\label{LP: sum of colors 1 for level 1}
\end{equation}

%\begin{eqnarray}
%\max&\sum_{c_{\rho}\in \chi_{\rho}}Y_{\rho}(c_{\rho})&\nonumber\\
%\mbox{s.t.}&&\nonumber\\
%&Y_h(c_h)\leq d_h&\forall 1\leq h\leq \rho, \forall c_h\in \chi_h \label{LP: bound of Yh by kh}\\
%&Y_h(c_h)=\sum_{c_{\rho}\in \tilde{\chi}_{\rho}(c_h)}Y_{\rho}(c_{\rho})&\forall 1\leq h< \rho, \forall c_h\in \chi_h \label{LP: Yh is sum of Yrhos}\\
%&Y_{\rho}(c_{\rho})=\sum_{Q_{\rho}\in \qset_{\rho}}y(Q_{\rho},c_{\rho})&\forall c_{\rho}\in \chi_{\rho}\label{LP: accounting for Yrho}\\
%&y(Q_{\rho},c_{\rho})\leq n(Q_{\rho},c_{\rho})\cdot x(Q_{\rho},c_{\rho})&\forall  c_{\rho}\in \chi_{\rho}, \forall  Q_{\rho}\in \qset_{\rho} \label{LP: bounding rho colored vertices in each square}\\
%&\sum_{c_1\in \chi_1}x(Q_1,c_1)=1&\forall Q_1\in \qset_1\label{LP: sum of colors 1 for level 1}
%\end{eqnarray}

%The set (\ref{LP: bound of Yh by kh}) ensures that for each level $h$, and each level-$h$ color $c_h$, no more than $d_h$ vertices of $U$ whose level-$h$ color is $c_h$ are in the solution.
%The set (\ref{LP: Yh is sum of Yrhos}) states that for every level $h$ and every level-$h$ color $c_h$, the total number of vertices of $U'$ whose level-$h$ color is $c_h$ is equal to the total number of vertices of $U'$ whose level-$\rho$ color is a descendant color of $c_h$. 

%The set (\ref{LP: accounting for Yrho}) states that for each level-$\rho$ color $c_{\rho}$, the total number of vertices of $U'$ whose level-$\rho$ color is $c_{\rho}$
%is equal to the summation, over all level-$\rho$ squares $Q$, of the number of vertices of $U'\cap V(Q)$, whose level-$\rho$ color is $c_{\rho}$.

%The set (\ref{LP: bounding rho colored vertices in each square}) requires that for each level-$\rho$ square $Q$, and each level-$\rho$ color $c_{\rho}$, if $Q$ is assigned the color $c$, then at most $n(Q_{\rho,c_{\rho}})$ vertices of $U'\cap V(Q)$ have level-$\rho$ color $c_{\rho}$, and otherwise none of them does. (As we cannot guarantee that $x(Q_{\rho},c_{\rho})$ is integral, we will obtain intermediate cases, for which the constraint will be useful).

%Finally, the set (\ref{LP: sum of colors 1 for level 1}) of constraints ensures that every level-$1$ square is assigned some level-$1$ color.

It is immediate to verify that all above constraints are satisfied by any valid integral solution to \HSC, so the above LP is indeed a relaxation of \HSC.

We now add a few additional constraints to coordinate between different levels, that will be crucial for our LP-rounding algorithm. 
Consider some level $1\leq h<\rho$, and some level-$h$ square $Q_h$. Let $Q_{h+1}$ be a child-square of $Q_h$. If $Q_h$ is assigned the level-$h$ color $c_h$, then $Q_{h+1}$ must be assigned some child-color of $c_h$. The following constraint expresses this requirement.
%The following two constraints are added for every pair of levels $1\leq h<h' \leq \rho$, every level-$h$ square $Q_h\in \qset_h$, and every color $c_h\in \chi_h$. 
%The first constraint requires that for every level-$h'$ sub-square $Q_{h'}$ of $Q_h$, we assign to $Q_{h'}$ a level-$h'$ color that is a descendant of $c_h$ if and only if we have assigned color $c_h$ to square $Q_h$: \mynote{Only need for parent? stopped here}
%\begin{equation}
%\sum_{c_{h'}\in \tilde{\chi}_{h'}(c_h)}x(Q_{h'},c_{h'})=x(Q_h,c_h)\quad\quad \forall 1\leq h<h'\leq \rho; \quad \forall Q\in \qset_h; \quad \forall c_h\in \chi_h; \quad \forall Q_{h'}\in \dset_{h'}(Q_h) \label{LP: color coordination across levels}
%\end{equation}


\begin{equation}
\sum_{c_{h+1}\in \tilde{\chi}_{h+1}(c_h)}x(Q_{h+1},c_{h+1})=x(Q_h,c_h)\quad\quad \forall 1\leq h<\rho; \quad \forall Q_h\in \qset_h; \quad \forall c_h\in \chi_h; \quad \forall Q_{h+1}\in \dset_{h+1}(Q_h) \label{LP: color coordination across levels}
\end{equation}

The next constraint requires that for every pair $1\leq h\leq h'\leq \rho$ of levels, for every level-$h$ square $Q_h$ and every level-$h$ color $c_h$, if $c_{h'}$ is a level-$h'$ descendant color of $c_h$, then  the total number of vertices in $U'\cap V(Q_h)$ that are assigned  the level-$h'$  color $c_{h'}$, is at most $d_{h'}$, if square $Q_{h}$ is assigned color $c_h$, and it is $0$ otherwise (notice that we also require this for $h=h'$):

\begin{equation}
\sum_{Q_{\rho}\in \dset_{\rho}(Q_h)}\sum_{c_{\rho}\in \tilde{\chi}_{\rho}(c_{h'})}y(Q_{\rho},c_{\rho})\leq d_{h'}\cdot x(Q_h,c_h)\quad\quad \forall 1\leq h\leq h'\leq \rho; \quad \forall Q_h\in \qset_h; \quad \forall c_h\in \chi_h;  \forall c_{h'}\in \tilde{\chi}_{h'}(c_h)\label{LP: color coordination with kh across levels}
\end{equation}

(Note that indeed for an integral solution, $\sum_{Q_{\rho}\in \dset_{\rho}(Q_h)}\sum_{c_{\rho}\in \tilde{\chi}_{\rho}(\chi_{h'})}y(Q_{\rho},c_{\rho})$ is the total  number of vertices in $U'\cap V(Q_h)$ that are assigned the level-$h'$ color $c_{h'}$.)

Finally, we add non-negativity constraints:

\begin{equation}
x(Q_h,c_h)\geq 0\quad\quad \forall 1\leq h\leq \rho; \quad \forall c_h\in \chi_h \label{LP: non-neg1}
\end{equation}

\begin{equation}
y(Q_{\rho},c_{\rho})\geq 0\quad\quad \forall Q_{\rho}\in \qset_{\rho};\quad \forall c_{\rho}\in \chi_{\rho} \label{LP: non-neg2}
\end{equation}

This completes the description of the LP-relaxation. We now proceed to describe the LP-rounding algorithm.



%Finally, we require that for every level $1\leq h\leq \rho$, every level-$h$ square $Q_h$ and level-$h$ color $c_h$, $U'\cap Q_h$ contains no more than $d_h$ vertices of level-$h$ color $c_h$ if $Q_h$ is assigned color $c_h$, and $0$ otherwise. (This is the same as Constraint~(\ref{LP: color coordination with kh across levels}), with $h'=h$).

%\begin{equation}
%\sum_{Q_{\rho}\in \qset_{\rho}(Q_h)}\sum_{c_{\rho}\in\tilde{\chi}_{\rho}(\chi_h)}y(Q_{\rho},c_{\rho})\leq d_h\cdot x(Q_h,c_h) \quad\quad\forall 1\leq h\leq \rho,\forall Q_h\in \qset_h,\forall c_h\in \chi_h \label{LP: num of vertices in a square bounded by kh}
%\end{equation}



%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
\subsection{LP-Rounding}\label{subsec: LP-rounding}
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
For convenience, we denote $|U|=n$.
Our LP-rounding algorithm proceeds in three stages. In the first stage we perform a simple randomized rounding, level-by-level. We will show that the expected number of vertices that we select to our solution $U'$ is equal to the LP-solution value. However, it is possible that we select too many vertices of some color. In the second stage, we define, for every level $h$, and every level-$h$ color $c_h$, a bad event that too many vertices of color $c_h$ are added to $U'$, and show that with high probability none of these bad events happen. If any of the bad events happen, we discard all vertices and return an empty solution. Notice that in this case, we will discard at most $|U|=n$ vertices. Therefore, if we can prove that the probability of any bad event happening is less than $1/(2n)$, then the expected solution cost will remain close to the optimal one. The result of the second stage is a set $U'$, whose expected cardinality is close to the LP-solution cost, and this solution is almost feasible: namely, for every level $h$ and every level-$h$ color $c_h$, the number of vertices in $U'$ whose level-$h$ color is $c_h$ is at most $d_h\cdot \poly\log(n)$. In the third stage, we turn the solution $U'$ into a feasible one, at the cost of losing a polylogarithmic factor on its cardinality.


For convenience, we let $Q_0$ denote the whole grid $\tilde G$, and we define a unique level-$0$ color $c_0$; every level-1 color $c_1\in \chi_1$ is a child-color of $c_0$. We assume that $Q_0$ is assigned the level-$0$ color $c_0$.


%--------------------------------------------------
%--------------------------------------------------
\subsection*{Stage 1: Randomized Rounding}
%--------------------------------------------------
%--------------------------------------------------
We perform $\rho$ iterations, where in iteration $h$ we settle the colors of all level-$h$ squares, by suitably modifying the LP-solution. 
We will maintain the following invariant:

\begin{properties}{P}
\item For all $1\leq h\leq \rho$, at the beginning of iteration $h$, the current LP-solution ($x', y'$) has the following properties.  For every level-$(h-1)$ square $Q_{h-1}$, if $c_{h-1}$ is the level-$(h-1)$ color assigned to $Q_{h-1}$, then for every level $h-1<h'\leq \rho$, for every level-$h'$ descendant-square $Q_{h'}\in \dset_{h'}(Q_{h-1})$, and every level-$h'$ color $c_{h'}\in \chi_{h'}$:  \label{invariant}

\begin{itemize}
\item If $c_{h'}$ is not a descendant-color of $c_{h-1}$, then $x'(Q_{h'},c_{h'})=0$ (and if $h'=\rho$ then $y'(Q_{h'},c_{h'})=0$);

\item Otherwise, $x'(Q_{h'},c_{h'})=x(Q_{h'},c_{h'})/x(Q_{h-1},c_{h-1})$. Moreover, if $h'=\rho$, then $y'(Q_{h'},c_{h'})=y(Q_{h'},c_{h'})/x(Q_{h-1},c_{h-1})$.
\end{itemize}
\end{properties}

(Here, the $x$ and the $y$-variables are the ones from the original LP-solution).


In order to perform the first iteration, each level-$1$ square $Q_1\in \qset_1$ chooses one of the colors $c_1\in \chi_1$, where each color $c_1$ is chosen with probability $x(Q_1,c_1)$ (recall that by Constraint~(\ref{LP: sum of colors 1 for level 1}), $\sum_{c_1\in \chi_1}x(Q_1,c_1)=1$). Assume now that we have chosen color $c_1$ for square $Q_1$. We update the LP-solution. For every level $2\leq h\leq \rho$, every level-$h$ square $Q_h\in \dset_h(Q_1)$, and every level-$h$ color $c_h$, we do the following: if $c_h$ is not a descendant color of $c_1$, then we set $x'(Q_h,c_h)=0$ (if $h=\rho$, then we also set $y'(Q_h,c_h)=0$). Otherwise, we set $x'(Q_h,c_h)=x(Q_h,c_h)/x(Q_1,c_1)$ (similarly, if $h=\rho$, then we also set $y'(Q_h,c_h)=y(Q_h,c_h)/x(Q_1,c_1)$). We then continue to the next iteration.

%Consider now some iteration $h>1$. We assume that we have selected colors for all level-$(h-1)$ squares. Fix some such square $Q_{h-1}$ and a color $c_{h-1}$ that was selected for it. 
The invariant clearly holds at the beginning of the second iteration. Assume now that it holds at the beginning of iteration $h$. The iteration is executed as follows. Consider some level-$h$ square $Q_h$. Suppose its parent square is $Q_{h-1}$, and it was assigned color $c_{h-1}$. Then Constraint~(\ref{LP: color coordination across levels}), together with  Invariant (\ref{invariant}) ensures that:

\[\sum_{c_h\in \tilde{\chi}_h(c_{h-1})}x'(Q_h,c_h)=1.\]

Square $Q_h$ chooses one of the child-colors $c_h$ of $c_{h-1}$, where color $c_h$ is chosen with probability $x'(Q_h,c_h)$.  Assume that we have assigned color $c_h$ to square $Q_h$. We now update the LP-solution. Consider some level $h<h'\leq \rho$, some level-$h'$ square $Q_{h'}\in \dset_{h'}(Q_{h})$ that is a descendant of $Q_{h}$, and some level-$h'$ color $c_{h'}\in \chi_{h'}$. Assume first that if $c_{h'}$ is not a descendant color of $c_{h}$. Then we set $x''(Q_{h'},c_{h'})=0$ (if $h'=\rho$, then we also set $y''(Q_{h'},c_{h'})=0$). Assume now that $c_{h'}$ is a descendant color of $c_{h}$. Let $Q_{h-1}$ be the parent-square of $Q_h$, and let $c_{h-1}$ be the parent-color of $c_h$. Then we set:

\[x''(Q_{h'},c_{h'})=\frac{x'(Q_{h'},c_{h'})}{x'(Q_h,c_h)}=\frac{x(Q_{h'},c_{h'})/x(Q_{h-1},c_{h-1})}{x(Q_h,c_h)/x(Q_{h-1},c_{h-1})}=\frac{x(Q_{h'},c_{h'})}{x(Q_h,c_h)}.\]

 (We have used the fact that  Invariant (\ref{invariant}) held at the beginning of the current iteration).
Similarly, if $h=\rho$, then we set:

\[y''(Q_{h'},c_{h'})=\frac{y'(Q_{h'},c_{h'})}{x'(Q_h,c_h)}=\frac{y(Q_{h'},c_{h'})/x(Q_{h-1},c_{h-1})}{x(Q_h,c_h)/x(Q_{h-1},c_{h-1})}=\frac{y(Q_{h'},c_{h'})}{x(Q_h,c_h)}.\]

We then replace solution $(x',y')$ with the new solution $(x'',y'')$.
This completes the description of iteration $h$. Observe that Invariant (\ref{invariant}) continues to hold at the end of the current iteration.

The final iteration $\rho$ is executed as follows. For every level-$\rho$ square $Q_{\rho}\in \qset_{\rho}$, we select a level-$\rho$ color $c_{\rho}$ for $Q_{\rho}$ exactly as before, but we do not update the LP-solution. If $\frac{y'(Q_{\rho},c_{\rho})}{x'(Q_{\rho},c_{\rho})}\geq 1$, then we add $\ceil{\frac{y'(Q_{\rho},c_{\rho})}{x'(Q_{\rho},c_{\rho})}}$ distinct  vertices of $Q_{\rho}\cap U$, whose level-$\rho$ color is $c_{\rho}$  to our solution  $U'$. This quantity is guaranteed to be bounded by $n(Q_{\rho},c_{\rho})$, 
due to constraint~(\ref{LP: bounding rho colored vertices in each square}) and Invariant (\ref{invariant}). Otherwise, with probability $\frac{y'(Q_{\rho},c_{\rho})}{x'(Q_{\rho},c_{\rho})}$, we add one vertex of $Q_{\rho}\cap U$ whose level-$\rho$ color is $c_{\rho}$ to our solution, and add $0$ such vertices with the remaining probability. (Recall that $\frac{y'(Q_{\rho},c_{\rho})}{x'(Q_{\rho},c_{\rho})}=\frac{y(Q_{\rho},c_{\rho})}{x(Q_{\rho},c_{\rho})}$ from Invariant (\ref{invariant}) --- we use this fact later.) The following theorem concludes the analysis of Stage 1.


%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
\begin{theorem}\label{thm: stage 1 analysis}
The expected number of vertices added to $U'$ at Stage 1 is at least $\sum_{c_{\rho}\in \chi_{\rho}}Y_{\rho}(c_{\rho})$.
\end{theorem}
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------

\begin{proof}
Consider some color $c_{\rho}\in \chi_{\rho}$. Recall that $Y_{\rho}(c_{\rho})=\sum_{Q_{\rho}\in \qset_{\rho}}y(Q_{\rho},c_{\rho})$ due to Constraint~(\ref{LP: accounting for Yrho}). For each level-$\rho$ square $Q_{\rho}$ we define a new random variable $z(Q_{\rho},c_{\rho})$ to be the number of vertices of $Q_{\rho}$, whose level-$\rho$ color is $c_{\rho}$, that are added to the solution $U'$ (this number may only be non-zero if $Q_{\rho}$ is assigned the color $c_{\rho}$). It is now enough to prove that $\expect{z(Q_{\rho},c_{\rho})}\geq y(Q_{\rho},c_{\rho})$. From now on we fix a square $Q_{\rho}$ and a color $c_{\rho}$ and prove the above inequality for them. We use the following claim:

\begin{claim}
The probability that square $Q_{\rho}$ is assigned color $c_{\rho}$ is $x(Q_{\rho},c_{\rho})$.
\end{claim}
\begin{proof}
For all $1\leq h<\rho$, let $Q_h$ be the level-$h$ ancestor-square of $Q_{\rho}$, and let $c_h$ the level-$h$ ancestor-color of $c_{\rho}$. For all $1\leq h\leq \rho$, let $\event_h$ be the event that square $Q_h$ is assigned color $c_h$. Then:

\[\prob{\event_1}=x(Q_1,c_1).\]

We now fix some $1<h\leq \rho$, and analyze the probability of event $\event_h$, assuming that event $\event_{h-1}$ has happened. Let $x',y'$ denote the LP-solution at the beginning of iteration $h$. Then:

\[\prob{\event_h\mid\event_{h-1}}=x'(Q_h,c_h)=\frac{x(Q_h,c_h)}{x(Q_{h-1},c_{h-1})}.\]

Therefore:

\[
\begin{split} 
\prob{\event_{\rho}}&=\prob{\event_{\rho}\mid \event_{\rho-1}}\cdot \prob{\event_{\rho-1}\mid \event_{\rho-2}} \cdots \prob{\event_2\mid \event_1}\cdot \prob{\event_1}\\
&=\frac{x(Q_{\rho},c_{\rho})}{x(Q_{\rho-1},c_{\rho-1})}\cdot \frac{x(Q_{\rho-1},c_{\rho-1})}{x(Q_{\rho-2},c_{\rho-2})}\cdots \frac{x(Q_{2},c_{2})}{x(Q_{1},c_{1})}\cdot x(Q_{1},c_{1})\\
&=x(Q_{\rho},c_{\rho}).\end{split}\]
\end{proof}

We are now ready to complete the proof of Theorem~\ref{thm: stage 1 analysis}.
Assume first that $\frac{y(Q_{\rho},c_{\rho})}{x(Q_{\rho},c_{\rho})}\geq 1$. Then, if $Q_{\rho}$ is assigned color $c_{\rho}$ (which happens with probability $x(Q_{\rho},c_{\rho})$), we select  $\ceil{\frac{y(Q_{\rho},c_{\rho})}{x(Q_{\rho},c_{\rho})}}$ vertices of $Q_{\rho}$, whose level-$\rho$ color is $c_{\rho}$ to the solution. Therefore, $\expect{z(Q_{\rho},c_{\rho})}\geq y(Q_{\rho},c_{\rho})$.

Assume now that $\frac{y(Q_{\rho},c_{\rho})}{x(Q_{\rho},c_{\rho})}< 1$. Then,  if $Q_{\rho}$ is assigned color $c_{\rho}$ (which again happens with probability $x(Q_{\rho},c_{\rho})$), we add one vertex of $Q_{\rho}$, whose level-$\rho$ color is $c_{\rho}$, with probability $\frac{y(Q_{\rho},c_{\rho})}{x(Q_{\rho},c_{\rho})}$. Clearly, in this case, $\expect{z(Q_{\rho},c_{\rho})}= y(Q_{\rho},c_{\rho})$.
\end{proof}

%-----------------------------------------------------------
%-----------------------------------------------------------
%-----------------------------------------------------------
\subsection*{Stage 2: Ensuring that the Solution is Almost Feasible}
%-----------------------------------------------------------
%-----------------------------------------------------------
%-----------------------------------------------------------
In this stage, for each level $1\leq h\leq \rho$ and for each level-$h$ color $c_h\in \chi_h$, we inspect the number of vertices in the solution $U'$ that we constructed at stage 1, whose level-$h$ color is $c_h$. If this number is greater than $64d_h\log^3n$, then we say that color $c_h$ has failed. In that case, we return an empty solution. We think of this as deleting all vertices from our solution, so overall at most $n$ vertices are deleted. 
We will use the following standard Chernoff bound (see e.g. \cite{measure-concentration}).

\begin{theorem}\label{thm: Chernoff}
Let $\set{X_1,\ldots,X_r}$ be a collection of independent random variables taking values in $[0,1]$, and let $X=\sum_iX_i$. Denote $\mu=\expect{X}=\sum_i\expect{X_i}$. Then for all  $0<\eps<1$:


\[\prob{X>(1+\eps)\mu }\leq e^{-\eps^2\mu /3},\]

and 
\[
\prob{X<(1-\eps)\mu}\leq e^{-\eps^2\mu/2}.\]
\end{theorem}

\begin{corollary}\label{cor: Chernoff upper bound}
Let $X_1,\ldots,X_r$ be a collection of independent random variables taking values in $[0,d]$ for some integer $d>0$, and let $X=\sum_iX_i$. Denote $\mu=\expect{X}=\sum_i\expect{X_i}$. Then for all  $0<\eps<1$:


\[\prob{X>(1+\eps)\mu }\leq e^{-\eps^2\mu /(3d)},\]

and 
\[
\prob{X<(1-\eps)\mu}\leq e^{-\eps^2\mu/(2d)}.\]
\end{corollary}

(The Corollary is obtained by replacing each variable $X_i$ with a variable $X'_i=X_i/d$ and then applying Theorem~\ref{thm: Chernoff}).
Following is the main theorem for the analysis of Stage 2.

\begin{theorem}\label{thm: stage 2 bad events}
Fix some level $1\leq h\leq\rho$ and some level-$h$ color $c_h\in \chi_h$. The probability that color $c_h$ fails is at most $1/(2n^3)$.
\end{theorem}

Note that there are at most $n$ colors at each level, and $\rho= O(\sqrt{\log n})$ levels. Therefore, using the union bound, we obtain the following corollary.

\begin{corollary}\label{cor: any color fails}
The probability that any color fails is at most $1/(2n)$.
\end{corollary}

We now turn to prove Theorem~\ref{thm: stage 2 bad events}.


%--------------------------------------------
%--------------------------------------------
%--------------------------------------------
%--------------------------------------------
%--------------------------------------------
\begin{proofof}{Theorem \ref{thm: stage 2 bad events}}
We assume that the level $h$ and the color $c_h$ are fixed. 
For consistency, we define a fractional solution $(x',y')$ obtained at the end of iteration $\rho$, as follows. Consider a level-$\rho$ square $Q_{\rho}$, and let $c_{\rho}$ be the level-$\rho$ color that was assigned to it at the end of iteration $\rho$. Then we set $x'(Q_{\rho},c_{\rho})=1$, and $y'(Q_{\rho},c_{\rho})=y(Q_{\rho},c_{\rho})/x(Q_{\rho},c_{\rho})$. For every other level-$\rho$ color $c'_{\rho}$, we set $x'(Q_{\rho},c'_{\rho})=0$, and $y'(Q_{\rho},c'_{\rho})=0$.

For simplicity, we denote $\chi'=\tilde{\chi}_{\rho}(c_h)$ - the set of all descendant-colors of $c_h$ at level $\rho$. For every level $1\leq h'\leq \rho$, we define a random variable $N_{h'}$, whose intuitive meaning is the number of color-$c_h$ vertices in the fractional solution, that is obtained at the end of iteration $h'$. 

Formally, let $(x',y')$ be the solution obtained at the end of iteration $h'$. 
Then: $$N_{h'}=\sum_{Q_{\rho} \in \qset_{\rho}}\sum_{c_{\rho}\in \chi'}y'(Q_{\rho},c_{\rho}).$$


For all $1\leq h'\leq \rho$, we define a bad event $\event_{h'}$ to be the event that $N_{h'}>d_h\cdot 16(1+1/\log n)^{h'}\log^3n$. The following lemma is central to the analysis.


%--------------------------------------------
%--------------------------------------------
%--------------------------------------------
\begin{lemma}\label{lem: bounding event rho}
$\prob{\event_{\rho}}\leq \frac 1{4n^3}$.
\end{lemma}
%--------------------------------------------
%--------------------------------------------
%--------------------------------------------



If $\event_{\rho}$ does not happen, then, if we denote by $(x',y')$ the solution obtained at the end of iteration $\rho$: 

\[N_{\rho}=\sum_{Q_{\rho}\in \qset_{\rho}}\sum_{c_{\rho}\in \chi'}y'(Q_{\rho},c_{\rho})<16d_h\left(1+\frac{1}{\log n}\right)^{\rho}\log^3n<32d_h\log^3n,\] 

since $\rho\leq \sqrt{\log n}$.

Recall that for every square $Q_{\rho}\in \qset_{\rho}$, if $y'(Q_{\rho},c_{\rho})\geq 1$, then we add $\ceil{y'(Q_{\rho},c_{\rho})}$ vertices of $Q_{\rho}$, whose level-$\rho$ color is $c_{\rho}$ to the solution. Otherwise, with probability $y'(Q_{\rho},c_{\rho})$, we add only one such vertex to our solution. Overall, from Theorem~\ref{thm: Chernoff}, it is immediate to verify that, if event $\event_{\rho}$ does not happen, then with probability at least $(1-1/n^4)$, the number of vertices in $U'$, whose level-$h$ color is $c_h$ is at most $2N_{\rho} \leq  64d_h\log^3n$. It now remains to prove Lemma~\ref{lem: bounding event rho}.


%--------------------------------------------
%--------------------------------------------
%--------------------------------------------

\begin{proofof}{Lemma \ref{lem: bounding event rho}}
For convenience, we also define event $\event_0$ that $N_0>d_h$, which, from Constraints~(\ref{LP: Yh is sum of Yrhos}) and (\ref{LP: bound of Yh by kh}) happens with probability $0$. Clearly,

\[\begin{split}
\prob{\event_{\rho}}&\leq\prob{\event_{\rho}\mid\neg \event_{\rho-1}}\cdot \prob{\neg \event_{\rho-1}}+\prob{\event_{\rho-1}}\\
&\leq\prob{\event_{\rho}\mid\neg \event_{\rho-1}}+\prob{\event_{\rho-1}\mid\neg \event_{\rho-2}}\cdot \prob{\neg\event_{\rho-2}}+\prob{\event_{\rho-2}} \\
&\vdots\\
&\leq \sum_{h'=1}^{\rho}\prob{\event_{h'}\mid \neg\event_{h'-1}}.
\end{split}
\]

We now analyze $\prob{\event_{h'}\mid \neg \event_{h'-1}}$. The following claim will finish the proof of the lemma.


%-----------------------------------------
%-----------------------------------------
%-----------------------------------------
\begin{claim}
For all $1\leq h'\leq \rho$, $\prob{\event_{h'}\mid \neg \event_{h'-1}}\leq 1/(4n^4)$.
\end{claim}

%-----------------------------------------
%-----------------------------------------
%-----------------------------------------

\begin{proof}
Fix some $1\leq h'\leq \rho$. Let $(x',y')$ be the solution at the beginning of iteration $h'$, and let $(x'',y'')$ be the solution at the end of iteration $h'$. 
We will repeatedly use Constraint~(\ref{LP: color coordination with kh across levels}) that we restate here; we slightly change the indexing to avoid confusion with the variables $h$ and $h'$ that we use here.

The constraint states that for all pairs $1\leq \tilde h\leq \tilde h'\leq \rho$ of levels, for every level-$\tilde h$ square $Q_{\tilde h}\in \qset_{\tilde h}$ and for every pair of a level-$\tilde h$ color $c_{\tilde h}$ and a level-$\tilde h'$ color $c_{\tilde h'}$, that is a descendant-color of $c_{\tilde{h}}$, the following inequality holds: 

\begin{equation}
\sum_{Q_{\rho}\in \dset_{\rho}(Q_{\tilde h})}\sum_{c_{\rho}\in \tilde{\chi}_{\rho}(c_{\tilde h'})}y(Q_{\rho},c_{\rho})\leq d_{\tilde h'}\cdot x(Q_{\tilde h},c_{\tilde h}). \label{LP-constraint restatement}
\end{equation}

Intuitively, if $Q_{\tilde h}$ is assigned the color $c_{\tilde h}$, then at most $d_{\tilde h'}$ vertices of $Q_{\tilde h}$ may be assigned the level-$\tilde h'$ color $c_{\tilde h'}$; otherwise, none of them can. Notice that due to Invariant~(\ref{invariant}), the above constraint remains valid with respect to the solution $(x',y')$, if $\tilde h\geq h'$. %obtained at the end of every iteration $h'<\tilde h$.


Consider some level-$h'$ square $Q_{h'}\in \qset_{h'}$. We assume that its parent-square is $Q_{h'-1}$, and that it was assigned some color $c_{h'-1}$. Recall that $(x',y')$ is the LP-solution at the beginning of iteration $h'$, and $(x'',y'')$ is the LP-solution at the end of iteration $h'$.
We define:

\[M'(Q_{h'})=\sum_{Q_{\rho}\in \dset_{\rho}(Q_{h'})}\sum_{c_{\rho}\in \chi'}y'(Q_{\rho},c_{\rho}),\]

and we define $M''(Q_{h'})$ similarly with respect to $y''$. Intuitively, $M'(Q_{h'})$ is the number of vertices of $Q_{h'}$ that are (possibly fractionally) assigned the level-$h$ color $c_h$ at the beginning of iteration $h'$, while $M''(Q_{h'})$ reflects the same quantity at the end of iteration $h'$.
The values of variables $M'(Q_{h'})$ are fixed at the beginning of iteration $h'$, while the values $M''(Q_{h'})$ are random variables.
Then:

\[N_{h'-1}=\sum_{Q_{h'}\in \qset_{h'}}M'(Q_{h'}),\]

and since we assume that event $\event_{h'-1}$ did not happen, $N_{h'-1}\leq d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n$. Similarly,

\[N_{h'}=\sum_{Q_{h'}\in \qset_{h'}}M''(Q_{h'}),\]

and it is enough to prove that the probability that $N_{h'}>16(1+1/\log n)^{h'}\log^3n$ is less than $1/(4n^4)$.

We consider two cases, depending on whether $h>h'$ holds.


\paragraph*{Case 1: $h>h'$.}
Let $c_{h'}$ be the unique ancestor-color of color $c_h$, that belongs to level $h'$.
 Using Constraint~(\ref{LP-constraint restatement}) with $\tilde h= h'$ and $\tilde h'=h$, we get that of each such level-$h'$ square $Q_{h'}$:


\[M'(Q_{h'})\leq d_{h}x'(Q_{h'},c_{h'}).\]

If $Q_{h'}$ is assigned the color $c_{h'}$ (which happens with probability at most $x'(Q_{h'},c_{h'})$), then $M''(Q_{h'})=M'(Q_{h'})/x'(Q_{h'},c_{h'})\leq d_{h}$; otherwise $M''(Q_{h'})=0$. Therefore, $\set{M''(Q_{h'})}_{Q_{h'}\in \qset_{h'}}$ is a collection of independent random variables taking values between $0$ and $d_{h}$, and:

\[\expect{N_{h'}}=\sum_{Q_{h'}\in \qset_{h'}}\expect{M''(Q_{h'})}=\sum_{Q_{h'}\in \qset_{h'}}M'(Q_{h'})=N_{h'-1}\leq d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n.\]

%whose expectation is $N_{h'-1}\leq d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n$. 

Let $\mu=d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n$.  From Corollary~\ref{cor: Chernoff upper bound}:

\[\prob{N_{h'}\geq (1+1/\log n)\mu}\leq e^{{-\mu}/{(3{d_h}\log^2n)}}\leq e^{-5\log n}\leq 1/(4n^4), \]

as required

 \paragraph*{Case 2: $h\leq h'$.}
Let $Q_{h'}\in \qset_{h'}$ be any level-$h'$ square, and let $c_{h'}\in \tilde{\chi}_{h'}(c_h)$ be any level-$h'$ descendant-color of $c_h$.
 Using Constraint~(\ref{LP-constraint restatement}) with $\tilde h=\tilde h'=h'$, we get that:
 
 \[\sum_{Q_{\rho}\in\dset_{\rho}(Q_{h'})}\sum_{c_{\rho}\in \tilde \chi_{\rho}(c_{h'})}y'(Q_{\rho},c_{\rho})\leq d_{h'}\cdot x'(Q_{h'},c_{h'}).\]
 
 Denote the left-hand-side by this inequality by $M'(Q_{h'},c_{h'})$, so:
 
 \[M'(Q_{h'},c_{h'})=\sum_{Q_{\rho}\in\dset_{\rho}(Q_{h'})}\sum_{c_{\rho}\in \tilde \chi_{\rho}(c_{h'})}y'(Q_{\rho},c_{\rho}),\]
 
 and
 
 \[M'(Q_{h'})=\sum_{c_{h'}\in \tilde{\chi}_{h'}(c_h)} M'(Q_{h'},c_{h'}).\]
 
 
For each color $c_{h'}\in \tilde{\chi}_{h'}(c_h)$, if $Q_{h'}$ is assigned the color $c_{h'}$ (which happens with probability $x'(Q_{h'},c_{h'})$), then $M''(Q_{h'})=M'(Q_h',c_{h'})/x'(Q_{h'},c_{h'})\leq d_{h'}\leq d_h$. If none of the colors in $\tilde{\chi}_{h'}(c_h)$ are assigned to $Q_{h'}$, then $M''(Q_{h'})=0$.
Therefore, the expectation of $M''(Q_{h'})$ is:

\[\expect{M''(Q_{h'})}=\sum_{c_{h'}\in \tilde{\chi}_{h'}(c_h)}M'(Q_{h'},c_{h'})=M'(Q_{h'}).\]

Overall, we conclude that variables in set $\set{M''(Q_{h'})}_{Q_{h'}\in \qset_{h'}}$ are independent random variables, taking values in $[0,d_h]$, and that:

\[\expect{N_{h'}}=\sum_{Q_{h'}\in \qset_{h'}}\expect{M''(Q_{h'})}=\sum_{Q_{h'}\in \qset_{h'}}M'(Q_{h'})=N_{h'-1}\leq d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n.\]
Let $\mu=d_h\cdot 16(1+1/\log n)^{h'-1}\log^3n$. From Corollary~\ref{cor: Chernoff upper bound}:

\[\prob{N_{h'}\geq (1+1/\log n)\mu}\leq e^{{-\mu}/{(3{d_h}\log^2n)}}\leq e^{-5\log n}\leq 1/(4n^4). \]
\end{proof} %(of Claim)
%-----------------------------------------
%-----------------------------------------
%-----------------------------------------
\end{proofof} %(of Lemma)
\end{proofof} %(of Thm)


%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
\subsection*{Stage 3: Turning the Solution into a Feasible One}
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------
%--------------------------------------------------

 If any of the colors fail, then we return an empty solution. 
Assume now that no color fails. Let $U'\subseteq U$ be the set of all vertices chosen by the current solution.

\begin{claim}\label{claim: stage 3} There is an efficient algorithm to compute a subset $U''\subseteq U'$ of vertices, with $|U''|\geq \frac{|U'|}{256\log^4n}$, such that $U''$ is a feasible solution to the \HSC problem.
\end{claim}

\begin{proof}
 If, for every level $h$, for every level-$h$ color $c_h$, at most $d_h$ vertices of $U'$ are assigned the level-$h$ color $c_h$, then we return the set $U'$ of vertices, which is a feasible solution to the \HSC problem instance.

Otherwise, denote $r=|U'|$, and consider an ordering $(u_1,u_2,\ldots,u_r)$ of the vertices of $U'$, that has the following property: for every level $1\leq h\leq \rho$, for every level-$h$ color $c_h\in \chi_h$, the vertices of $U'$ whose level-$h$ color is $c_h$ appear consecutively in this ordering. Due to the nested definition of the colors, it is easy to see that such an ordering exists (in particular, we can use the ordering induced by the ordering of the original source vertices on $R^*$). We now let $U''$ contain all vertices $u_i\in U'$, where $i = 1\mod \ceil{128\log^4n}$. It is now immediate to verify that $|U''|\geq \frac{|U'|}{256\log^4n}$, and that it is a feasible solution to the \HSC problem.
\end{proof}
%
%
%
\iffalse
we perform a slight transformation to the solution $U'$.
The hierarchical structure of the set $\cset$ of colors naturally defines a tree $T$: for every level $0\leq h\leq \rho$, and every level-$h$ color $c_h$, we add a vertex $v(c_h)$ to the tree. We associate with this vertex the subset $U'(c_h)\subseteq U'$ of vertices, whose level-$h$ color is $c_h$. We add an edge between $v(c)$ and $v(c')$ whenever $c'$ is a child-color of $c$. We view the tree as rooted at the vertex $v(c_0)$, corresponding to the unique level-$0$ color $c_0$. We say that a vertex $v(c)$ is \emph{important} iff $|U'(c)|\geq 64\log^4n$. We mark every vertex $v(c)$, such that (i) $v(c)$ is important; and (ii) no descendant of $v(c)$ in the tree $T$ is important. Note that if $v(c)$ and $v(c')$ are marked, then $U'(c)\cap U'(c')=\emptyset$. Let $v(c)$ be any marked vertex. Let $U''(c)\subseteq U'(c)$ be any subset of $\floor{\frac{|U'(c)|}{32\log^4n}}$ vertices. We delete from $U'$ all vertices of $U'(c)\setminus U''(c)$. Once we process all marked vertices this way, since $d_h>32\log^4n$ for all $h$, it is easy to verify that the resulting set $U''$ of vertices has the property that for each level $h$, for each level-$h$ color $c_h$, at most $d_h$ vertices of $U''$ have the level-$h$ color $c_h$. In other words, $U''$ is a feasible solution to the \HSC problem. It is easy to verify that  $|U''|\geq \frac{|U'|}{64\log^4n}$.
\fi
%\end{proof}

Let $\optLP$ denote the value of the optimal LP solution.
% We think of the algorithm described in Claim~\ref{claim: stage 3} as Stage 3 of the algorithm.
Let $N_1$ be the total number of vertices that belong to the solution at the end of phase $1$, so $\expect{N_1}=\optLP$. Let $N_2$ be the total number of vertices that were deleted during the second phase. Then with probability at least $(1-1/(2n))$, $N_2=0$, and with the remaining probability, $N_2\leq n$. Therefore, $\expect{N_2}\leq 1/2$. Finally, let $N_3$ denote the cardinality of the final set $U''$ of vertices that our algorithm returns. Then:

\[N_3\geq \frac{N_1-N_2}{256\log^4n},\]

and therefore, $\expect{N_3}\geq \frac{\optLP}{512\log^4n}$. 
Since $U''$ is a feasible solution to the \HSC problem, $N_3 \leq \optLP$.

\begin{claim}
    $\prob{N_3 \geq \frac{\optLP}{1024\log^4 n}} \geq \frac1 {1024\log^4 n}$
\end{claim}
\begin{proof}
    Assume otherwise. Then:
    
    
    \[ \expect{N_3} < \left ( \frac{1}{1024\log^4 n} \cdot \optLP \right ) + \frac{\optLP}{1024\log^4 n} <\left (\frac{\optLP}{512\log^4 n} \right ),\]
    
    a contradiction.
\end{proof}

We run the above algorithm $c\log^5n$ times independently (for some large constant $c$), and return a solution of largest cardinality across all runs. The probability that the solution value is less than $\optLP/(1024\log^4n)$ is then bounded by $1/\poly(n)$. This concludes the proof of Theorem \ref{thm: main finding the coloring}.
%\mynote{need this to happen w.h.p.}




==> arxiv final/existence-of-coloring.tex <==
%-----------------------------------------------------------
%-----------------------------------------------------------
%-----------------------------------------------------------
\label{---------------------------------------sec: existence of coloring----------------------}
%-----------------------------------------------------------
\section{The Existence of Coloring}\label{sec: existence of coloring}
%-----------------------------------------------------------
%-----------------------------------------------------------
%-----------------------------------------------------------
In this section we prove Theorem~\ref{thm: existence of perfect set}. Recall that we assume that we are given a lower bound $\opt$ on the value of the optimal solution; a hierarchical system $\thset=(\qset_1,\ldots,\qset_{\rho})\in \fset$, and a sequence $L=(\ell_1,\ldots,\ell_{\rho})$ of integers as in Theorem~\ref{thm: partition of R1}. As before, we denote by $(\jset_1,\ldots,\jset_{\rho})$ the $L$-hierarchical decomposition of $R^*$. From Theorem~\ref{thm: partition of R1}, there is a set $\tmset^{**}$ of demand pairs, with $|\tmset^{**}|\geq \opt/2^{O(\sqrt{\log n}\log \log n)}$, such that for all demand pairs in $\tmset^{**}$, their destinations belong to $\thset$, so in particular $\tmset^{**}\subseteq \tmset$. Moreover, all demand pairs in $\tmset^{**}$ can be routed via node-disjoint paths in $G$,  
 all squares in $\bigcup_{h=1}^{\rho}\qset_h$ have the $1/\eta^2$-shadow property with respect to $\tmset^{**}$, and
 the set $\tmset^{**}$ of demand pairs is compatible with the sequence $L$. Recall that the latter means that for each $1\leq h\leq \rho$, for every level-$h$ interval $I\in \jset_h$ of $R^*$, either $I\cap S(\tmset^{**})=\emptyset$, or $d_h/(16\eta)\leq |S(\tmset^{**})\cap I|\leq d_h/4$.
 
 For each $1\leq h\leq \rho$, for every level-$h$ square $Q\in \qset_h$, let $\hmset(Q)\subseteq \tmset^{**}$ denote the set of all demand pairs whose destinations lie in $Q$.
 We use the following simple observation.
 
 \begin{observation}\label{obs: squares spanning few intervals}
 For each $1\leq h\leq \rho$, for every level-$h$ square $Q\in \qset_h$, the source vertices of the demand pairs in $\hmset(Q)$ belong to at most two level-$h$ intervals in $\jset_h$.
 \end{observation}
 
 \begin{proof}
 Assume otherwise, and let $I',I'',I'''\in \jset_h$ be three distinct level-$h$ intervals that  each contain at last one source vertex of $\hmset(Q)$. Assume that $I',I'',I'''$ lie on $R^*$ in this left-to-right order. Then $I''$ is contained in the shadow $L_{\hmset}(Q)$. From the $1/\eta^2$-shadow property of $Q$, the length of this shadow must be at most $d_h/\eta^2$. But from our construction, the length of the shadow is at least $|S(\tmset^{**})\cap I''|\geq d_h/(16\eta)> d_h/\eta^2$, a contradiction.
 \end{proof}
 
 We start with the set $\hmset_0=\tmset^{**}$ of demand pairs, and perform $\rho$ iterations. In iteration $h$, the input is some subset $\hmset_{h-1}\subseteq \hmset_0$ of demand pairs, and an assignment of level-$(h-1)$ colors to all level-$(h-1)$ squares, that has the following property: for each demand pair $(s,t)\in \hmset_{h-1}$, if $Q\in \qset_{h-1}$ is the level-$(h-1)$ square containing $t$, and $I\in \jset_{h-1}$ is the level-$(h-1)$ interval containing $s$, then $Q$ and $I$ are assigned the same level-$(h-1)$ color, or in other words, $Q$ is assigned the level-$(h-1)$ color $c_{h-1}(I)$.
 Our starting point is the set $\hmset_0$ of demand pairs. We assume that the level-$0$ color of all vertices is $c_0$, so, letting $\tilde G$ be a unique level-$0$ square, the invariant holds.
 
 Consider now some iteration $h$, together with the corresponding set $\hmset_{h-1}\subseteq \tmset^{**}$ of demand pairs. Consider some level-$h$ square $Q\in \qset_h$, and assume that its parent-square is assigned the level-$(h-1)$ color $c_{h-1}$. Let $\hmset'(Q)\subseteq \hmset_{h-1}$ be the set of all demand pairs, whose destinations lie in $Q$. From the above observation, there are at most two level-$h$ intervals of $R^*$ (that we denote by $I$ and $I'$, where possibly $I=I'$) that contain the source vertices of $\hmset'(Q)$. Assume w.l.o.g. that $I$ contains at least half of these source vertices. From our invariant, all vertices of the parent-interval of $I$ are also assigned the level-$(h-1)$ color $c_{h-1}$ - same as the color assigned to the parent-square of $Q$. We then assign to $Q$ the level-$h$ color $c_h(I)$ - that is, the color associated with the interval $I$. We also discard from $\hmset'(Q)$ all demand pairs except those whose sources are contained in $I$, obtaining a new set $\hmset''(Q)\subseteq \hmset'(Q)$ of demand pairs, containing at least $|\hmset''(Q)|/2$ demand pairs. We then set $\hmset_h=\bigcup_{Q\in \qset_h}\hmset''(Q)$.
 
 Let $\tmset'=\hmset_{\rho}$ be the set of demand pairs obtained after the last iteration. Then it is immediate to verify that:
 
 \[|\tmset'|\geq \frac{|\tmset^{**}|}{2^{\rho}}\geq \frac{|\tmset^{**}|}{2^{\sqrt{\log n}}}\geq \frac{\opt}{2^{O(\sqrt{\log n}\log \log n)}}.\]
 
 Clearly, for each demand pair $(s,t)\in \tmset'$, both $s$ and $t$ are assigned the same level-$\rho$ color.
 Finally, fix some level $1\leq h\leq \rho$, and some level-$h$ color $c_h(I)$, that is associated with some level-$h$ interval $I$. It remains to verify that at most $d_h$ demand pairs are assigned color $c_h(I)$. This is clearly true, since all such demand pairs have their source vertices lying on $I$, and, since $\tmset^{**}$ is compatible with $L$ from Theorem~\ref{thm: partition of R1}, we are guaranteed that the number of such demand pairs is at most $d_h/4$.
 
 
 

==> arxiv final/general-case.tex <==
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------

\label{-------------------------------------sec: destinations anywhere-----------------------------------}
\section{Approximating \restrictedNDP}\label{sec:destinations anywhere}
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
In this section we complete the proof of Theorem~\ref{thm: main}. 
Suppose we are given an instance $(G,\mset)$ of \RNDP.
We assume that we know the value $\opt$ of the optimal solution to this instance, by going over all such possible choices, and running the algorithm on each of them.
Let $\Gamma_1,\Gamma_2,\Gamma_3$ and $\Gamma_4$ denote the four boundary edges of the grid $G$, and let $\Gamma=\bigcup_{q=1}^4\Gamma_q$ be its full boundary.
For every destination vertex $t\in T(\mset)$, we denote by $\tilde{t}$ the vertex of $\Gamma$ minimizing the distance $d(t,\tilde t)$, breaking ties arbitrarily. 
Recall that, given any subset $\mset'\subseteq \mset$ of the demand pairs, we denoted by $S(\mset')$ and $T(\mset')$ the sets of all vertices that serve as the sources and the destinations of the demand pairs in $\mset'$, respectively. We denote by $\tilde{T}(\mset')=\set{\tilde t\mid t\in T(\mset')}$.

Given two disjoint sub-paths $\pi,\pi'\subseteq \Gamma$ (that we call intervals), and a subset $\mset'\subseteq \mset$ of demand pairs, we let $\mset'_{\pi,\pi'}\subseteq \mset'$ contain all demand pairs $(s,t)$ with $s\in \pi$ and $\tilde t\in \pi'$. %We denote by $\opt(\pi,\pi')$ the value of the optimal solution to instance $(G,\mset(\pi,\pi'))$. 


\subsection{Special Instances}
It will be convenient for us to define special sub-instances of instance $(G,\mset)$, that have a specific structure. 
We start by defining interesting pairs of intervals.

\begin{definition}
Let $I,I'\subseteq \Gamma$ be two disjoint intervals, and let $d>0$ be an integer. We say that $(I,I')$ is a \emph{$d$-interesting pair of intervals}, iff:

\begin{itemize}
\item interval $I'$ is contained in a single boundary edge of $G$, and every vertex of $I'$ is within distance at least $16d$ from each of the remaining three boundary edges of $G$; 
\item interval $I$ is contained in a single boundary edge of $G$ (possibly the same as $I'$);

\item $d\leq |V(I')|\leq  \sqrt{n}/2$, and $d(I,I')\geq 16 d$.
\end{itemize}
\end{definition}

\begin{definition}
Suppose we are given an integer $d>0$, and a pair $(I,I')$ of disjoint intervals of $\Gamma$.
Assume further that we are given a subset $\mset'\subseteq \mset$ of the demand pairs, and consider the sub-instance $(G,\mset')$ of the problem, defined over the same graph $G$, with the set $\mset'$ of demand pairs. We say that $(G,\mset')$ is a \emph{valid $(I,I',d)$-instance} iff:
(i) $S(\mset')\subseteq I$; 
(ii) $\tilde{T}(\mset')\subseteq I'$; and
(iii) for each $t\in T(\mset')$, $d\leq d(t,\tilde t)<2d$.
If, additionally, $(I,I')$ is a $d$-interesting pair of intervals, then we say that $(G,\mset')$ is a \emph{perfect $(I,I',d)$-instance}.
\end{definition}



The main idea of the algorithm is to compute a partition of the set $\mset$ of the demand pairs into subsets $\mset_1,\ldots,\mset_z$, where each set $\mset_i$ is a perfect $(I,I',d)$-instance for some pair $(I,I')$ of intervals. We will then solve the problem defined by each such sub-instance separately, by first casting it as a special case in which the destinations lie far from the grid boundary, and then employing Theorem~\ref{thm: main w destinations far from boundary}. We now define the modified instances, to which Theorem~\ref{thm: main w destinations far from boundary}  will eventually be applied.


\subsection{Modified Instances}
Assume that we are given an integer $d>0$, and a $d$-interesting pair $(I,I')$ of intervals, together with a perfect $(I,I',d)$-sub-instance $(G,\mset')$ of $(G,\mset)$. We define a corresponding \emph{modified instance} $(G',\mset'')$. The underlying graph $G'$ will be an appropriately chosen sub-grid of $G$, and each demand pair in the new set $\mset''$ will correspond to a unique demand pair in $\mset'$.

In order to define the grid $G'$, we assume without loss of generality that $I'$ is a sub-path of the bottom boundary edge of the grid. Let $\wset''$ be the subset of the columns of $G$ that intersect $I'$, and let $\rset''$ be the set of $4d$ bottommost rows of $G$. Let $G''\subseteq G$ be the sub-grid of $G$ spanned by the set $\wset''$ of columns and the set $\rset''$ of rows. In order to obtain the final graph $G'$, we add to $\wset''$ $4d$ columns lying immediately to its left and $4d$ consecutive columns lying immediately to its right, denoting the resulting set of columns by $\wset'$. We also add to $\rset''$ a set of $|\wset'|-4d$ rows lying immediately above $\rset''$, obtaining a set $\rset'$ of rows of $G$. Graph $G'$ is the sub-grid of $G$ spanned by the columns of $\wset'$ and the rows of $\rset'$. Notice that $G'$ is a square grid.

The set $\mset''$ of demand pairs is constructed as follows. For each demand pair $(s,t)\in \mset'$, we add a demand pair $(s',t')$ to $\mset''$. Vertex $t'$ is mapped to the same location as vertex $t$ in $G'$. Vertex $s'$ is mapped to one of the vertices on the top row of $G'$, using the following procedure. Let $X$ denote the set of $|S(\mset')|$ leftmost vertices on the top row of $G'$. Let $v$ be the bottom left corner of the grid $G'$. The traversal of $\Gamma(G)$ in the clock-wise direction, starting from $v$, defines an ordering $\pi$ of the vertices in $S(\mset')$. Similarly, a traversal of $\Gamma(G')$ in the clock-wise direction, starting from $v$, defines an ordering $\pi'$ of the vertices in $X$. Consider some vertex $s\in S(\mset')$, and assume that it is the $i$th vertex of $S(\mset')$ according to the ordering $\pi$. We map it to the $i$th vertex of $X$, according to the ordering $\pi'$.
This finishes the definition of the modified instance $(G',\mset'')$ corresponding to the valid $(I,I',d)$ sub-instance $(G,\mset')$ of $(G,\mset)$. We need the following simple claim, whose proof is straightforward and is deferred to the Appendix.

\begin{claim}\label{claim: modified instance preserves solutions}
Let $d>0$ be an integer, let $(I,I')$ be a $d$-interesting pair of intervals, and let $(G,\mset')$ be a perfect $(I,I',d)$ sub-instance of $(G,\mset)$. Let $\opt'$ be the value of the optimal solution to instance $(G,\mset')$. Then the value of the optimal solution to the corresponding modified instance $(G',\mset'')$ is at least $\min\set{\opt',d}$.
\end{claim}



Let $d>0$ be an integer, let $(I,I')$ be a $d$-interesting pair of intervals, and let $(G,\mset')$ be a valid $(I,I',d)$ sub-instance of $(G,\mset)$. Let $\opt'$ be the value of the optimal solution to this instance.
Consider the corresponding modified instance $(G',\mset'')$ of $(G,\mset')$. Then $(G',\mset'')$, together with the parameter $\opt=\min\set{d,\opt'}$ is a valid input to Theorem~\ref{thm: main w destinations far from boundary}. Even though we do not know the value of this parameter, we can try all $d$ possibilities for it, and apply Theorem~\ref{thm: main w destinations far from boundary} to each one of them, selecting the best resulting solution. We are then guaranteed to compute, with high probability, a solution to instance $(G',\mset'')$, whose value is at least $\frac{\min\set{d,\opt'}}{2^{O(\sqrt{\log n}\log\log n)}}$. We let $\aset(G',\mset'')$ denote the resulting solution, and we let $|\aset(G',\mset'')|$ denote its value.





\subsection{Main Partitioning Theorem}

The following theorem is central to our proof.


%\mynote{Need width at most $\sqrt{n}/2$ or so}
 \begin{theorem}\label{thm: partition into intervals}
Suppose we are given two disjoint intervals $\pi,\pi'$ of $\Gamma$, each of which is contained in a single boundary edge of $G$, an integer $d>0$, and a valid $(\pi,\pi',d)$-instance $(G,\mset')$. Assume further that $|\mset'|\geq 1024 d$, and all demand pairs in $\mset'$ can be simultaneously routed via node-disjoint paths. Let $z=\ceil{\frac{|\mset'|}{160d}}-1$. Then there is a collection $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of disjoint sub-intervals of $\pi$, and a collection $\Sigma'=\set{\sigma_1',\ldots,\sigma'_z}$ of disjoint sub-intervals of $\pi'$, such that:

 \begin{itemize}
 \item the intervals $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order;
 
  \item for every pair of intervals $\sigma\in \Sigma\cup \Sigma'$  and $\sigma'\in \Sigma'$, at least $16d$ vertices of $\Gamma$ separate the two intervals; 
  
  
  \item every interval $\sigma'\in \Sigma'$ contains at least $16d$ and at most $\sqrt{n}/2$ vertices, and lies within distance at least $16d$ from every boundary edge of $G$, except for that containing $\pi'$; and
  
  \item for all $1\leq i\leq z$, the value of the optimal solution of the \NDP instance $(G,\mset'_{\sigma_i,\sigma'_i})$ is at least $d$.
  \end{itemize}
  \end{theorem}
  

  
 Notice that in particular, for each $1\leq i\leq z$, $(\sigma_i,\sigma'_i)$ is a $d$-interesting pair of intervals. Consider the set $\tmset\subseteq \mset$ of all demand pairs, such that for each $(s,t)\in \tmset$, $s\in \pi$, $\tilde t\in \pi'$, and $d\leq d(t,\tilde t)<2d$, and apply Theorem~\ref{thm: partition into intervals} to it. Consider the resulting sets $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ and $\Sigma'=\set{\sigma'_1,\ldots,\sigma'_z}$ of segments. Then for all $1\leq i\leq z$, $(G,\tmset_{\sigma_i,\sigma'_i})$ is a perfect $(\sigma_i,\sigma'_i,d)$-instance. Let $(G_i,\tmset'_{\sigma_i,\sigma'_i})$ denote the corresponding modified instance for $(G,\tmset_{\sigma_i,\sigma'_i})$.
 Then all resulting sub-graphs $G_1,\ldots,G_z$ of $G$ are disjoint. Moreover, since the length of each interval $\sigma'_i$ is bounded by $\sqrt{n}/2$, if we assume w.l.o.g. that $\pi'$ is contained in the bottom boundary of the grid $G$, then, assuming that $d<\sqrt n/8$, the sub-graphs $G_1,\ldots,G_z$ must be disjoint from the top $\sqrt{n}/2-4d$ rows of $G$. For each $1\leq i\leq z$, with high probability, $|\aset(G_i,\tmset'_{\sigma_i,\sigma'_i})|\geq d/\approxfactor$, and so $\sum_{i=1}^z|\aset(G_i,\tmset'_{\sigma_i,\sigma'_i})|\geq |\tmset|/\approxfactor$ with high probability.
We now turn to prove Theorem~\ref{thm: partition into intervals}.
  
 \begin{proofof}{Theorem \ref{thm: partition into intervals}}
 Let $\pset^*$ be the set of node-disjoint paths routing the demand pairs in $\mset'$.
 For each demand pair $(s,t)\in \mset'$, let $P(s,t)\in \pset^*$ be the path routing it. For convenience, we assume that $\pi'$ is contained in the bottom boundary of $G$.
 
For every interval $\sigma'\subseteq \pi'$, let $\mset'(\sigma')\subseteq \mset'$ be the set of all demand pairs $(s,t)$ with $\tilde t\in \sigma'$. Note that it is possible that for $t,t'\in T(\mset')$ with $t\neq t'$, $\tilde t=\tilde t'$. Given a vertex $v\in \sigma'$, we let $I(v)\subseteq \pi'$ be the shortest interval, whose leftmost vertex is $v$, such that $I(v)$ contains at least $16d$ vertices, and $|\mset'(I(v))|\geq 16d$. If no such interval exists, then $I(v)$ is undefined.

\begin{observation}\label{obs: length of int}
For each vertex $v\in \pi'$, if $I(v)$ is defined, then $|\mset'(I(v))|\leq 20d$.
\end{observation}

\begin{proof}
Let $v'$ be the rightmost vertex of $I(v)$, and let $I'=I(v)\setminus\set{v'}$. Since we have chosen $I(v)$ over the shorter interval $I'$, either $|\mset'(I')|<16d$, or $|V(I')|<16 d$. Assume first that the former is true. Since all demand pairs in $\mset'$ are routable via node-disjoint paths, all vertices in $S(\mset')$ are distinct. As for each terminal $t\in T(\mset')$, $d(t,\tilde t)\leq 2d$, there may be at most $2d$ demand pairs $(s,t)\in \mset'$ with $\tilde t=v'$. But $\mset'(I')$ contains all demand pairs of $\mset'(I(v))$ except for those pairs $(s,t)$ with $\tilde t=v'$. Therefore, $|\mset'(I(v))|\leq |\mset'(I')|+2d\leq 18d$.

Assume now that $|V(I')|<16d$. Let $G'\subseteq G$ be the sub-grid of $G$, whose bottom boundary is $I(v)$, and whose height is $2d$. Then the width of $G'$ is $16d$, and its top, left, and right boundary has total length $20d$. All paths routing the demand pairs in $\mset'(I(v))$ have to cross the boundary of $G'$, and so $|\mset'(I(v))|\leq 20d$.
\end{proof} 
 
  Let $\tilde T=\set{\tilde t\mid t\in T(\mset')}$. We start by defining a sequence $(\mu_1,\ldots, \mu_{2z+2})$ of $2z+2$ disjoint intervals of $\pi'$, as follows. Let $v_1$ be the first vertex of $\pi'$. We then set $\mu_1=I(v_1)$. Assume now that we have defined intervals $\mu_1,\ldots,\mu_i$. Let $v_{i+1}$ be the vertex lying immediately to the right of the right endpoint of $\mu_i$. We then set $\mu_{i+1}=I(v_{i+1})$. Notice that from Observation~\ref{obs: length of int}, for each $i$, $16d\leq |\mset'(\mu_i)|\leq 20d$. Since $z=\ceil{\frac{|\mset'|}{160d}}-1$, all intervals $\mu_1,\ldots,\mu_{2z+2}$ are well-defined.
  For convenience, we denote, for each $1\leq i\leq 2z$, $\mset'(\mu_i)$ by $\mset_i$.
For every vertex $t\in T(\mset')$, let $Q_t$ be the shortest path connecting $t$ to $\tilde t$ in $G$, so $Q_t$ is contained in the column of $G$ which contains $t$. %For each $1\leq i\leq 2z$, let $\mset_i\subseteq \mset'$ be the set of all demand pairs $(s,t)$ for which $\tilde t\in \mu_i$, so that $|\mset_i|=16d$. %We say that the demand pairs in $\mset_i$ \emph{belong to the interval $\mu_i$}. 
We also let  $U(\mu_i)=\bigcup_{(s,t)\in \mset_i}V(Q_t)$. %: the set of all vertices appearing on the paths $Q_t$ whose corresponding demand pair $(s,t)$ belongs to $\mu_i$.
   
For all $1\leq i,j\leq 2z$, we say that intervals $\mu_i$ and $\mu_j$ are \emph{neighbors} iff $|i-j|\leq 1$. 
Consider now some interval $\mu_i$, with $1\leq i\leq 2z$ and some demand pair $(s,t)\in \mset_i$. We say that $(s,t)$ is a \emph{bad demand pair} iff path $P(s,t)$ contains a vertex of $U(\mu_j)$ for some interval $\mu_j$ that is not a neighbor of $\mu_i$. Otherwise, we say that $(s,t)$ is a \emph{good demand pair}.

\begin{claim}\label{claim: bound bad pairs}
For each $1\leq i\leq 2z$, at most $8d$ demand pairs of $\mset_i$ are bad.
\end{claim}

We prove the claim below, after we complete the proof of Theorem~\ref{thm: partition into intervals} using it. Note that at most one interval $\mu_j$ may contain more than $\sqrt{n}/2$ vertices; we assume without loss of generality that, if such an interval $\mu_j$ exists, then $j$ is an odd integer.
The set $\Sigma'=\set{\sigma'_1,\ldots,\sigma'_z}$ of intervals of $\pi'$ is defined as follows: for each $1\leq i\leq z$, we let $\sigma'_i=\mu_{2i}$. Notice that every pair of such intervals is separated by at least $16d$ vertices, since each odd-indexed interval $\mu_j$ must contain at least $16d$ vertices by definition. Since we discard the first and the last intervals $\mu_j$, the distance from each resulting interval $\sigma'_i$ to interval $\pi$, and to each of the remaining three boundaries of $G$ is also at least $16d$.

In order to define the set $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of intervals, fix some $1\leq i\leq z$. Let $\mset_{i}'\subseteq \mset_{2i}$ be the set of all good demand pairs in $\mset_{2i}$. We let $\sigma_i$ be the smallest sub-interval of $\pi$, containing all vertices of $S(\mset'_{i})$. 

It is immediate to verify that, for each $1\leq i\leq z$, the value of the optimal solution of the \NDP instance $(G,\mset'_{\sigma_i,\sigma'_i})$ is at least $d$, since we can route all demand pairs of $\mset'_i$ in $G$. From our construction, every interval $\sigma'_i\in \Sigma'$ contains at least $16d$ and at most $\sqrt{n}/2$ vertices, and it is separated by at least $16d$ vertices from all other intervals in $\Sigma\cup \Sigma'$,  and from each of the remaining three boundaries of $G$.  It remains to show that the intervals in $\Sigma$ are all disjoint, and that $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order. 

Fix some pair of indices $1\leq i<j\leq z$. If we traverse $\Gamma$ in counter-clock-wise order, starting from the first vertex of $\sigma'_1$, then we will first encounter all vertices of $\sigma_i'$, then all vertices of $\sigma_j'$, and finally all vertices of $\sigma_i\cup \sigma_j$. It is enough to show that we will encounter every vertex of $\sigma_j$ before we encounter any vertex of $\sigma_i$. In particular, it is enough to show that for every pair $(s,t)\in \mset'_j$ and $(s',t')\in \mset'_i$ of demand pairs, we will encounter $s$ before $s'$ in our traversal. 

Assume for contradiction that this is false for some  $(s,t)\in \mset'_j$ and $(s',t')\in \mset'_i$. Then $\tilde{t}',\tilde{t},s',s$ appear on $\Gamma$ in this circular order  (see Figure~\ref{fig: good pairs routing}). Since both demand pairs $(s,t)$ and $(s',t')$ are good, path $P(s,t)$ may not contain a vertex of $Q_{t'}$, and path $P(s',t')$ may not contain a vertex of $Q_t$ (see Figure~\ref{fig: good pairs routing}). But then the union of the path $P(s',t')$ and $Q_{t'}$ separates $s$ from $t$ in $G$, a contradiction. It now remains to prove Claim~\ref{claim: bound bad pairs}.

\begin{figure}[h]
\scalebox{0.5}{\includegraphics{good-pairs-routing}}
\caption{Ordering of the terminals of good demand pairs.\label{fig: good pairs routing}}
\end{figure}

\begin{proofof}{Claim~\ref{claim: bound bad pairs}}
Fix some index $1\leq i\leq 2z$, and let $\nset$ be the set of all bad demand pairs in $\mset_i$. We further partition $\nset$ into two subsets: set $\nset'$ contains all demand pairs $(s,t)$ whose corresponding path $P(s,t)$ contains a vertex in some set $U(\mu_j)$ for $j>i+1$, and set $\nset''$ containing all remaining demand pairs (for each such demand pair $(s,t)$, the corresponding path $P(s,t)$ must contain a vertex in some set $U(\mu_j)$, for some $j<i-1$). It is enough to show that $|\nset'|,|\nset''|\leq 4d$. We show that $|\nset'|\leq 4d$; the bound for $\nset''$ is proved similarly. 
Given a pair $(s,t)\in \nset'$, and a pair $(\hat s,\hat t) \in \mset_{i+1}$, we say that there is a \emph{conflict} between $(s,t)$ and $(\hat s,\hat t)$ iff $P(s,t)$ contains a vertex of $Q_{\hat t}$.

We need the following simple observation.

\begin{observation}\label{obs: containing many U-vertices}
Let $(s,t)$ be any demand pair in $\nset'$. Then there are at least $12d$ demand pairs $(\hat s,\hat t)\in \mset_{i+1}$, such that there is a conflict between $(s,t)$ and $(\hat s,\hat t)$.
\end{observation}

Assume first that the observation is correct, and assume for contradiction that $|\nset'|>4d$. Then there are at least $48d^2$ pairs $((s,t),(\hat s,\hat t))$ with $(s,t)\in \nset'$ and 
$(\hat s,\hat t)\in \mset_{i+1}$, such that there is a conflict between $(s,t)$ and $(\hat s,\hat t)$. However, $|\mset_{i+1}|\leq 20d$, and, since, for each pair $(\hat s,\hat t)\in \mset_{i+1}$, $Q_{\hat t}$ contains at most $2d$ vertices, there may be at most $2d$ pairs $(s,t)\in \nset'$ that conflict with $(\hat s,\hat t)$, a contradiction. We now proceed to prove the observation.


%Notice that if the observation is correct, then, since $|U(\mu_{i+1})|\leq |\mset_{i+1}|\cdot (2d)\leq 40d$, and all paths in $\pset^*$ are node-disjoint, we get that $|\nset'|\leq 4d$ as required. We now proceed to prove the observation.

Let $v$ be some vertex on path $P(s,t)$, that belongs to a set $U(\mu_j)$, for some $j>i+1$. Then $v$ lies on some path $Q_{t'}$, for some $t'\in T(\mset_j)$ (see Figure~\ref{fig: obs-proof1}). We construct a (not necessarily simple) curve $\gamma$, by concatenating the path $Q_t$; the sub-path of $\pi'$ between $\tilde t$ and $\tilde{t}'$; the sub-path of $Q_{t'}$ between $\tilde t'$ and $v$; and the sub-path of $P(s,t)$ between $v$ and $t$ (see Figure~\ref{fig: obs-proof2}). Consider now some demand pair $(\hat s,\hat t)\in \mset_{i+1}$. If path $P(s,t)$ does not contain a vertex of $Q_{\hat t}$, then curve $\gamma$ separates $\hat t$ from $\hat s$, and so path $P(\hat s,\hat t)$ has to cross the curve $\gamma$. This is only possible if path $P(\hat s,\hat t)$ contains a vertex of $Q_t\cup Q_{t'}$. But since both $Q_t$ and $Q_{t'}$ contain at most $2d$ vertices each, at most $4d$ paths of $\pset^*$ may intersect the curve $\gamma$. Therefore, there are at least $16d-4d= 12 d$ demand pairs in $\mset_{i+1}$, whose corresponding path in $\pset^*$ does not intersect the curve $\gamma$. From the above discussion, for each such pair $(\hat s,\hat t)$, path $P(s,t)$ must contain a vertex of $Q_{\hat t}$, and so $(s,t)$ conflicts with $(\hat s,\hat t)$.  We conclude that $(s,t)$ conflicts with at least  $12d$ pairs of $\mset_{i+1}$.



\begin{figure}[h]
\scalebox{0.4}{\includegraphics{obs-proof1}}
\caption{Illustration to the proof of Observation~\ref{obs: containing many U-vertices}. Demand pairs $(s,t)$ and $(\hat s,\hat t)$. Path $P(s,t)$ is shown in red.\label{fig: obs-proof1}}
\end{figure}

\begin{figure}[h]
\scalebox{0.4}{\includegraphics{obs-proof2}}
\caption{Illustration to the proof of Observation~\ref{obs: containing many U-vertices}. The curve $\gamma$ is shown in brown. 
\label{fig: obs-proof2}}
%\hspace{1cm}
%\subfigure[caption subfigure 3]{\scalebox{0.2}{\includegraphics{file3.pdf}}\label{fig: label3}}
%\caption{Illustration to the proof of Observation~\ref{obs: containing many U-vertices} \label{fig: obs-proof}}
\end{figure}



\iffalse
\begin{figure}[h]
\centering
\subfigure[Demand pairs $(s,t)$ and $(\hat s,\hat t)$. Path $P(s,t)$ is shown in red.]{\scalebox{0.4}{\includegraphics{obs-proof1}}\label{fig: obs-proof1}}
\hspace{1cm}
\subfigure[The curve $\gamma$ is shown in brown]{
\scalebox{0.4}{\includegraphics{obs-proof2}}\label{fig: obs-proof2}}
%\hspace{1cm}
%\subfigure[caption subfigure 3]{\scalebox{0.2}{\includegraphics{file3.pdf}}\label{fig: label3}}
\caption{Illustration to the proof of Observation~\ref{obs: containing many U-vertices} \label{fig: obs-proof}}
\end{figure}
\fi


\end{proofof}
\end{proofof}



\iffalse

\paragraph{Special Sub-Instances.}

The following observation is immediate:
\begin{observation}\label{obs: partitioning intervals valid instance}
Let $\pi,\pi'$ be two disjoint sub-paths of $\Gamma$, each of which is contained in a single boundary edge of $G$. Let $d>0$ be an integer, and let $\mset'\subseteq \mset_{\pi,\pi'}$ be any subset of at least $128d$ demand pairs that can be routed in $G$ via node-disjoint path. Assume further that for each $t\in T(\mset')$, $d\leq d(t,\tilde t)\leq 2d$. Consider the sequences $\Sigma=(\sigma_1,\ldots,\sigma_z),\Sigma'=(\sigma_1',\ldots,\sigma_z')$ of intervals computed by Theorem~\ref{thm: partition into intervals} on input $\pi,\pi',\mset'$ and $d$. Then for each $1\leq i\leq z$, instance $(G,\mset'_{\sigma_i,\sigma_i'})$ is a valid $(\sigma_i,\sigma_i',d)$-instance.
\end{observation}

The main idea of the algorithm is to compute a partition of the demand pairs into sets $\mset'_{\sigma_i,\sigma_i'}$ with properties similar to those  given by Theorem~\ref{thm: partition into intervals}, and then solve the problem separately for each one of the subsets $\mset'_{\sigma_i,\sigma_i'}$ of demand pairs on a carefully selected sub-graph $G_i$ of $G$. The subgraph $G_i$ will be selected in such a way that the destinations of the demand pairs in $\mset'_{\sigma_i,\sigma_i'}$  will lie at a distance at least $d$ from the boundary of the resulting grid, and we will only attempt to route at most $d$ demand pairs in it. We will then be able to employ Theorem~\ref{thm: main w destinations far from boundary}  to approximately solve each such resulting instance. We now define the modified instances, to which Theorem~\ref{thm: main w destinations far from boundary}  will eventually be applied.



Assume that we are given two disjoint sub-paths $I,I'\subseteq\Gamma$, an integer $d>0$, and a valid $(I,I',d)$-sub-instance $(G,\mset')$ of $(G,\mset)$. We define a corresponding \emph{modified instance} $(G',\mset'')$. The underlying graph $G'$ will be an appropriately chosen sub-grid of $G$, and each demand pair in the new set $\mset''$ will correspond to a unique demand pair in $\mset'$.

In order to define the grid $G'$, we assume without loss of generality that $I'$ is a sub-path of the bottom boundary edge of the grid. Let $\wset''$ be the subset of the columns of $G$ that intersect $I'$, and let $\rset''$ be the set of $4d$ bottommost rows of $G$. Let $G''\subseteq G$ be the sub-grid of $G$ spanned by the set $\wset''$ of columns and the set $\rset''$ of rows. In order to obtain the final graph $G'$, we add to $\wset''$ $4d$ columns lying immediately to its left and $4d$ consecutive columns lying immediately to its right, denoting the resulting set of columns by $\wset'$. We also add to $\rset''$ a set of $|\wset'|-4d$ rows lying immediately above $\rset''$, obtaining a set $\rset'$ of rows of $G$. Graph $G'$ is the sub-grid of $G$ spanned by the columns of $\wset'$ and the rows of $\rset'$. Notice that $G'$ is a square grid.

The set $\mset''$ of demand pairs is constructed as follows. For each demand pair $(s,t)\in \mset'$, we add a demand pair $(s',t')$ to $\mset''$. Vertex $t'$ is mapped to the same location as vertex $t$ in $G'$. Vertex $s'$ is mapped to one of the vertices on the top row of $G'$, using the following procedure. Let $X$ denote the set of $|S(\mset')|$ leftmost vertices on the top row of $G'$. Let $v$ be the bottom left corner of the grid $G'$. The traversal of $\Gamma(G)$ in the clock-wise direction, starting from $v$, defines an ordering $\pi$ of the vertices in $S(\mset')$. Similarly, a traversal of $\Gamma(G')$ in the clock-wise direction, starting from $v$, defines an ordering $\pi'$ of the vertices in $X$. Consider some vertex $s\in S(\mset')$, and assume that it is the $i$th vertex of $S(\mset')$ according to the ordering $\pi$. We map it to the $i$th vertex of $X$, according to the ordering $\pi'$.
This finishes the definition of the modified instance $(G',\mset'')$ corresponding to the valid $(I,I',d)$ sub-instance $(G,\mset')$ of $(G,\mset)$. We need the following simple claim, whose proof is straightforward and deferred to the Appendix.

\begin{claim}\label{claim: modified instance preserves solutions}
Let $I,I'\subseteq \Gamma$ be two disjoint intervals of $\Gamma$, $d>0$ an integer, and let $(G,\mset')$ be a valid $(I,I',d)$ sub-instance of $(G,\mset)$. Let $\opt'$ be the value of the optimal solution to instance $(G,\mset')$. Then the value of the optimal solution to the corresponding modified instance $(G',\mset'')$ is at least $\min\set{\opt',d}$.
\end{claim}



Let $I,I'\subseteq \Gamma$ be two disjoint intervals of $\Gamma$, let $d>0$ be an integer, and let $(G,\mset')$ be a valid $(I,I',d)$ sub-instance of $(G,\mset)$. Let $\opt'$ be the value of the optimal solution to this instance.
Consider the corresponding modified instance $(G',\mset'')$ of $(G,\mset')$. Then $(G',\mset'')$, together with the parameter $\opt=d$ is a valid input to Theorem~\ref{thm: main w destinations far from boundary}. We can then use the algorithm from Theorem~\ref{thm: main w destinations far from boundary} to compute, with high probability, a solution to instance $(G',\mset'')$, whose value is $\frac{\min\set{d,\opt'}}{2^{O(\sqrt{\log n}\log\log n)}}$. We let $\aset(G',\mset'')$ denote the resulting solution, and we let $|\aset(G',\mset'')|$ denote its value.



Combining Theorem~\ref{thm: partition into intervals} with Claim~\ref{claim: modified instance preserves solutions}, we obtain the following corollary.

\begin{corollary}\label{cor: interval partitioning with solution}
Suppose we are given two disjoint intervals $\pi,\pi'$ of $\Gamma$, each of which is contained in a single boundary edge of $G$, and a subset $\mset'\subseteq \mset_{\pi,\pi'}$ of demand pairs, together with an integer $d\geq 1$, such that $|\mset'|\geq 128d$, all demand pairs in $\mset'$ can be routed via node-disjoint paths in $G$, and  for each pair $(s,t)\in \mset'$, $d\leq d(t,\tilde t)<2d$. Let $z=\ceil{\frac{|\mset'|}{64d}}-1$. Then there is a collection $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of disjoint sub-intervals of $\pi$, and a collection $\Sigma'=\set{\sigma_1',\ldots,\sigma'_z}$ of disjoint sub-intervals of $\pi'$, such that:

 \begin{itemize}
 \item the intervals $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order;
 
 
  \item for every pair of intervals $\sigma\in \Sigma\cup \Sigma'$  and $\sigma'\in \Sigma'$, at least $16d$ vertices of $\Gamma$ separate the two intervals; 
  
  \item every interval $\sigma'\in \Sigma'$ has length at most $\sqrt{n}/2$; and
 
 
  \item for each $1\leq i\leq z$, $(G,\mset'_{\sigma_i,\sigma'_i})$ is a valid $(\sigma_i,\sigma'_i,d)$-instance. Moreover, if we denote by $(G_i,\mset''_i)$ the corresponding modified instance, then $|\aset(G_i,\mset''_i)|\geq d/2^{O(\sqrt{\log n}\log\log n)}$, and in particular,
   $\sum_{i=1}^z|\aset(G_i,\mset''_i)|\geq |\mset'|/2^{O(\sqrt{\log n}\log\log n)}$.
  \end{itemize}
  \end{corollary}

\fi



\subsection{The Algorithm} \label{subsec: general case algo}
If all vertices of $T(\mset)$ lie on the boundary $\Gamma$ of $G$, then we can solve the problem efficiently using standard dynamic programming. Therefore, we assume from now on, that for each $t\in T(\mset)$, $d(t,\tilde t)\geq 1$.

Recall that $\Gamma_1,\ldots,\Gamma_4$ denote the four boundary edges of $G$.
We partition the set $\mset$ of demand pairs into $16$ subsets $\mset_{q,q'}$, for $1\leq q,q'\leq 4$: demand pair $(s,t)$ belongs to set $\mset_{q,q'}$ iff $s\in \Gamma_q$ and $\tilde t\in \Gamma_{q'}$. We then solve each of the resulting instances $(G,\mset_{q,q'})$ separately, and return the best of the resulting solutions. Since one of these instances is guaranteed to have a solution of value at least $\opt/16$, it is enough to show a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximation algorithm for each such instance separately.
 Therefore, from now on we focus on one such instance $(G,\mset_{q,q'})$, and we assume w.l.o.g. that the value of the optimal solution in this instance is at least $\opt/16$.
 
 
 We further partition the set $\mset_{q,q'}$ of demand pairs into the following subsets: we let $\mset^0_{q,q'}$ contain all demand pairs $(s,t)$ with $d(t,\tilde t)\geq \opt/\eta$, and for $0<r<\log n$, we let $\mset^r_{q,q'}$ contain all demand pairs $(s,t)$ with $\frac{\opt}{\eta\cdot 2^r} \leq d(t,\tilde t)<\frac{\opt}{\eta\cdot 2^{r-1}}$. Clearly, there is an index $0< r^*< \log n$, for which the value of the optimal solution of instance $(G,\mset^{r^*}_{q,q'})$ is at least $\Omega(\opt/\log n)$. Therefore, it is enough to compute a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximation for each such instance separately. Notice that we can compute a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximate solution for instance $\mset^0_{q,q'}$ using Theorem~\ref{thm: main w destinations far from boundary}. Therefore, we now focus on an instance $(G,\mset^{r^*}_{q,q'})$, for some fixed $r^*>0$. 
 
 In order to simplify the notation, we denote by $\mset$ the corresponding set $\mset^{r^*}_{q,q'}$ of demand pairs; we assume that we are given an integer $1\leq d\leq \opt/2\eta$, such that all destination vertices $t\in T(\mset)$ have $d\leq d(t,\tilde{t})< 2d$. We denote by $\opt'$ the value of the optimal solution of the resulting instance $(G,\mset)$, and we assume that $\Theta(\opt/\log n)\leq \opt'\leq \opt$. Moreover, we can assume that $\opt'>2^{13}d$, since otherwise we can directly apply Theorem~\ref{thm: main w destinations far from boundary} to instance $(G,\mset)$ with parameter $\opt=d$ to obtain an $2^{O(\sqrt{\log n}\log\log n)}$-approximation.  We now consider three cases, depending on the location of the boundary edges $\Gamma_q$ and $\Gamma_{q'}$.
 
 
  
 \paragraph*{Case 1: $\Gamma_q$ and $\Gamma_{q'}$ are opposite boundary edges.} Without loss of generality, we assume that $\Gamma_q$ is the top row of the grid $G$, and it contains the vertices of $S(\mset)$, while $\Gamma_{q'}$ is the bottom row of the grid, and it contains the vertices $\set{\tilde t\mid t\in T(\mset)}$.
 
Let $\mset'\subseteq \mset$ be the set of the demand pairs routed by the optimal solution. 
 Let $I$ denote the top boundary of the grid $G$, and let $I'$ denote its bottom boundary.
Theorem~\ref{thm: partition into intervals} guarantees the existence of a set  $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of disjoint sub-intervals of $I$, and a set $\Sigma'=\set{\sigma_1',\ldots,\sigma'_z}$ of disjoint sub-intervals of $I'$, for $z=\ceil{\frac{|\mset'|}{160d}}-1$, such that the intervals $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order;
  every pair $\sigma\in \Sigma\cup \Sigma'$, $\sigma'\in \Sigma'$ of  intervals is separated by at least $16d$ vertices of $\Gamma$; the length of each interval $\sigma'\in \Sigma'$ is at least $16d$ and at most $\sqrt{n}/2$, and for each $1\leq i\leq z$, if we consider the perfect $(\sigma_i,\sigma'_i,d)$-instance $(G,\tmset_i)$, where $\tmset_i=\mset_{\sigma_i,\sigma_{i'}}$, and denote by $(G_i,\tmset'_i)$ the corresponding modified instance, then $|\aset(G_i,\tmset'_i)|\geq d/2^{O(\sqrt{\log n}\log\log n)}$. Moreover, for every $1\leq i\leq z$, $(\sigma_i,\sigma_i')$ is a $d$-interesting pair of intervals. Notice, however, that, since the set $\mset'$ of demand pairs routed by the optimal solution is not known to us, we cannot compute the sets $\Sigma$ and $\Sigma'$ of intervals directly. We now show how to overcome this difficulty.
  
For every $d$-interesting pair $(\sigma,\sigma')$ of intervals, with $\sigma\subseteq I$, $\sigma'\subseteq I'$, consider the perfect $(\sigma,\sigma',d)$-instance $(G, \mset_{\sigma,\sigma'})$, and the corresponding modified instance $(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})$. We can then compute an approximate solution $
\aset(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})$ of value $|\aset(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})|$ to this instance, using the algorithm from Theorem~\ref{thm: main w destinations far from boundary}, together with the parameter $\opt=d$. 
We can assume w.l.o.g. that, if $\mset'_{\sigma,\sigma'}\neq\emptyset$, then $|\aset(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})|\geq 1$. Let $c$ be a constant, so that the approximation factor of Algorithm $\aset$ given in Theorem~\ref{thm: main w destinations far from boundary} is $2^{c\sqrt{\log n}\log\log n}$.
Assume now that we have computed the values  $|\aset(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})|$  for all $d$-interesting pairs $\sigma\subseteq I$ and $\sigma'\subseteq I'$ of intervals.
We say that a pair $(\sigma,\sigma')$ of interesting intervals is a \emph{good pair} iff $ |\aset(G'_{\sigma,\sigma'},\mset'_{\sigma,\sigma'})|\geq \ceil{d/2^{c \sqrt{\log n}\log\log n}}$.
It is now enough to compute a collection $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of disjoint sub-intervals of $I$, and a collection $\Sigma'=\set{\sigma_1',\ldots,\sigma'_z}$ of disjoint sub-intervals of $I'$, for $z=\ceil{\frac{|\mset'|}{160d}}-1$, such that the intervals $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order; for all $i$, $(\sigma_i,\sigma_i')$ is a good pair of intervals, and $\sigma_i'$ is at a distance at least $16d$ from every interval in $\Sigma\cup \Sigma'$. This can be done by using simple dynamic programming.


Assume now that we have computed the collections $\Sigma$ and $\Sigma'$ of intervals as above. For each $1\leq i\leq z$, let $\pset_i=\aset(G'_{\sigma_i,\sigma'_i},\mset'_{\sigma_i,\sigma'_i})$ be the set of paths routed by the solution of value $|\aset(G'_{\sigma_i,\sigma'_i},\mset'_{\sigma_i,\sigma'_i})|$ that we have computed. Let $\nset'_i\subseteq \mset'(\sigma_i,\sigma'_i)$ be the set of the demand pairs routed by this solution, and let $\nset_i\subseteq \mset(\sigma_i,\sigma'_i)$ be the set of the original demand pairs corresponding to the pairs in $\nset'_i$. For convenience, we denote $G_i=G'_{\sigma_i,\sigma'_i}$. Finally, let $\tilde{\nset}_i$ denote the set of pairs $(s,s')$, where $(s,t)\in \nset_i$, and $(s',t')\in \nset'_i$ is the corresponding demand pair in the modified instance. 

From the above discussion, $\sum_{i=1}^z|\nset_i|\geq \opt'/\approxfactor$.
It is now enough to show that all demand pairs in set $\bigcup_{i=1}^z\nset_i$ can be routed in $G$. In order to do so, it is enough to show that all pairs in $\bigcup_{i=1}^z\tilde{\nset}_i$ can be routed in graph $G$ via paths that are internally disjoint from $\bigcup_{i=1}^zG_i$, as we can exploit the paths in $\bigcup_{i=1}^z\pset_i$ in order to complete the routing. Recall that the graphs $G_i$ are disjoint from the top $\sqrt{n}/4$ rows of the grid, and the source vertices of the demand pairs in  $\bigcup_{i=1}^z\tilde{\nset}_i$ appear in the same left-to-right order as their destination vertices. It is now immediate to complete the routing of the demand pairs in $\bigcup_{i=1}^z\tilde{\nset}_i$.

\paragraph*{Case 2: $\Gamma_q$ and $\Gamma_{q'}$ are neighboring boundary edges.}
Assume w.l.o.g. that $\Gamma_q$ is the left boundary edge of $G$ and $\Gamma_{q'}$ is its bottom boundary edge. This case is dealt with very similarly to Case 1, with minor changes.
As before, we assume that we are given a set $\mset$ of demand pairs and an integer $d$, such that for each pair $(s,t)\in \mset$, $s\in \Gamma_q$, $\tilde t\in \Gamma_{q'}$, and $d\leq d(t,\tilde t)<2d$. We assume that we know the value $\opt'$ of the optimal solution to instance $(G,\mset)$, and we assume w.l.o.g. that $\opt'\geq 2^{13}d$. 
 We let $I$ be the left boundary edge of $G$, and we let $I'$ be the bottom boundary edge of $G$, excluding its $\ceil{\opt'/16}$ leftmost vertices. 
 Let $\mset'\subseteq \mset$ be the subset of all demand pairs $(s,t)$ with $\tilde{t}\in I'$. Let $\opt''$ be the value of the optimal solution to instance $(G,\mset')$.
 
 \begin{observation}
 $\opt''\geq \opt'/2$.
 \end{observation}
 
 \begin{proof}
 Let $\pset^*$ be the optimal solution to instance $(G,\mset)$, and let $\mset^*$ be the set of the demand pairs routed by it. Let $\hmset=\mset^*\setminus \mset'$. Then it is enough to show that $|\hmset|\leq \opt'/2$. Let $R''$ be the bottom row of $G$, and let $I''=R''\setminus I'$. Then for each demand pair $(s,t)\in \hmset$, $\tilde t\in I''$ must hold. Let $Q$ be a sub-grid of $G$, whose bottom boundary is $I''$, and whose height is $\ceil{\opt'/16}>2d$. Then the boundary of $Q$ has length at most $\opt'/4+4$, and every path routing a demand pair in $\hmset$ must cross the boundary of $Q$. Therefore, $|\hmset|\leq \opt'/2$.
 \end{proof}  
 
 The remainder of the algorithm is exactly the same as in Case 2. The only difference is in how the demand pairs in set $\tilde \nset=\bigcup_{i=1}^z\tilde{\nset}_i$ are routed. This is done by utilizing the $\opt'/16$ first columns of $G$ and the $\opt'/2$ top rows of $G$. Since we can assume that $|\tilde \nset|<\opt'/64$,  it is straightforward to find a suitable routing.

%------------------------------------------------------
%------------------------------------------------------
%------------------------------------------------------
\paragraph*{Case 3: $\Gamma_q=\Gamma_{q'}$.}
%------------------------------------------------------
%------------------------------------------------------
We assume w.l.o.g. that $\Gamma_q$ is the bottom boundary of $G$. 
We assume that we are given a set $\mset$ of demand pairs and an integer $d$, such that for each pair $(s,t)\in \mset$, $s,\tilde t\in \Gamma_q$, and $d\leq d(t,\tilde t)<2d$. We assume that we know the value $\opt'$ of the optimal solution to instance $(G,\mset)$, and we assume w.l.o.g. that $\opt'\geq 2^{13}d$. 


We partition the set $\mset$ of the demand pairs into three subsets: set $\mset^0$ contains all pairs $(s,t)$ with $|\col(s)-\col(t)|\leq 2d$; set $\mset^1$ contains all remaining pairs $(s,t)$ with $\col(s)<\col(t)$; and set $\mset^2$ contains all remaining demand pairs. 
We deal with the demand pairs in $\mset^0$ using the following claim.

\begin{claim}\label{claim: short pairs}
There is an efficient randomized algorithm that computes a factor-$2^{O(\sqrt{\log n}\log\log n)}$ approximation to instance $(G,\mset^0)$ of \NDP.
\end{claim}

\begin{proof}
Let $\rho$ be a random integer between $0$ and $4d$. We define a collection $\qset'=\set{Q_1,\ldots,Q_r}$ of square sub-grids of $G$ as follows. Let $Q_1$ be a sub-grid of size $((4d+\rho)\times (4d+\rho))$, containing the bottom left corner of $G$ as the bottom left corner of $Q_1$. Assume now that we have defined $Q_1,\ldots,Q_i$. Let $N$ be the number of columns of $G$ that do not intersect the grids of $Q_1,\ldots,Q_i$. If $N>8d$, then we let $Q_{i+1}$ be the $(4d\times 4d)$ sub-grid of $G$, whose bottom left corner is the vertex serving as the bottom right corner of $Q_i$. Otherwise, we set $r=i+1$, and we let $Q_r$ be the square grid whose bottom left corner is the  vertex serving as the bottom right corner of $Q_i$, and whose bottom right corner is the bottom right corner of the grid $G$. Notice that each grid $Q_i$ has width and height $4d$, except for $Q_1$ and $Q_r$, whose widths and heights may be between $4d$ and $8d$.

For $1\leq i\leq r$, let $\nset_i\subseteq \mset^0$ be the set of all demand pairs $(s,t)$ with $s,t\in V(Q_i)$. Let $\nset=\bigcup_{i=1}^r\nset_i$. Notice that each demand pair $(s,t)\in \mset^0$ belongs to $\nset$ with constant probability, and therefore, with high probability, $\opt(G,\nset)=\Omega(\opt(G,\mset^0))$.

We partition the set $\qset'$ of the squares into four subsets, $\qset^1,\ldots,\qset^4$, where for $1\leq i\leq 4$, $\qset^i$ contains all squares $Q_j$, where $j=i\mod 4$.
For $1\leq i\leq 4$, let $\nset^i\subseteq \nset$ be the subset of all demand pairs $(s,t)$, such that for some $Q\in \qset^i$, $s,t\in V(Q)$. We solve each problem $(G,\nset^i)$ separately and return the best of the resulting four solutions.

We now fix $1\leq i\leq 4$, and solve the problem $(G,\nset^i)$. Consider some square $Q_j\in \qset^i$. Let $Q^+_j$ be obtained by adding a margin of $4d$ columns to the left and to the right of $Q_j$, and $8d$ rows above $Q_j$ (if $j=1$ or $j=r$, then we do not add columns on one of the sides of $Q_j$, and we add only $4d$ rows above $Q_j$, so that $Q_j^+$ is a square grid). Notice that from our construction, if $Q_j,Q_{j'}\in \qset^i$, then $Q^+_j,Q^+_{j'}$ are disjoint. Using the same reasoning as in the proof of Claim~\ref{claim: modified instance preserves solutions}, $\opt(Q^+_j,\nset_j)\geq \opt(G,\nset_j)$. Notice that $\opt(G,\nset_j)\leq 4d$, as all source vertices of the demand pairs routed by the optimal solution must be distinct, and they lie on the bottom boundary of $Q_j$. It is then easy to see that $(Q^+,\nset_j)$ is a special case of \restrictedNDP where all destination vertices lie at a distance at least $\opt/4$ from the grid boundary, and we can find a $2^{O(\sqrt{\log n}\log\log n)}$-approximation for it using Theorem~\ref{thm: main w destinations far from boundary}.
\end{proof}


\iffalse
We say that a demand pair $(s,t)\in \mset^0$ survives iff both $s$ and $t$ belong to some squarey 

Let $\mset^*$ be the set of the demand pairs routed by the optimal solution to instance $(G,\mset^0)$. Notice that all demand pairs in $\mset^*$ have distinct source vertices. Therefore, if we denote $S=S(\mset^0)=\set{s_1,\ldots,s_z}$, where all vertices in $S$ are distinct, then $|\mset^*|\leq |S|$. We show an efficient algorithm to route $|S|/130$ demand pairs of $\mset^0$, thus obtaining a factor-$130$ approximation. Assume that the vertices of $S$ are indexed according to their left-to-right order on the bottom boundary of $G$. Let $S'=\set{s_i\mid i=1\mod 130}$. Let $\mset'\subseteq \mset^0$ contain one demand pair $(s_i,t_i)$ for every source vertex $s_i\in S'$; if several such pairs exist, we choose one of them arbitrarily. Let $H_i$ be the sub-grid of $G$, whose left and right boundaries are $\col(s_i)$ and $\col(t_i)$, and whose top and bottom boundaries coincide with the top and the bottom boundaries of $G$. Then all graphs $H_i$ are disjoint from each other, and each such graph $H_i$ contains $s_i$ and $t_i$. We can now route each pair $(s_i,t_i)\in \mset'$ inside the corresponding grid $H_i$.
\end{proof}
\fi

%We solve each one of the three resulting subinstances $(G,\mset^0)$, $(G,\mset^1)$, and $(G,\mset^2)$ separately. 
If the optimal solution value to instance $(G,\mset^0)$ is at least $\opt'/3$, then we obtain a $2^{O(\sqrt{\log n}\log\log n)}$-approximation to this instance, and a $\approxfactor$-approximation overall, using Claim~\ref{claim: short pairs}. Therefore, we assume from now on that any optimal solution must route at least $2\opt'/3$ demand pairs from $\mset^1\cup \mset^2$.
We compute an approximate solution to each of the problems $(G,\mset^1)$ and $(G,\mset^2)$ separately, and take the better of the two solutions. Clearly, it is enough to design a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximation to each of these two problems separately. We now focus on one of these problem, say $(G,\mset^1)$, and for simplicity denote $\mset^1$ by $\mset$ and the value of the optimal solution to instance $(G,\mset^1)$ by $\opt'$.

Recall that $\ell=\sqrt{n}$ is the length of the grid $G$. We can naturally associate with each demand pair $(s,t)\in \mset$ an interval $I(s,t)\subseteq [\ell]$: the left endpoint of $I(s,t)$ is the index of $\col(s)$, and its right endpoint is the index of $\col(t)$.

Next, we partition the demand pairs in $\mset$ into $h=\log n$ classes $\mset_1,\mset_2,\ldots, \mset_h$, as follows. Pair $(s,t)$ belongs to class $\mset_i$ iff $2^{i-1}\leq |I(s,t)|<2^i$. Note that for $i\leq \log d$, $\mset_i=\emptyset$, as all such pairs belong to $\mset^0$. Thus, we obtain a collection of $h$ instances $(G,\mset_i)$ of the problem. As before, we will compute a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximation to each of these instances separately, and return the best of the resulting solutions. We now fix some index $\log d\leq i\leq h$, and design a factor-$2^{O(\sqrt{\log n}\log\log n)}$-approximation algorithm to the corresponding instance $(G,\mset_i)$. 

%We need to consider two subcases. The first subcase happens when $2^i\geq 512d$, and the second subcase happens when $2^i< 512d$.

%(
Let $\rho$ be an integer chosen uniformly at random from $[0,2^{i+3})$. Let $Z$ be the set of all integers $1\leq z\leq \ell$, such that $z=\rho+j\cdot 2^{i+3}$ for some integer $j$.
 Let $\mset'\subseteq \mset$ contain all demand pairs $(s,t)$, such that there is some number $z\in Z$ with $\col(s)<z<\col(t)$, and for all $z'\in Z$, $|\col(s)-z'|,|\col(t)-z'|\geq 2^{i-1}/4$. Let $I(s,t)$ be an interval whose left endpoint is $\col(s)$ and right endpoint is $\col(t)$, and let $I'(s,t)\subseteq I(s,t)$ be its sub-interval that excludes the first and the last $2^{i-1}/4$ vertices of $I(s,t)$. Then it is easy to see that $(s,t)\in \mset'$ iff some integer in $I'(s,t)$ belongs to $Z$, and that this happens with probability at least $1/32$ over the choice of $\rho$. We now focus on solving the instance $(G,\mset')$ of the problem, and we denote by $\opt''$ the value of its optimal solution, so $\expect{\opt''}=\Omega(\opt')$. %]

Let $Z'$ contain all integers that lie halfway between consecutive pairs of integers of $Z$, that is: $Z'=\set{z+2^{i+2}\mid z\in Z \mbox{ and } z+2^{i+2}\leq \ell}$. We partition the grid $G$ into sub-grids $H_1,\ldots, H_r$, by deleting all columns $W_z$, where $z\in Z'$. 
Then for every demand pair $(s,t)\in \mset'$, there is a unique sub-grid $H_j$ containing both $s$ and $t$. For each $1\leq j\leq r$, let $\hmset_j\subseteq \mset'$ be the set of all demand pairs $(s,t)$ with both $s$ and $t$ contained in $H_j$. For each $1\leq j\leq r$, we then consider the instance $(G,\hmset_j)$. We can further partition $H_j$ into two sub-grids $H'_j$ and $H''_j$ along the unique column $W_z$ that is contained in $H_j$, and for which $z\in Z$. Notice that all source vertices lie on the bottom boundary of $H'_j$ at distance at least $2^{i-3}$ from the left and the right boundaries of $H'_j$, while all destination vertices lie in $H''_j$, at distance at least $2^{i-3}$ from the left and the right boundaries of $H''_j$. Let $I$ and $I'$ denote the bottom boundaries of $H'_j$ and $H''_j$, respectively.


Assume first that the value $\opt_j$ of the optimal solution to instance $(G,\hmset_j)$ is at least $1024d$. Then we employ an algorithm similar to the one for Case 1: we use dynamic programming, together with the algorithm given by Theorem~\ref{thm: main w destinations far from boundary} to compute  a collection $\Sigma=\set{\sigma_1,\ldots,\sigma_z}$ of disjoint sub-intervals of $I$, and a set $\Sigma'=\set{\sigma_1',\ldots,\sigma'_z}$ of disjoint sub-intervals of $I'$, for $z=\ceil{\frac{|\mset'|}{160d}}-1$, such that the intervals $\sigma_1,\sigma_2,\ldots,\sigma_z,\sigma'_z,\ldots,\sigma_2',\sigma_1'$ appear on $\Gamma$ in this circular order, and for all $q$, $(\sigma_q,\sigma_q')$ is a good pair of intervals. For each $1\leq q\leq z$, let $(G'_{\sigma_q,\sigma'_q},\hmset'_{\sigma_q,\sigma'_q})$ denote the corresponding modified instance. The key is to notice that all such graphs $G'_{\sigma_q,\sigma'_q}$ are mutually disjoint and are contained in $H''_j$. We construct the set $\tilde {\nset}=\bigcup_{q=1}^z\tilde{\nset}_q$ of new demand pairs as before, and show that they can be routed in $H_j$ via paths that are internally disjoint from $\bigcup_{q=1}^zG'_{\sigma_q,\sigma'_q}$. The routing is straightforward and exploits the columns of $H'_j$ and the top $\sqrt{n}/4$ rows of $H''_j$.

Finally, assume that the value of the optimal solution $\opt_j$ to instance  $(G,\hmset_j)$ is less than $1024d$. 
Note that $\opt_j<2^{i+2}$ must also hold, as interval $I$ contains at most $2^{i+2}$ vertices.  %Let $d'=\min\set{d,2^{i}}$. 

Let $\hat I'$ be obtained from $I'$ by discarding its first $2^{i-3}$ and its last $2^{i-3}$ vertices, and recall that $2^i\geq d$. Then $(I,\hat I')$ is a $d$-interesting pair of intervals, and $(G,\hmset_j)$ is a perfect $(I,\hat I',d)$ sub-instance of $(G,\mset)$.
Let $(\tilde{H}_j,\hmset'_j)$ be the corresponding modified instance. Notice that $\tilde{H}_j\subseteq H''_j$. Then, from Claim~\ref{claim: modified instance preserves solutions}, the value of the optimal solution to instance $(\tilde H_j,\hmset'_j)$ is at least $\min\set{\opt_j,d}=\Omega(\opt_j)$. We can use  Theorem~\ref{thm: main w destinations far from boundary} in order to compute a $2^{O(\sqrt{\log n}\log\log n)}$-approximate solution $\pset_j$ to instance $(H'_j,\hmset'_j)$. From the above discussion $|\pset_j|\geq \frac{\opt_j}{\approxfactor}$. It now remains to route the vertices of $S(\hmset_j)$ to the corresponding vertices of $S(\hmset'_j)$ via node-disjoint paths that are internally disjoint from $\tilde H_j$. This is done in exactly the same way as before.


%Assume first that $2^i>64d$. Then, if we let $I$ be the bottom boundary of $H'_j$, excluding its first $16d$ and its last $16d$ vertices, and we define $I'$ in the same way for $H''_j$, then $(I,I')$ is a $d$-good pair of intervals, and $(G,\nset_j)$ is a perfect $(I,I,d)$-instance. We can define a modified instance $(G',\nset'_j)$ for $(G,\nset_j)$, as before. In the modified instance, the sources appear on the top boundary of $G'$, and the destination vertices $t\in T(\nset'_j)$ have $\tilde t$ appearing on the bottom boundary of $G'$. We can then solve the modified instance as it is a special case of Case 1, and then extend the routing to the original demand pairs in $\nset_j$ inside the grid $H_j$, as before.




%Finally, assume that $2^i\leq 64d$. Then the value of the optimal solution to instance $(G,\nset_j')$ is at most $2^{i+3}\leq 2^9d$, as the number of distinct source vertices in $S(\nset'_j)$ is be bounded by the width of $H'_j$, which is at most $2^{i+3}$. Let $\opt_j$ denote the value of the optimal solution to instance $(G,\mset_j')$. Let 


%-----------------------------------
%-----------------------------------
%-----------------------------------

\iffalse
%-----------------------------------
%-----------------------------------
%-----------------------------------

\paragraph{Subcase 3b: $2^i<512d$.}
 Let $\rho$ be a random integer between $0$ and $1024$. Let $Z$ be the set of all integers $1\leq z\leq \ell$, such that $z=\rho+j(1024d)$ for some integer $j$. We discard from $\mset$ all demand pairs $(s,t)$, such that, if we denote the index of $\col(s)$ by $i$ and the index of $\col(t)$ by $i'$, then there is an element $z\in Z$ for which either $|i-z|\leq 16d$ or $|i'-z|\leq 16 d$ holds. Since we select a random offset $\rho$, the probability that a pair $(s,t)$ is discarded is at most $64d/128d\leq 1/2$. Therefore, if $\mset'$ denotes the resulting set of the demand pairs, and $\opt''$ is the optimal solution to instance $(G,\mset')$, then $\expect{\opt''}\geq \opt'/2$.
 
 We partition the grid $G$ into subgrids $H_1,H_2,\ldots,H_r$, by deleting all columns $W_z$ with $z\in Z$. For each demand pair $(s,t)\in \mset'$, there is one subgrid $H_j$ containing both $s$ and $t$. 
 For each $1\leq j\leq r$, let $\mset_j\subseteq \mset'$ be the set of the demand pairs $(s,t)$ with $s,t\in H_j$. Let $\wset_j$ be the set of all columns of grid $G$ contained in $H_j$, so $|\wset_j|=128d-2$, and let $\wset'_j$ be obtained from $\wset_j$ by deleting the leftmost $15d-1$ and the rightmost $15d-1$ columns, so $|\wset'_j|=98d$. Let $\rset'$ be the set of $98d$ bottom rows of $G$, and let $H'_j\subseteq H_j$ be the square sub-grid spanned by the set $\wset''_j$ of columns and the set $\rset'$ of rows. Note that for each demand pair $(s,t)\in \mset_j$, both $s,t\in H'_j$, and moreover, $t$ is within distance at least $d$ from the boundaries of $H_j'$. 
Let $\opt_j$ be the value of the optimal solution to instance $(G,\mset_j)$, and let $\opt'_j$ be the value of the optimal solution to instance $(H'_j,\mset_j)$.

\begin{claim}\label{claim: equivalent solutions}
$\opt'_j=\Omega(\opt_j)$.
\end{claim}

Assume first that the claim is correct. Then we can use Theorem~\ref{thm: main w destinations far from boundary} in order to compute a $2^{O(\sqrt{\log n}\log\log n)}$-approximate solution $\pset_j$ to instance $(H'_j,\mset_j)$. The value of the solution is then at least $\frac{\opt_j}{2^{O(\sqrt{\log n}\log\log n)}}$. Taking the union of all resulting solutions $\pset_j$ gives us a $2^{O(\sqrt{\log n}\log\log n)}$-approximate solution to instance $(G,\mset)$. It now remains to prove the claim.

\begin{proofof}{Claim~\ref{claim: equivalent solutions}}
We assume that the value of $\opt_j$ is at least a large enough constant, since otherwise, we may simply route one demand pair of $\mset_j$ inside $H'_j$, which is possible since all $(s,t)\in\mset_j$ have $s,t\in H'_j$ and $H'_j$ is connected. Note that $\opt_j \le 96d$, since the sources of $\mset_j$ are at distance at least $16d$ from the left and right boundaries of $H_j$ and each source in $\opt_j$ takes a distinct vertex on the bottom row. Let $H''_j\subseteq H'_j$ be the $96d\times 96d$ square sub-grid spanned by columns $\wset''_j$ and rows $\rset''$, where $\wset''_j$ is obtained by deleting the leftmost and the rightmost columns of $\wset'_j$, and $\rset''$ the top two rows of $\rset'$. Note that every $(s,t)\in\mset_j$ has $s,t\in H''_j$, and the distance between the left, right, and top boundaries of $H''_j$ to those of $H'_j$ is exactly $d$. Let $U$ denote the vertices comprising the left, right, and top boundaries of $H''_j$.

Then at least $1/2$ of the demand pairs of $\opt_j$ must have paths that intersect $U$ at most $1000d/|\opt_j|$ times. Otherwise, at least $1/2$ of the demand pairs of $\opt_j$ have paths that intersect $U$ at least $1000d/|\opt_j|$ times, for a total of at least $500d$ vertices. However, $U\le 288d$, and since the paths for $\opt_j$ are node-disjoint, this is a contradiction. Then out of the $|\opt_j|/2$ demand pairs which intersect $U$ at most $1000d/|\opt_j|$ times, we arbitrarily choose $1/500$-fraction of such demand pairs, say $\opt''_j\subseteq\opt_j$, for a total of $|\opt''_j| = |\opt_j|/1000$ demand pairs, and route them inside $H'_j$, by modifying their paths in $\opt_j$. Then since the routing of $\opt''_j$ is contained in $H'_j$, $\opt'_j\ge \opt''_j=\Omega(\opt_j)$, and the claim follows. It remains to show the routing of $\opt''_j$.

For each $(s,t)\in\opt''_j$, let $P(s,t)$ denote the path which routes $(s,t)$ in $\opt_j$. Let $(u_1,\ldots,u_x)$ denote the sequence of vertices in $P(s,t)$ which belong to $U$ and appear in this order as we traverse $P(s,t)$ from $s$ to $t$. Then each $(u_y,u_{y+1})$ pair for $1\le y<x$ defines a sub-path of $P(s,t)$ which is either contained in $H''_j$ or internally disjoint from $H''_j$. Let $\pset''$ denote the set of all such sub-paths which are internally disjoint from $H''_j$ over all $(s,t)\in \opt''_j$. Then $|\pset''|\le |\opt''_j|\cdot 1000d/|\opt_j| \le d$. Then It is straightforward to route all demand pairs of $\opt''_j$ as follows: we first arbitrarily order all paths in $\pset''$ and denote them by $\pset''=\set{P_1,\ldots,P_q}$ ($q\le d$). We modify each $P_i$ such that if $u$ and $v$ are the endpoints of $P_i$, then we route $u$ to the closest vertex in $H'_j$ at distance exactly $i$ from $U$ of $H''_j$, and likewise route $v$ to the closest vertex in $H'_j$ at distance exactly $i$ from $U$. We then connect $u$ to $v$ using vertices at distance $i$ from $U$ in $H'_j$. Then to route $(s,t)\in\opt''_j$, we traverse $P(s,t)$ from $s$ to $t$, but replace each sub-path of $P(s,t)$ which is internally disjoint from $H''_j$ with the corresponding path in $\pset''$. Note that two paths $P_a,P_b\in \pset''$ may share vertices iff $b=a+1$ and the endpoints of $P_a$ are $(u_k,u_{k+1})$ and $P_b$'s are $(u_{k+1},u_{k+2})$, and appear consecutively on some path $P(s,t)$ for some $(s,t)\in\opt''_j$. In this case, we may simply concatenate $P_a$ and $P_b$ on a single edge at distance $a$ and $a+1$ from $u_{k+1}$.
\end{proofof}

\fi
  

==> arxiv final/hard-example.tex <==
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
\label{------------------------------------sec: hard example--------------------------------------}

\section{Negative Example for the Distance Property} \label{sec: hard-example}
We say that an instance $(G,\mset)$ of \NDPgrid is \emph{perfectly routable} iff there is a set $\pset$ of node-disjoint paths in $G$, routing all demand pairs in $\mset$.

Assume now that we are given some instance $(G,\mset)$ of \NDPgrid, where all vertices of $S(\mset)$ lie on the top boundary of the grid $G$, and let $\mset' \subseteq \mset$ be any subset of the demand pairs, whose sources are all distinct.
For any two sources $s, s' \in S(\mset')$, let $N_{\mset'}(s,s')$ be the number of all sources in $S(\mset')$ lying between $s$ and $s'$ on the top boundary of $G$.
Recall that we say that $\mset'$ has the $1$-distance property iff for each $(s,t), (s',t') \in \mset'$, $N_{\mset'}(s,s')  \leq d(t,t')$.
For convenience, in the remainder of this section, we refer to the $1$-distance property simply as the \emph{distance property}.

The goal of this section is to construct a family of perfectly routable instances  $(G,\mset)$ of \NDPgrid, with sources lying on the top boundary of the grid, such that every subset $\mset'\subseteq \mset$ of the demand pairs, if $\mset'$ has the distance property, then $|\mset'|\leq |\mset|/2^{\Omega(\sqrt{\log n})}$, where $n=|V(G)|$.
More precisely, we prove the following theorem.

\begin{theorem} \label{thm: main hard}
For each sufficiently large integer $n$, there is a perfectly routable instance $(G,\mset)$ of \rNDPgrid, where $G$ is an $(n^{\Theta(1)}\times n^{\Theta(1)})$-grid, all source vertices in $S(\mset)$ lie on the top boundary of $G$, and for every subset $\mset' \subseteq \mset$ of the demand pairs that has the distance property, $|\mset'|\leq |\mset| / 2^{\Omega(\sqrt{\log n})}$.
\end{theorem}

We note that in the instances that we construct, the destination vertices may lie close to the grid boundaries; however, adding a padding of $\sqrt n$ columns on either side of the grid, and possibly additional rows at the bottom of the grid, rectifies this problem without affecting the final result.

We use a parameter $g=1.1$. Our construction is iterative. In iteration $i$, we construct a level-$i$ instance $(G_i,\mset_i)$; the instance is perfectly routable and has all vertices of $S(\mset_i)$ lying on the top boundary of $G_i$.  We denote the dimensions of the grid $G_i$ by $\ell_i$ (so $G_i$ is the $(\ell_i\times \ell_i)$-grid), and we denote $|\mset_i|=N_i$. We will ensure that the largest subset of the demand pairs in $\mset_i$ that has the distance property has cardinality at most $N_i/g^i$. We now set the parameters $\ell_i$ and $N_i$. Let $\gamma_i=20g^{2i}$. We then set $N_0=1$, and for all $i\geq 1$, $N_i=2\gamma_{i-1}N_{i-1}$. A simple calculation shows that $N_i=2^{\Theta(i^2)}$. We also set $\ell_i=9N_ig^i=2^{\Theta(i^2)}$. It is now enough to prove the following theorem.



\begin{theorem}\label{thm: iterations}
For every integer $i\geq 0$, there is an instance $(G_i,\mset_i)$ of \rNDPgrid, such that:

\begin{itemize}
\item $G_i$ is the $(\ell_i\times \ell_i)$ grid, $|\mset_i|=N_i$; 
\item all source vertices of $\mset_i$ lie on the top boundary of $G_i$;
\item instance $(G_i,\mset_i)$ is perfectly routable; and
\item for every subset $\mset'_i\subseteq \mset_i$ of demand pairs that has the distance property, $|\mset'_i|\leq N_i/g^i$.
\end{itemize}
\end{theorem}

Indeed, suppose we are given a large enough parameter $n$. We set $\rho=\ceil{\sqrt{\log n}}$, and consider the level-$\rho$ instance $(G_{\rho},\mset_{\rho})$. Then $G_{\rho}$ is the $(\ell_{\rho}\times \ell_{\rho})$ grid, where $\ell_{\rho}=n^{\Theta(1)}$, and the instance $(G_{\rho},\mset_{\rho})$ is perfectly routable, with all source vertices lying on the top row of $G_{\rho}$. Moreover, if $\mset'\subseteq \mset_{\rho}$ has the distance property, then $|\mset'|\leq |\mset_{\rho}|/g^{\rho}=|\mset_{\rho}|/2^{\Omega(\sqrt{\log n})}$. In the remainder of this section we prove Theorem~\ref{thm: iterations}.



\begin{figure}[h]
\scalebox{0.18}{\includegraphics{level0}}
\caption{Level-$0$ instance \label{fig: level0}}
\end{figure}

\begin{figure}[h]
\scalebox{0.4}{\includegraphics{flip}}
\caption{Flipping a level-$i$ instance \label{fig: flip}}
\end{figure}


\iffalse
\begin{figure}[h]
%\centering
\hspace{1cm}
\subfigure[Level-$0$ instance]{\scalebox{0.18}{\includegraphics{level0}}\label{fig: level0}}
\hspace{2cm}
\subfigure[Flipping a level-$i$ instance]{
\scalebox{0.4}{\includegraphics{flip}}\label{fig: flip}}
\caption{
  Illustration to the proof of Theorem~\ref{thm: iterations}.
  \label{fig: routing-spaced}}
\end{figure}
\fi

\iffalse

We set a parameter $g = 0.9$.
For some sufficiently large parameter $\rho$, let $N=2^{\Omega(\rho^2)}$.
We will construct a $\sqrt{N} \times \sqrt{N}$ grid $G$ with a set $\mset$ of $\Omega(\sqrt{N})$ demand pairs.
We will place all the sources on the top boundary and all the destinations on a single row of $G$.
We will ensure that all the demand pairs in $\mset$ can be routed via node-disjoint paths, but on the other hand, no subset of more than $g^\rho \cdot |\mset| = |\mset|/2^{\Omega(\sqrt{\log N})}$ of demand pairs has distance property.


The idea is to construct the instance in a hierarchical fashion, in a sequence of steps, which we call \textit{levels}.
There are $\rho$ levels, in total.
For each $0 \leq i \leq \rho$, the level-$i$ instance $I_i = (G_i, \mset_i)$ is a $\ell_i \times \ell_i$ grid $G_i$ with $|\mset_i| = N_i$ demand pairs.
We say that the instance $I_i$ is \emph{perfect} iff
(i) it is routable;
(ii) all sources $S(\mset_i)$ lie on the top boundary of $G_i$; and
(iii) no subset of $N'_i > g^i N_i$ demand pairs of $\mset_i$ has distance property.
For each level $0 \leq i \leq \rho$, we set a parameter $\gamma_i = 20/g^{2i}$.


\begin{theorem} \label{thm: induct hard}
  For each $0 \leq i \leq \rho$, there is a \textit{perfect} level-$i$ instance $I_i = (G_i, \mset_i)$ with the following properties:
  \begin{itemize}
    \item $N_0 = 1$ and for all other $0 < i \leq \rho$, $N_i = 2 \gamma_{i-1}N_{i-1}$
    \item $\ell_i = 9 \cdot N_i/g^i$
  \end{itemize}
\end{theorem}

Before proving the theorem, let us complete the proof of Theorem \ref{thm: main hard} using it.

\proofof{Theorem \ref{thm: main hard}}
Consider level-$\rho$ instance $I_{\rho}=(G_\rho, \mset_\rho)$.
The number of demand pairs:
\[ N_\rho = N_0 \cdot \prod_{i=1}^{\rho} 2\gamma_{i-1}  \leq \gamma_\rho ^ {O(\rho)} \leq g^{-O(\rho^2)}\]
The size of the grid is $\ell_\rho \times \ell_\rho$ where $\ell_\rho = O(N_\rho / g^\rho) \leq g^{-O(\rho^2)}$.
In other words, $n = g^{-O(\rho^2)}$.
Thus, the final gap we achieve is $N'_\rho/N_\rho < g^\rho = 2^{-\Theta(\rho)} = 2^{-\Omega(\sqrt{\log n})}$.
\endproofof

Notice that in the instance that we construct, the sources are quite close to the grid boundary.
This is not a problem, since we can pad $G_\rho$ by $\ell_\rho$ columns on left and right sides and $2 \ell_\rho$ rows on the bottom.
In the new \emph{routable} instance obtained, all the destination nodes are at distance $\Omega(\ell_\rho)$ from the grid boundaries.
In the remainder of the section, we prove Theorem \ref{thm: induct hard}.

%-------------------------------------
%-------------------------------------
%-------------------------------------
%-------------------------------------
\fi



\proofof{Theorem \ref{thm: iterations}}
The proof is by induction on $i$.
The base case is when $i=0$.
The level-$0$ instance, $(G_0, \mset_0)$, is defined as follows. Notice that from our setting of the parameters, $N_0=1$ and $\ell_0=9$. Graph $G_0$ is the $(9 \times 9)$ grid, and $\mset_0$ consists of a single demand pair $(s_0, t_0)$, with both $s_0$ and $t_0$ lying on the first column of the grid, with $s_0$ lying on its first row and $t_0$ on its $5$th row (see Figure \ref{fig: level0}).
It is immediate to see that this instance has all required properties.
 
We now assume that the theorem holds for some integer $i\geq 0$, and prove it for $(i+1)$. We let $G_{i+1}$ be the $(\ell_{i+1}\times \ell_{i+1})$-grid. In order to define the set $\mset_{i+1}$ of demand pairs, we carefully combine $2\gamma_i$ copies of level-$i$ instances. Each such copy will be mapped to a square sub-grid of $G_{i+1}$, with the different copies being horizontally aligned, and lying roughly midway between the top and the bottom rows of $G_{i+1}$. For convenience, we denote $\gamma_i$ by $\gamma$ from now on.



Let $R^*$ be the top row of the grid $G_{i+1}$, and let $R'$ be the row appearing at distance exactly $\gamma N_i$ from the bottom row of $G_{i+1}$. Let $\rset$ be the set of $\ell_i$ consecutive rows of $G_{i+1}$, such that $R'$ is the last row in $\rset$. Consider the horizontal strip $S$ of $G_{i+1}$ spanned by the rows in $\rset$. Next, we define $2\gamma_i$ square $(\ell_i\times \ell_i)$ sub-grids of $S$, to which the copies of the level-$i$ instances will be mapped. The sub-grids are denoted by $A_1,A_2, \ldots,A_{2\gamma}$. We place these sub-grids side-by-side in this left-to-right order inside $S$, so that the left boundary of $A_1$ is at a  distance at least $\gamma N_i$ from the left boundary of $G_{i+1}$ (see Figure~\ref{fig: leveli}). Since:

\[\ell_{i+1}=9N_{i+1}g^{i+1}=18\gamma N_i g^{i+1} \geq (2\gamma)\cdot \ell_i + \gamma N_i,\]

there is enough horizontal space to find such a placement.

For each $1\leq j\leq 2\gamma$, where $j$ is an even integer, we view $A_j$ as a copy of the level-$i$ instance $(G_i,\mset_i)$. In other words, we map the vertices and the edges of $G_i$ to the vertices and the edges $A_j$ in the natural manner. This mapping defines a set $\nset_j$ of pairs of vertices of $A_j$, that correspond to the demand pairs in $\mset_i$.

Similarly, for each $1\leq j\leq 2\gamma$, where $j$ is an odd integer, we view $A_j$ as a copy of the level-$i$ instance $(G_i,\mset_i)$, except that now the instance is {\bf flipped}: when we map $G_i$ to $A_j$, we reverse the order of its rows (so they now appear from bottom to top), and the order of its columns (so they now appear from right to left); in particular, all source vertices of $S(\mset_i)$ appear on the bottom boundary of $A_j$ (see Figure~\ref{fig: flip}). This mapping again defines a set $\nset_j$ of pairs of vertices of $A_j$, that correspond to the demand pairs in $\mset_i$.

We are now ready to define the set $\mset_{i+1}$ of the demand pairs of our level-$(i+1)$ instance. This set is a union of $2\gamma$ disjoint subsets, $\nset_1',\ldots,\nset_{2\gamma}'$. For each $1\leq j\leq 2\gamma$, set ${\nset}'_j$ of demand pairs contains, for each pair $(s,t)\in \nset_j$, one new demand pair $(s',t')$, whose destination vertex $t'=t$, and the source vertex appears on the top boundary $R^*$ of $G_{i+1}$ (we specify its exact location below).

%Similarly, set $\tilde{\nset}'_j$ of demand pairs contains, for each pair $(s,t)\in \nset'_j$, one new demand pair $(s',t')$, whose destination vertex $t'=t$, and the source vertex appears on $R^*$. 

Finally, we need to specify the locations of the $N_{i+1}=2\gamma N_i$ new source vertices on $R^*$. The sources are mapped to the $2\gamma N_i$ leftmost vertices of $R^*$. We first place the sources of the odd-indexed sets: $S(\nset_{2\gamma-1}'),S(\nset_{2\gamma-3}'),\ldots,S(\nset_3'),S(\nset_1')$ in this left-to-right order; within each set $S(\nset_{2j-1}')$, the sources are placed in the reversed order of their appearance on the bottom boundary of $A_{2j-1}$. 
Next, we place the sources of the even-indexed sets $S(\nset_2'),S(\nset_4'),\ldots,S(\nset_{2\gamma}')$ in this left-to-right order; within each set $\nset_{2j}'$, the sources are placed in exactly the same order as the order of their appearance on the top boundary of $A_{2j}$ (see Figure~\ref{fig: leveli}). 
This completes the description of the level-$(i+1)$ instance $(G_{i+1}, \mset_{i+1})$.
In the remainder of the proof, we show that it has the required properties.






%  Notice that $N_0=1$ and $\ell_0 = 9 = 9 \cdot N_0/g^0$ by our construction.
 % Now we complete the induction step by constructing level-$i+1$ instance $I_{i+1} = (G_{i+1}, \mset_{i+1})$.
 % We will use the \emph{perfect} level-$i$ instance $I_i = (G_i, \mset_i)$ with above mentioned properties guaranteed to exist by the induction hypothesis.

\begin{figure}[h]
\center
\scalebox{0.4}{\includegraphics{leveli}}
\caption{Level-$(i+1)$ instance $(G_{i+1},\mset_{i+1})$.
% TODO The sources of a constituent level-$i$ instance $I$ are denoted by $S(I)$.
\label{fig: leveli}}
\end{figure}


\iffalse
\paragraph{Level-$i+1$ Instance.}
Consider a $\ell_{i+1} \times \ell_{i+1}$ grid $G_{i+1}$.
Intuitively, we will consider $2\gamma_i$ copies of level-$i$ instance $I_i$, place their sources on the top row of $G_{i+1}$ and \textit{interlace} their destinations in $G_{i+1}$ (see: Figure \ref{fig: leveli}).
Let $(A^1, \cdots, A^{\gamma_i})$, $(B^1, \cdots, B^{\gamma_i})$ be fresh copies of level-$i$ instance $I_{i}$.
We call $A^1, \cdots, A^{\gamma_i}$ as \textit{blue} instances and $B^1, \cdots, B^{\gamma_i}$ as \textit{red} instances.
%Let $s(1), s(2), \cdots, s({N_i})$ be $N_i$ left-most vertices on the top row of $G_i$.
%For each $1 \leq j \leq \eta$ and $1 \leq k \leq N_{i-1}$, we map $k^{th}$ source node from left of the instance $I^j$ to the node $s(k + (j-1) \cdot N_{i-1})$.

Let $R$ be the top row of $G_{i+1}$ and $v(1), v(2). \ldots, v(\ell_{i+1})$ be the nodes of $R$ in the natural left-to-right order.
We map leftmost $\gamma_i N_i$ nodes on $R$ to the sources of \textit{blue} instances in \textbf{right-to-left} order (see: Figure \ref{fig: leveli}).
Formally, let $s_A(j,1), \ldots, s_A(j,N_i)$ be the sources $S(A^j)$ in left-to-right order.
For each $1 \leq k \leq N_i$, we map the source $s_A(j,k)$ to the node $v((j-1)N_i + k)$ on $R$ that we denote by $s'_A(j,k)$.
Similarly, we map next $\gamma_i N_i$ nodes of $R$ to the sources of \textit{red} instances in \textbf{left-to-right} order.
Formally, let $s_B(j,1), \ldots, s_B(j,N_i)$ be the sources $S(B^j)$ in left-to-right order.
For each $1 \leq k \leq N_i$, we map the source $s_B(j,k)$ to the node $v(\gamma_iN_i + (j-1)N_i + k)$ on $R$ that we denote by $s'_B(j,k)$.
Note that the placement of sources is well defined since $\ell_{i+1} \geq N_{i+1}$.
This completes the mapping of sources on the top row $R$ of $G_{i+1}$.


Our idea of placing the destination nodes motivates yet another definition: \textit{flipped} instances.
For a grid $G_i$, the flipped grid $G_{-i}$ is obtained by toggling the order of rows and columns in $G_i$ (see: Figure \ref{fig: flip}).
For an instance $A^j = (G_i, \mset_i)$, the corresponding flipped instance is given by $A^{-j} = (G_{-i}, \mset_i)$. 
Notice that each of the flipped instance $A^{-j}$ is also a perfect instance inheriting the same properties as $A^j$.


For $1 \leq j \leq \gamma_i$, we put the grids corresponding to \textit{blue} and \textit{red} instances $A^{-j}$ and $B^j$ side-by-side in alternating fashion, in their natural left-to-right order far away from top, left and bottom grid boundaries (see: Figure \ref{fig: leveli}).
We also ensure that all the destinations are mapped to the same row of $G_{i+1}$.
For each demand pair $(s_A(j,k), t_A(j,k))$ of $A^{-j}$, we add a unique demand pair $(s'_A(j,k), t_A(j,k))$ to $\mset_{i+1}$.
Similarly, for each demand pair $(s_B(j,k), t_B(j,k))$ of $B^{j}$, we also add a unique demand pair $(s'_B(j,k), t_B(j,k))$ to $\mset_{i+1}$.
%------------------------
%------------------------
%------------------------
%------------------------
\fi


It is immediate from our construction that $G_{i+1}$ is the $(\ell_{i+1}\times \ell_{i+1})$-grid, that $|\mset_{i+1}|=2\gamma_i N_i=N_{i+1}$, and that all source vertices of  $\mset_{i+1}$ lie on the top boundary of $G_{i+1}$. It now remains to show that instance $(G_{i+1},\mset_{i+1})$ is perfectly routable, and
that every subset $\hmset\subseteq \mset_{i+1}$ of demand pairs that has the distance property has cardinality at most $N_{i+1}/g^{i+1}$.
We prove this in the following two claims.

%Note that when we put these instances, we only map the destinations, as sources are already mapped on the first row of $G_{i+1}$.
%We note that the distance of $\gamma_i N_i$ from the left and bottom boundary; and $t_i$ from the top and right boundary is sufficient.
%Notice that the size of grid $\ell_{i+1} \times \ell_{i+1}$, where $\ell_{i+1} = 9 \cdot N_{i+1}/g_{i+1} \geq \gamma_i N_i + 2 \gamma_i \ell_i$ is sufficient to route every demand pair of $I_i$ by node-disjoint paths.

\begin{claim} \label{clm: routable}
 Instance $(G_{i+1},\mset_{i+1})$ is perfectly routable.
\end{claim}
\begin{proof}
  From the induction hypothesis, for each $1\leq j\leq 2\gamma$, there is a set $\pset_j$ of node-disjoint paths contained in $A_j$, that route all demand pairs in $\nset_j$. In order to complete the proof, it is enough to show that there is a set $\pset^*$ of node-disjoint paths, that are internally disjoint from $\bigcup_{j=1}^{2\gamma}A_j$, such that for each $1\leq j\leq 2\gamma$, for each pair $(s,t)\in \nset_j$, some path $P(s,t)\in\pset^*$ connects $s$ to its corresponding new source vertex $s'$.  
  %Notice that $\ell_{i+1} = 9 \cdot N_{i+1}/g^{i+1} \geq \gamma_i N_i + 2 \gamma_i \ell_i$.
 It is straightforward to construct the required set $\pset^*$ of paths, by utilizing the $\gamma N_i$ columns to the left of $A_1$ and the $\gamma N_i$ rows lying above and below the strip $S$ (see Figure \ref{fig: leveli}). 
\end{proof}

The next claim will finish the proof of Theorem~\ref{thm: iterations}.


\begin{claim} \label{clm: dist prop}
Let $\hmset\subseteq\mset_{i+1}$ be any subset of demand pairs that has the distance property. Then $|\hmset|\leq N_{i+1}/g^{i+1}$.
\end{claim}
\begin{proof}
Assume for contradiction that $|\hmset|> N_{i+1}/g^{i+1}$. For each $1\leq j\leq 2\gamma$, let $\hmset'_j=\nset'_j\cap \hmset$, and let $\hmset_j\subseteq \nset_j$ contain all demand pairs $(s,t)$ for which the corresponding new demand pair $(s',t')\in \hmset_j$. Notice that all demand pairs in $\hmset_j$ must also have the distance property inside the level-$i$ instance defined by $A_j$, and so, from the induction hypothesis, $|\hmset'_j|=|\hmset_j|\leq  N_i/g^i$. We say that index $1\leq j\leq 2\gamma$ is \emph{interesting} iff $\hmset'_j\neq \emptyset$. From the above discussion, the number of interesting indices is at least $\frac{N_{i+1}}{g^{i+1}}/\frac{N_i}{g^i} = \frac{N_{i+1}}{g\cdot N_i}=\frac{2\gamma}{g}>1.8\gamma$. 
We claim that there is an index $j> 0.8\gamma$, such that both $2j-1$ and $2j$ are interesting. Indeed, assume otherwise. Then the number of interesting indices is at most $1.6\gamma+0.2\gamma\leq 1.8\gamma$, a contradiction.
Let $j^*>0.8\gamma$ be an index, such that both $2j^*-1$ and $2j^*$ are interesting.
 Let $(s_1,t_1)\in \hmset'_{2j^*-1}$, and let $(s_2,t_2)\in \hmset'_{2j^*}$ be any demand pairs. From our construction, the two grids $A_{2j^*-1}$ and $A_{2j^*}$ are consecutive, and so $d(t_1,t_2) < 3 \ell_i = 27 N_i g^i$. We next show that $N_{\hmset}(s_1,s_2)>27N_ig^i$, contradicting the distance property of $\hmset$. The following claim will then finish the proof.
 
 
\begin{claim}
 $N_{\hmset}(s_1,s_2) > 27N_ig^i$
\end{claim}
\begin{proof}
Notice that if $(s,t)\in \hmset$ is a demand pair with $s$ lying to the left of $s_1$ on $R^*$, then $(s,t)\in \hmset'_{2j-1}$, where $j\geq j^*> 0.8\gamma$. Similarly, if   $(s,t)\in \hmset$ is a demand pair with $s$ lying to the right of $s_2$ on $R^*$, then $(s,t)\in \hmset'_{2j}$, where $j\geq j^*> 0.8\gamma$. Recall that for each $j$, 
  $|\hmset'_j|\leq  N_i/g^i$, and so overall the number of the demand pairs $(s,t)\in \hmset$ with $s$ lying to the left of $s_1$ or to the right of $s_2$ is bounded by $0.4\gamma\cdot N_i/g^i$ (this number includes the pairs $(s_1,t_1)$ and $(s_2,t_2)$). The remaining demand pairs must lie between $s_1$ and $s_2$ and therefore contribute to $N_{\hmset}(s_1,s_2)$. We then get that:
  
\[\begin{split}
N_{\hmset}(s_1,s_2)&\geq |\hmset|-\frac{0.4\gamma\cdot N_i}{g^i}\\
&\geq \frac{N_{i+1}}{g^{i+1}}-\frac{0.4\gamma\cdot N_i}{g^i}\\
&=\frac{2\gamma N_i}{1.1g^{i}}-\frac{0.4\gamma\cdot N_i}{g^i}\\
&\geq 1.4\frac{\gamma N_i}{g^i} \\
&=28 N_ig^i.\end{split}\]
  
    %Recall that $j \geq 0.8 \gamma_i$.
%    Let $\cset = \set{A^{-\gamma_i}, \ldots, A^{-j}, B^{j}, \ldots, B^{\gamma_i}}$ be a set of level-$i$ instances.
%    Notice that if a source $s \in S(\mset'_{i+1})$ appears either to the left of $s'$ or to the right of $s''$ on $R$, then $s$ belongs to some instance in $\cset$.
%    From level-$i$ analysis, at most $g^iN_i$ sources of $\mset'_{i+1}$ may belong to any such instance.
%    Thus, 
%    \[N_{\mset'_{i+1}}(s',s'') \geq |\mset'_{i+1}| -  |\cset| g^i N_i \]
%    Since $j \geq 0.8 \cdot \gamma_i$, $|\cset| \leq 2(\gamma_i - j)+2 \leq 0.5 \cdot \gamma_i$.
%    Recall that $|\mset'_{i+1}| > g^{i+1}N_{i+1}$, $\gamma_i = 20/g^{2i}$ and $N_{i+1} = 2 \gamma_i N_i$.
%    Substituting these values, we obtain the claimed bound.
  \end{proof}
\end{proof}
%
%From Claim \ref{clm: routable} and Claim \ref{clm: dist prop}, we conclude that $I_{i+1}$ is a \emph{perfect} instance, completing the induction step.
%
%
\endproofof




==> arxiv final/ndp-to-edp.tex <==
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
\label{------------------------------------sec: ndp tp edp--------------------------------------}
\section{Approximating NDP/EDP on Walls with Sources on the Boundary}\label{sec: ndp to edp}
In this section we prove Theorem \ref{thm: main edp}, by extending our results for \rNDPgrid to \EDP and \NDP on wall graphs.

\begin{figure}[h]
\center
\scalebox{0.20}{\includegraphics{dotted-wall}}
\caption{The red dotted edges are deleted to obtain wall $\hat G$ from grid $G$.
\label{fig: dotted wall}}
\end{figure}

Let $G=G^{\ell,h}$ be a grid of length $\ell$ and height $h$.
Assume that $\ell>0$ is an even integer, and that $h>0$.
For every column $W_j$ of the grid, let $e^j_1,\ldots,e^j_{h-1}$ be the edges of $W_j$ indexed in their top-to-bottom order. Let $E^*(G)\subseteq E(G)$ contain all edges $e^j_z$, where $z\neq j \mod 2$, and let $\hat G$ be the graph obtained from $G\setminus E^*(G)$, by deleting all degree-$1$ vertices from it.
Graph $\hat G$ is called a \emph{wall of length $\ell/2$ and height $h$} (see Figure~\ref{fig: dotted wall}).
%The boundary of $\hat G$, $\Gamma(\hat G)$ is the collection of all the edges constituting its outer face.
Consider the subgraph of $\hat G$ induced by all horizontal edges of the grid $G$ that belong to $\hat G$. This graph is a collection of $h$ node-disjoint paths, that we refer to as the \emph{rows} of $\hat G$, and denote them by $R_1,\ldots,R_h$ in this top-to-bottom order; notice that $R_j$ is a sub-path of the $j$th row of $G$ for all $j$. Graph $\hat G$ contains a unique collection $\wset$ of $\ell/2$ node-disjoint paths that connect vertices of $R_1$ to vertices of $R_h$ and are internally disjoint from $R_1$ and $R_h$. We refer to the paths in $\wset$ as the \emph{columns} of $\hat G$, and denote them by $W_1,\ldots,W_{\ell/2}$ in this left-to-right order.
Paths $W_1, W_{\ell/2},R_1$ and $R_h$ are called the left, right, top and bottom boundary edges of $\hat G$, respectively, and their union is the boundary of $\hat G$, that we denote by $\Gamma(\hat G)$.

In both \NDPwall and \EDPwall problems, the input is a wall $\hat G$ of length $\sqrt n/2$ and height $\sqrt n$ (we assume that $\sqrt n/2$ is an integer), and a collection $\mset = \set{(s_1,t_1), \ldots, (s_k, t_k)}$ of $k$ demand pairs. The goal is to route the maximum number of the demand pairs via paths that are node-disjoint (for \NDPwall) or edge-disjoint (for \EDPwall). We will exploit the $(\sqrt n\times \sqrt n)$ grid $G$, and the fact that $\hat G \subseteq G$ can be obtained from $G$ as described above. 

For any two nodes $u,v$ of $\hat G$, we denote the shortest-path distance between them in $\hat G$ by $\hat d(u,v)$. Distances between subsets of vertices, and between a vertex and a subset of vertices, are defined as before, using $\hat d$.

The following simple observation relates the values of the optimal solutions to the \EDPwall and \NDPwall problems, defined over the same wall $\hat G$ and the same set $\mset$ of demand pairs.

\begin{observation}\label{obs: NDP vs EDP in walls}
Let $\hat G$ be a wall of length $\sqrt n/2$ and height $\sqrt n$, and let $\mset = \set{(s_1,t_1), \ldots, (s_k, t_k)}$ be a set of $k$ demand pairs. Let $\optEDP$ be the value of the optimal solution to the \EDPwall problem instance $(\hat G, \mset)$, and let $\optNDP$ be the value of the optimal solution to the \NDPwall problem instance $(\hat G, \mset)$. Then: $\optNDP\leq \optEDP\leq O(\optNDP)$.
\end{observation}
\begin{proof}
Observe first that for any set $\pset$ of paths in $\hat G$, if the paths in $\pset$ are mutually node-disjoint, then they are also mutually edge-disjoint. Therefore, $\optNDP\leq \optEDP$. 

To show the other direction, consider any set $\pset$ of paths, such that the paths in $\pset$ are edge-disjoint. It is enough to show that there is a subset $\pset'\subseteq\pset$ of paths that are node-disjoint, and $|\pset'|\geq \Omega(|\pset|)$. Since the maximum vertex degree in $\hat G$ is $3$, the only way for two paths $P,P'\in \pset$ to share a vertex $x$ is when $x$ is an endpoint of at least one of the two paths.

We construct a directed graph $H$, whose vertex set is $\set{v_P\mid P\in \pset}$, and there is an edge $(v_P,v_{P'})$ iff an endpoint of $P'$ belongs to $P$. It is immediate to verify that the maximum in-degree of any vertex in $H$ is $4$. Therefore, there is a set $U\subseteq V(H)$ of $\Omega(|V_H|)$ vertices, such that no two vertices of $U$ are connected with an edge. We let $\pset'=\set{P\mid v_P\in U}$. Then the paths in $\pset'$ are node-disjoint, and $|\pset'|=\Omega(|\pset|)$.
\end{proof}

Since for any set $\pset$ of node-disjoint paths, the paths in $\pset$ are also mutually edge-disjoint, it is now enough to prove Theorem~\ref{thm: main edp} for the \NDPwall problem, with all source vertices lying on the wall boundary. We do so in the remainder of this section.

Our main approach is to consider the corresponding instance $(G,\mset)$ of the \NDPgrid problem on the underlying grid $G$, and to exploit our algorithm for this problem.
However, we cannot use this approach directly, since the boundary of the wall $\hat G$ is not contained in the boundary of the grid $G$, and so some of the source vertices of  $S(\mset)$ may not lie on $\Gamma(G)$. We overcome this difficulty by mapping each vertex in $S(\mset)$ to its closest vertex lying on $\Gamma(G)$. Formally, we define a new set $\mset'$ of demand pairs, containing, for each pair $(s,t)\in \mset$, a new pair $(s',t')$, with $t'=t$, and $s'$ defined as follows. If $s\in \Gamma(G)$, then $s'=s$; otherwise, either $s$ belongs to the first column of $\hat G$, in which case $s'$ is defined to be the vertex of $\Gamma(G)$ lying immediately to the left of $s$; or $s$ belongs to the last column of $\hat G$, in which case $s'$ is defined to be the vertex of $\Gamma(G)$ lying immediately to its right (see Figure~\ref{fig: dotted wall}). The following simple observation shows that the solution value does not change by much.

\begin{observation} \label{obs: perturbed edp}
Let $\opt$ be the value of the optimal solution to instance $(\hat G,\mset)$ of \NDPwall, and let $\opt'$ be defined in the same way for instance $(\hat G,\mset')$. Then $\opt'=\Omega(\opt)$. Moreover, given any set $\pset'$ of node-disjoint paths routing a subset of the demand pairs in $\mset'$, there is an efficient algorithm to compute a set $\pset$ of $\Omega(|\pset'|)$ node-disjoint paths routing a subsets of the demand pairs in $\mset$.
 \end{observation}
 
 \begin{proof}
 In order to prove the first assertion, let $\pset^*$ be the optimal solution to instance $(\hat G,\mset)$. We show that there is a set $\pset'$ of $\Omega(|\pset^*|)$ paths routing demand pairs in $\mset'$. Let $\pset''$ be obtained from $\pset^*$ as follows. Consider any path $P\in \pset^*$, and assume that it routes some pair $(s,t)\in \mset$. If $(s,t)\in \mset'$, then we add $P$ to $\pset''$; otherwise, we extend $P$ by adding the edge $(s,s')$ to it, and add the resulting path to $\pset''$. Consider the final set $\pset''$ of paths. While $|\pset''|=|\pset^*|$, it is possible that the paths in $\pset''$ are no longer node-disjoint. However, a pair $P_1,P_2\in \pset''$ of paths may share a vertex $x$ iff $x$ is an endpoint of at least one of the two paths. We can now employ the same argument as in the proof of Observation~\ref{obs: NDP vs EDP in walls} to obtain a subset $\pset'\subseteq \pset''$ of node-disjoint paths, with $|\pset'|\geq\Omega(\pset'')$. 
 
 The proof of the second assertion is almost identical.
 \end{proof}

From now on, it is sufficient to design a randomized $\approxfactor$-approximation algorithm to the new instance $(\hat G,\mset')$ of \NDPwall. Therefore, from now on we will assume that all source vertices lie on $\Gamma(\hat G)\cap \Gamma(G)$.



%--------

 Our first step is, as before, to consider a special case of the problem, where the destination vertices lie far from the boundary of the wall. We prove the following analogue of Theorem~\ref{thm: main w destinations far from boundary}.



\begin{theorem} \label{thm: far edp}
  There is an efficient randomized algorithm $\hat \aset$, that, given an instance $(\hat G, \mset)$ of the \NDPwall
  problem, with all sources lying on $\Gamma(G)\cap \Gamma(\hat G)$ (where $G$ is the grid corresponding to $\hat G$), and an integer $\opt$, such that the value of the optimal solution to instance $(\hat G,\mset)$ of \NDPwall  is at least $\opt$, and every destination vertex lies at a distance at least $\opt/\eta$ from $\Gamma(\hat G)$ in $\hat G$, returns a solution that routes at least $\opt/\approxfactor$ demand pairs in $\hat G$, with high probability.
\end{theorem}



\begin{proof}
%We further assume that no terminal vertex lie on corner of $G$, losing at most an additive constant in the approximation guarantee.
%The main idea of the proof is to consider the \rNDPgrid instance on the underlying grid $G$, and to adapt the algorithm $\aset$ for \rNDPgrid from Section \ref{sec:alg-overview} to this setting.
%To this end, we exploit the following key properties: (i) $\hat G\subseteq G$; (ii) maximum vertex degree in $\hat G$ is $3$; and (iii) the snakes constructed in Section \erf{sec: snakes} are \textit{wide enough}.
%
 Consider the \rNDPgrid instance defined over the grid $G$, with the set $\mset$ of the demand pairs. Since $\hat G\subseteq G$, the value of the optimal solution to this instance is at least $\opt$. We can apply  Algorithm $\aset$  to instance $(G,\mset)$ of \rNDPgrid, to obtain a set
 $\pset$ of node-disjoint paths routing some subset $\tmset\subseteq \mset$ of demand pairs in graph $G$, such that with high probability, $|\tmset|\geq \opt / \approxfactor$.
We now show that all demand pairs in $\tmset$ can also be routed in the wall $\hat G$.
Indeed, in the analysis in Section \ref{sec: snakes}, we have constructed disjoint level-$\rho$ snakes of width at least $3$, such that each demand pair $(s,t)\in \tmset$ is contained in a distinct snake, that we denote by $\yset(s,t)$.
With a loss of an additive constant in the approximation guarantee, we can ensure that no snake passes through any corner of $G$.

\begin{observation}
  Let $\yset=(\Y_1,\ldots,\Y_z)$ be any snake of width at least $3$ in the grid $G$. Let $H$ be the union of all graphs $\Y_j\cap \hat G$, for $1\leq j\leq z$. Then $H$ is a connected sub-graph of $\hat G$.
\end{observation}

It is now immediate to obtain a routing of the demand pairs in $\tmset$ via node-disjoint paths in $\hat G$. For every snake $\yset(s,t)$, let $H(s,t)$ be the corresponding sub-graph of $\hat G$, given by the above observation. Then all graphs $\set{H(s,t)}_{(s,t)\in \tmset}$ are mutually disjoint, and each such graph is connected. We simply connect $s$ to $t$ by any path contained in $H(s,t)$.\end{proof}

Finally, we complete the proof of Theorem~\ref{thm: main edp}, by removing the assumption that the destination vertices lie far from the wall boundaries. As before, we assume that we are given an instance $(\hat G,\mset)$ of \NDPwall, such that, if $G$ denotes the corresponding grid graph, then all source vertices in $S(\mset)$ lie on $\Gamma(G)\cap \Gamma(\hat G)$. As before, we use the algorithm from Section \ref{sec:destinations anywhere} on the underlying grid $G$ and adapt the resulting solution to the wall $\hat G$.

%With only an additive loss in the approximation guarantee, we can assume that no terminal lie on any corner of $G$.
Recall that for every destination vertex $t \in T(\mset)$, we denoted by $\tilde t$ the vertex of $\Gamma(G)$ minimizing $d(t,\tilde t)$, breaking ties arbitrarily.
For any subset $\mset' \subseteq \mset$ of demand pairs, we denoted by $\tilde T(\mset') = \set{\tilde t \mid t \in T(\mset')}$.
If all vertices of $\tset(\mset)$ lie on the boundary $\Gamma(\hat G)$ of wall $\hat G$, then we can efficiently obtain a constant-factor approximation for the problem using standard dynamic programming techniques.
Thus, we assume from now on that $\hat d(t, \tilde t) \geq 1$ for each $t \in T(\mset)$.

Recall that we showed that it suffices to consider the case where all sources $S(\mset)$ lie on a single boundary edge $\Gamma_q$ of $G$, and all vertices of $\tilde T(\mset)$ lie on a single boundary edge $\Gamma_{q'}$ of $G$, where possibly $\Gamma_q=\Gamma_{q'}$.
We further saw that it suffices to consider only two cases:
(i) $d(t, \tilde t) \geq \opt/\eta$ for all destination nodes $t$; or
(ii) we are given an integer $1 \leq d \leq \opt/2\eta$ such that $d \leq d(t, \tilde t) < 2d$ for all destination nodes $t$, and $\opt > 2^{13}d$.
In case (i), we can compute a factor $\approxfactor$-approximate solution directly using Theorem \ref{thm: far edp}.
In the remainder of this section, we consider case (ii).


Let $\mset'$ be the set of the demand pairs that was chosen to be routed by our algorithm from Section~\ref{sec:destinations anywhere}. Then all vertices of $\tilde T(\mset')$ lie on the same boundary edge of the grid -- we assume w.l.o.g. that it is the bottom boundary. Recall that we have defined a collection $\set{(G_1,\mset_1),\ldots,(G_z,\mset_z)}$ of modified sub-instances, such that all grids $G_1,\ldots,G_z$ are disjoint from each other and from the top $\sqrt n/4$ rows of $G$, and in each of the instances $(G_i,\mset_i)$, the destination vertices lie far enough from the boundary of the grid $G_i$, so that Theorem~\ref{thm: main w destinations far from boundary} could be applied  to each such sub-instance separately. Let $\mset_i'\subseteq \mset'$ be the subset of the demand pairs corresponding to the pairs in $\mset_i$.  For each $1\leq i\leq z$, we have also defined a set $\tilde N_i$ of pairs, connecting the original source vertices in $S(\mset'_i)$ to their corresponding source vertices in $S(\mset_i)$. We have implicitly constructed, for each $1\leq i\leq z$, a snake $\yset_i$, inside which the demand pairs in $\tilde N_i$ are routed. All snakes $\yset_1,\ldots,\yset_z$ are disjoint, and have width at least $3|\nset_i|$ each. We can now translate this routing into a set of node-disjoint paths routing the demand pairs in $\mset'$ in the wall $\hat G$. The routing inside each sub-grid $G_i$ is altered exactly like in the proof of Theorem~\ref{thm: far edp}; the routings of the sets $\tilde{\nset}_i$ of demand pairs exploit the same snakes $\yset_i$ inside the wall $\hat G$. 




\iffalse

Recall that in the case of $\Gamma_q \neq \Gamma_{q'}$, the algorithm of Section \ref{subsec: general case algo} selected a subset $\mset' \subseteq \mset$ of at least $\Omega(\opt/\sqrt{\log n})$ demand pairs for routing and defined $\Omega(\opt/d)$ sub-instances $\set{(G_i, \mset'_i)}_{i=1}^{z}$ of the problem, such that:
\begin{itemize}
  \item all grids $G_i$ are disjoint from each other, and they appear at a distance at least $\Omega(\opt/\sqrt{\log n})$ from $\Gamma_q$. Moreover, no two subgrids $G_i$ and $G_j$ share a column of $G$
  \item $\opt(G_i, \mset'_i) \geq \min{\set{\opt, d}}$
  \item For each demand pair $(s,t) \in \mset'$, there is a unique demand pair $(s', t) \in \mset'_i$ for some $1 \leq i \leq z$ such that $s' \in \Gamma(G_i)$ and $d(t, \Gamma(G_i)) \geq d$
  \item The corresponding sources $S'(\mset') = \set{s' \mid s \in \mset'}$ appear in the same left-to-right order as $S(\mset')$
\end{itemize}
It is now straightforward to compute routing of $d/\approxfactor$ demand pairs inside each of the subgrids $G_i$ using Theorem \ref{thm: far edp}.
Finally, since all the subgrids $\set{G_i}$ are far away from $\Gamma_q$, we can extend this routing to route $\opt/\approxfactor$ demand pairs of $\mset$ in $\hat G$.


The remaining case in which $\Gamma_q = \Gamma_{q'}$, can also be dealt in the same way, obtaining an edge-disjoint routing of at least $\opt/\approxfactor$ demand pairs in $\hat G$.
Notice that the demand pairs that we select to route in $\hat G$ has unique sources and destinations.
Since the maximum vertex degree in $\hat G$ is $3$, each such edge-disjoint routing is node-disjoint as well.
Theorem \ref{thm: main edp} then follows by recalling that $\optEDP = \Theta(\optNDP)$.

\fi

==> arxiv final/shadow-property.tex <==


%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
\label{---------------------------sec: shadow property-------------------------------}
\section{The Shadow Property}\label{sec: shadow property}
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
%-------------------------------------------------------------
This section is dedicated to proving Theorem~\ref{thm: shadow property for one set of squares}. 

%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
%--------------------------------------------------------------
  
For every demand pair $(s,t)\in \hmset$, we let $P(s,t)$ denote the path routing this pair in $\pset$. We assume that $G$ is embedded into the plane in the natural manner, and we construct a number of discs in the plane. Whenever we refer to a disc, we mean a simple disc, whose boundary is a simple cycle. Let $D^0$ denote the disc whose outer boundary is the boundary of the grid $G$. 

\begin{definition}
We say that a disc $D$ in the plane is \emph{canonical}, if either (i)  $D=D^0$, or (ii) we can partition the boundary $\sigma(D)$ of $D$ into four contiguous segments, $\sigma_1(D),\sigma_2(D),\sigma_3(D),\sigma_4(D)$, such that $\sigma_1(D)\subseteq R^*$; $\sigma_3(D)$ is contained in the boundary of some square $Q\in \qset$; $\sigma_2(D)$ is contained in some path $P(s,t)\in \pset$, and $\sigma_4(D)$ is contained in some path $P(s',t')\in \pset$ (where possibly $(s,t)=(s',t')$).
\end{definition}

\begin{definition}
We say that a collection $\dset$ of canonical discs is \emph{nested} iff for every pair $D,D'\in \dset$, either one of the discs is contained in the other, or they are disjoint. Moreover, if the boundaries of two distinct discs $D,D'\in \dset$ intersect, then $\sigma(D)\cap \sigma(D')\subseteq R^*$ must hold.
\end{definition}


 Assume now that we are given a nested collection $\dset$ of canonical discs. Consider some disc $D\in \dset$, and let $\dset'\subseteq \dset$ be the set of all discs $D'$ with $D'\subseteq D$. We define the region of the plane associated with $D$ as $R_{\dset}(D)=D\setminus (\bigcup_{D'\in \dset'}D')$.

The idea is to compute a collection $\dset=\set{D^0,D^1,\ldots,D^z}$ of nested canonical discs, and for every disc $D^i$ a set $\mset_i\subseteq \hmset$ of demand pairs, such that all demand pairs in $\mset_i$ are routed inside the region $R_{\dset}(D^i)$ by $\pset$. Clearly, for $i\neq i'$, $\mset_i\cap \mset_{i'}=\emptyset$ will hold. We denote by $\overline{\mset}=\hmset\setminus \bigcup_i\mset_i$ the set of the demand pairs we discard, and we will ensure that $|\overline{\mset}|$ is small enough compared to $|\hmset|$. 

Given a set $\overline{\mset}$ of discarded demand pairs, we say that a square $Q\in \qset$ is \emph{active} iff at least one demand pair in $\hmset\setminus\overline{\mset}$ has a destination vertex lying in $Q$. We say that the set $\dset$ of discs \emph{respects} the active squares, iff for every active square $Q\in \qset$, there is a unique disc $D^i\in \dset$ with $Q\subseteq R_{\dset}(D^i)$. We will ensure that the set $\dset$ of discs we construct respects all active squares.

\paragraph*{Heavy demand pairs.}
Consider any demand pair $(s,t)\in \hmset$ and the path $P(s,t)$ routing $(s,t)$ in $\pset$. We say that $(s,t)$ \emph{covers} the demand pair $(s',t')\in \hmset$ iff $P(s,t)$ intersects the unique square $Q\in \qset$ with $t'\in Q$. Notice that $(s',t')$ may be covered by at most $4d$ demand pairs. This is since $t'$ belongs to exactly one square of $\qset$; for every pair $(s,t)$ covering $(s',t')$, path $P(s,t)$ must contain a vertex from the boundary of that square; and the length of the boundary of each such square is at most $4d$. We say that demand pair $(s,t)$ is \emph{heavy} if it covers more than $2^{9}d\log n$ other pairs in $\hmset$.

\begin{observation}
The number of heavy demand pairs is at most $|\hmset|/(2^7\log n)$.
\end{observation}
\begin{proof}
Assume otherwise. Then the total number of demand pairs covered by heavy pairs (counting multiplicities) is more than $4|\hmset|d$. But every demand pair can be covered by at most $4d$ demand pairs, a contradiction.
\end{proof}


\paragraph*{Partitioning algorithm.}
Initially, we let $\overline{\mset}$ contain all heavy demand pairs, so $|\overline{\mset}|\leq |\hmset|/(128\log n)$. We start with $\dset=\set{D^0}$, and let the corresponding set of the demand pairs be $\mset_0=\hmset\setminus \overline{\mset}$. We then iterate. Let $D^i\in \dset$ be any disc and let $\mset_i$ be the corresponding set of demand pairs. Consider any pair $(s,t),(s',t')\in \mset_i$ of demand pairs. Let $N_{\mset_i}(t,t')$ be the number of the demand pairs $(s'',t'')\in \mset_i$ whose source lies between $s$ and $s'$ on $R^*$. Let $N'_{\mset_i}(t,t')$ denote the number of the remaining demand pairs in $\mset_i$ -- those pairs whose sources do not lie between $s$ and $s'$ on $R^*$.

\begin{definition}
 We say that $(s,t),(s',t')$ is a \emph{candidate pair for $\mset_i$} iff:

\begin{itemize}
\item there is a square $Q\in \qset$ with $t,t'\in Q$; and

\item both $N_{\mset_i}(t,t'),N'_{\mset_i}(t,t')>2^{20}d\log^3n$.
\end{itemize}
\end{definition}

If a candidate pair $(s,t),(s',t')$ exists in $\mset_i$, then we do the following.
Let $Q\in \qset$ be the square that contains both $t$ and $t'$.  We define a new canonical disc $D'\subseteq D^i$. Let $v$ be the first vertex on path $P(s,t)$ that lies in $Q$ (we view the path as directed from $s$ to $t$), and let $P'(s,t)$ be the sub-path of $P(s,t)$ between $s$ and $v$. Similarly, let $v'$ be the first vertex on path $P(s',t')$ that lies in $Q$, and let $P'(s',t')$ be the sub-path of $P(s',t')$ between $s'$ and $v'$. We let $\sigma_3(D')$ be a path connecting $v$ to $v'$, such that $\sigma_3(D')$ is contained in the boundary of $Q$, and the length of $\sigma_3(D')$ is at most $2d$.  Let $\sigma_2(D')=P'(s,t)$, $\sigma_4(D')=P'(s',t')$, and let $\sigma_1(D')$ be the subpath of $R^*$ between $s$ and $s'$. Finally, let $\sigma(D')$ be the concatenation of these four curves, and let $D'$ be the disc whose boundary is $\sigma(D')$. Let $\overline{\mset}_i\subseteq\mset_i$ contain all demand pairs $(s'',t'')$, such that either (i) $P(s'',t'')$ crosses $\sigma(D')$; or (ii) $(s,t)$ covers $(s'',t'')$; or (iii) $(s',t')$ covers $(s'',t'')$. Recall that there are at most $2d$ pairs of the first type (as all their paths must cross $\sigma_3(D')$), and at most $2^{9}d\log n$ pairs of each of the remaining types (as we have discarded all heavy demand pairs).
 Altogether, $|\overline{\mset}_i|\leq 2d+2^{10}d\log n$.
  Notice that $\overline{\mset}_i$ contains the pairs $(s,t)$ and $(s',t')$, and also all pairs whose destinations lie in the squares of $\qset$ that $\sigma(D')$ visits, including the pairs whose destinations lie in $Q$.

We  create two new subsets of the demand pairs: $\mset'\subseteq \mset_i\setminus \overline{\mset}_i$ contains all demand pairs whose corresponding path in $\pset$ is contained in the new disc $D'$, and we update $\mset_i$ to contain all remaining demand pairs of the original set $\mset_i$ (excluding the pairs in $\mset'$ and $\overline{\mset}_i$). Therefore, for every demand pair in the new set $\mset_i$, the path routing the pair in $\pset$ is contained in $R_{\dset}(D^i)\setminus D'$. We then add $D'$ to $\dset$, with $\mset'$ as the corresponding set of the demand pairs, and we add all demand pairs in $\overline{\mset}_i$ to $\overline {\mset}$. It is easy to verify that the resulting set of discs remains nested and canonical. From the above discussion, it also respects the currently active squares.

We have discarded at most $2d+2^{10}d\log n\leq 2^{11}d\log n$ demand pairs in the current iteration, but both $\mset'$ and the new set $\mset_i$ contain at least $2^{20}d\log^3n-2^{10}d\log n -2d\geq 2^{19}d\log^3n$ demand pairs (after excluding the discarded demand pairs).

We continue this partitioning procedure, as long as there is some disc $D^i\in \dset$, whose corresponding set $\mset_i$ of demand pairs contains a candidate pair $(s,t),(s',t')$. Let $\dset=\set{D^0,\ldots,D^z}$ be the final set of discs, and for each $i$, let $\mset_i$ be the corresponding set of the demand pairs. 


\begin{claim}\label{claim: charging}
At the end of the algorithm,  $|\overline{\mset}|< |\hmset|/(64\log n)$.
\end{claim}

\begin{proof}
Recall that at the beginning of the algorithm, $|\overline{\mset}|\leq |\hmset|/(128\log n)$ held. Over the course of the algorithm, for every demand pair $(s,t)\in \hmset\setminus \overline{\mset}$, we define a budget of $(s,t)$ as follows. Assume that $(s,t)$ belongs to some set $\mset_i$, corresponding to some disc $D^i\in \dset$. We set the budget of $(s,t)$ to be $B(s,t)=\frac{\log(|\mset_i|)}{128\log^2 n}$. Notice that this budget may change as the algorithm progresses. At the beginning of the algorithm, the total budget of all demand pairs is at most $\frac{|\hmset|}{128\log n}$, while $|\overline{\mset}|\leq \frac{|\hmset|}{128\log n}$. It is now enough to prove that throughout the algorithm, the total budget of all demand pairs plus the cardinality of $\overline{\mset}$ do not increase.

Consider some iteration of the algorithm, where we processed some set $\mset_i$ of demand pairs as above, adding a new set $\overline{\mset}_i$ of demand pairs to $\overline{\mset}$, and creating two new sets of demand pairs: $\mset'$ and $\mset'_i$ (that replaces $\mset_i$). Recall that we have guaranteed that $|\overline{\mset}_i|\leq 2^{11}d\log n$, while $|\mset'|,|\mset'_i|\geq 2^{19}d\log^3n$. Assume without loss of generality that $|\mset'|\leq |\mset'_i|$. Then the budget of every demand pair in $\mset'$ decreases by at least $\frac{1}{128\log^2n}$ (as $|\mset'|\leq |\mset_i|/2$), and the total decrease in the budgets is therefore at least $\frac{|\mset'|}{128\log^2n}\geq \frac{2^{19}d\log^3n}{128\log^2n}\geq 2^{12}d\log n$, while $|\overline{\mset}|$ increases by at most $2^{11}d\log n$. Therefore, the total budget of all demand pairs plus $|\overline{\mset}|$ do not increase.
\end{proof}


From the above discussion, the final set $\dset$ of discs is canonical, nested, and respects all remaining active squares.

%------------------------------------------------------------
%------------------------------------------------------------
%------------------------------------------------------------
\paragraph*{Boundary Pairs.}
%------------------------------------------------------------
%------------------------------------------------------------
%------------------------------------------------------------
Consider some disc $D^i\in \dset$, and assume first that $|\mset_i|\geq 2^{21}d\log^3n$.
Let $a_i,b_i$ be the two endpoints of $\sigma_1(D^i)$, and let $\zset^i_0\subseteq \mset_i$ contain $2^{20}d\log^3n$ demand pairs whose sources lie closest to $a_i$ and $2^{20}d\log^3n$ demand pairs whose sources lie closest to $b_i$. If $|\mset_i|< 2^{21}d\log^3n$, then we set $\zset^i_0=\mset_i$.
In either case, $|\zset^i_0|\leq 2^{21}d\log^3n$. We call the demand pairs in $\zset^i_0$ \emph{boundary pairs}. If $|\mset_i|>2^{23}d\log^4n$, then we discard the boundary pairs from $\mset_i$, and add them to $\overline{\mset}$. After this procedure, we are still guaranteed that $|\overline{\mset}|\leq \frac{|\hmset|}{64\log n}+\frac{|\hmset|}{4\log n}\leq \frac{|\hmset|}{2\log n}$. So we assume from now on that whenever the boundary pairs are present in $\mset_i$, $|\mset_i|\leq 2^{23}d\log^4n$. 



%------------------------------------------------------------
%------------------------------------------------------------
%------------------------------------------------------------
\paragraph*{Forest of Discs.}
%------------------------------------------------------------
%------------------------------------------------------------
%------------------------------------------------------------
It would be convenient for us to organize the discs in $\dset$ into a directed forest $F$, in a natural way. In each arborescence of the forest, the edges will be directed towards the root.
The set of vertices of $F$ is $v_0,v_1,\ldots,v_z$, where $v_i$ represents disc $D^i$. There is a directed edge $(v_i,v_{i'})$ iff $D^i\subsetneq D^{i'}$, and there is no disc $D^x\in \dset$ with $D^i\subsetneq D^x\subsetneq D^{i'}$. Since the discs in $\dset$ are nested, it is immediate to verify that $F$ is indeed a directed forest. For every arborescence $\tau$ of $F$, the root of $\tau$ is the vertex $v_i$ corresponding to a disc $D^i$ that has the largest area. For every vertex $v_j\in V(F)$, we let its weight $w_j$ be $|\mset_j|$.
We denote by $\mset'=\bigcup_{i=0}^z \mset_i$, so $|{\mset'}|\geq |\hmset|/2$.

We use the following well-known result. For completeness, its proof appears in Appendix.

\begin{claim}\label{claim: partition the forest} There is an efficient algorithm, that, given a directed forest $F$ with $n$ vertices, computes a partition $\yset=\set{Y_1,\ldots,Y_{\ceil{\log n}}}$ of $V(F)$ into subsets, such that for each $1\leq j\leq \ceil{\log n}$, $F[Y_j]$ is a collection of disjoint directed paths, that we denote by $\pset_j$. Moreover, for all $v,v'\in Y_j$, if there is a directed path from $v$ to $v'$ in $F$, then they both lie on the same path in $\pset_j$.
\end{claim} 



Let $\set{Y_1,\ldots,Y_{\ceil{\log z}}}$ be the partition of $V(F)$ given by Claim~\ref{claim: partition the forest}. Then there is some index $1\leq x\leq \ceil{\log z}$, such that the total weight of all vertices in $Y_x$ is at least $|{\mset'}|/\ceil{\log z}\geq |\hmset|/(2\log n)$. 
Let $\dset'\subseteq \dset$ be the set of all discs $D^i$, whose corresponding vertex $v_i\in Y_x$, and let $\mset''\subseteq \mset'$ be the set of all demand pairs that belong to all such discs, that is, $\mset''=\bigcup_{D^i\in\dset'}\mset_i$. Consider now some vertex $v_i\in Y_x$. Notice that at most one child-vertex $v_{i'}$ of $v_i$ in the forest $F$ may belong to $Y_x$. If such a vertex $v_{i'}$ does not exist, then all demand pairs in $\mset_i$ are called \emph{right pairs}. Otherwise, for each demand pair $(s,t)\in \mset_i$, if $s$ appears to the left of $\sigma_1(\mset_{i'})$ on $R^*$, then we call it a \emph{left pair}, and otherwise we call it a right pair. Therefore, all demand pairs in $\mset''$ are now partitioned into right pairs and left pairs. We assume without loss of generality that at least half of the demand pairs in $\mset''$ are left pairs; the other case is symmetric. Let $\mset'''\subseteq \mset''$ be the set of all left pairs, so $|\mset'''|\geq |\mset''|/2\geq |\hmset|/(4\log n)$.

\begin{claim}\label{claim: the final shadow property}
The squares in $\qset$ have the $r$-shadow property with respect to $\mset'''$, for $r=2^{23}\log^4n$.
\end{claim}

Notice that, assuming the claim is correct, from Observation~\ref{obs: boosting shadow}, there is a subset $\hmset'\subseteq \mset'''$ of at least $\frac{|\mset'''|}{2^{25}\log^4n}\geq\frac{|\hmset|}{2^{27}\log^5n}\geq\frac{|\hmset|}{\log^6n}$ demand pairs, such that all squares in $\qset$ have the $1$-shadow property with respect to $\hmset'$ (we have used the assumption that $n$ is large enough, so $\log n\geq 2^{27}$). It now remains to prove Claim~\ref{claim: the final shadow property}.




\begin{proofof}{Claim~\ref{claim: the final shadow property}}
Assume otherwise, and let $Q\in \qset$ be some square that does not have the $r$-shadow property with respect to $\mset'''$. Since $Q$ must be an active square, there is some disc $D^i\in \dset'$, such that the square $Q$ belongs to $R_{\dset}(D^i)$. Consider the shadow $J_{\tmset'''}(Q)$ of $Q$, and let $s,s'$ be its left and right endpoints respectively. Then there are two demand pairs $(s,t),(s',t')\in \mset'''$, with $t,t'\in Q$, such that at least $rd$ vertices of $S(\mset''')$ lie between $s$ and $s'$ on $R^*$. Let $S'$ be the set of all these source vertices, and let $\nset\subseteq\mset'''$ be their corresponding demand pairs. We claim that $\nset\subseteq \mset_i$. Indeed, assume that there is some demand pair $(s^*,t^*)\in \nset$ that does not belong to $\mset_i$. Then it must belong to some set $\mset_j$, where $v_j$ is a descendant of $v_i$ in the forest $F$. This can only happen if $v_j\in Y_x$. Moreover, the segment $\sigma_1(D^j)$ must be contained in the shadow $L_{\tmset''}(Q)$. Let $v_{i'}$ be the child vertex of $v_i$ that lies in $Y_x$ (such a vertex must exist due to the vertex $v_j\in Y_x$). Then $v_j$ is also the descendant of $v_{i'}$, and $D^j\subseteq D^{i'}\subseteq D^i$. In particular, the segment $\sigma_1(D^{i'})$ must also be contained in the shadow $L_{\tmset''}(Q)$. But then $(s,t)$ is a left pair, while $(s',t')$ is a right pair, which is impossible, since we have discarded all the right pairs. We conclude that $\nset\subseteq \mset_i$.

Since $|\mset_i|\geq |\nset|>rd=2^{23}d\log^4n$, we have deleted the boundary pairs from the set $\mset_i$, and so in particular, $(s,t)$ and $(s',t')$ are not boundary pairs. It follows that $(s,t)$ and $(s',t')$ was a valid candidate pair, and we should have continued our partitioning algorithm.
\end{proofof}






==> arxiv final/snakes.tex <==
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
\label{------------------------------------sec: snakes--------------------------------------}
\section{Finding the Routing}\label{sec: snakes}
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------


The goal of this section is to prove Theorem~\ref{thm: snake-like routing}. 
Recall that we are given as input a hierarchical system $\thset=(\qset_1,\ldots,\qset_{\rho})\in \fset$ of squares and a hierarchical L-partition $(\jset_1,\ldots,\jset_{\rho})$ of the row $R^*$ of $G'$.
We are also given a coloring $f$ of $\thset$ by the corresponding hierarchical system  $\cset$ of colors, and a set $\tmset'\subseteq \tmset$ of at most $d_1$ demand pairs that are perfect for $f$.
In particular, we are guaranteed that for each demand pair $(s,t)\in \tmset'$, both $s$ and $t$ are assigned the same level-$\rho$ color, and, moreover, for every $1 \leq h \leq \rho$, for every level-$h$ color $c_h$, at most $d_h$ demand pairs in $\tilde \mset'$ are assigned color $c_h$.
Recall that all destination vertices appear within distance at least $\opt/\eta>4d_1$ from the grid boundary. For consistency, we define a single level-$0$ square $Q_0$, as follows: let $\rset$ contain all but the $d_1$ top and the $d_1$ bottom rows of the grid $G$, and let $\wset$ contain all but the first $d_1$ and the last $d_1$ columns of the grid $G$. Then $Q_0$ is the sub-grid of $G$ spanned by the rows in $\rset$ and the columns in $\wset$. We discard from $\qset_1$ all level-$1$ squares that are not contained in $Q_0$: such squares do not contain any destination vertices. We also discard from all other sets $\qset_h$ all descendant-squares of the level-$1$ squares that were discarded. Abusing the notation, we denote the resulting hierarchical system of squares by $\thset$. For convenience, we define a unique level-$0$ color $c_0$, that serves as a parent of every level-$1$ color, and we assign this color to $Q_0$.


Assume w.l.o.g. that $\tmset'=\set{(s_1,t_1),\ldots,(s_{z},t_{z})}$, where $s_1,\ldots,s_{z}$ appear on $R^*$ in this left-to-right order.
We define a set $\hmset=\set{(s_i,t_i)\mid i\equiv 1 \mod 2 \eta^3}$, of $\Omega(|\tilde \mset'|/\eta^3)$ demand pairs. In the remainder of this section, we show an efficient algorithm for routing all demand pairs in $\hmset$.
Consider a level-$h$ color $c_h$, where $1 \leq h \leq \rho$.
Let $N(c_h)$ be the number of demand pairs $(s,t)\in \hmset$, such that $s$ and $t$ have level-$h$ color $c_h$. 
Since $d_h = \eta^{\rho-h+3}$, $N(c_h) \leq \ceil{d_h/(2\eta^3)} \leq \eta^{\rho-h}$, and $|\hmset|\leq d_1/(2\eta^3)$.
Notice that for every level-$\rho$ color $c_\rho$, $N(c_\rho) \leq 1$ holds.

We say that a level-$h$ square $Q\in \qset_h$ is \emph{empty} iff no demand pair in $\hmset$ has a destination in $Q$.
As before, for each square $Q$, we let $\Gamma(Q)$ denote its boundary. 
For each level $1 \leq h \leq \rho$ and for each level-$h$ square $Q_h \in \qset_{h}$, let $Q_h^+$ be an extended square, obtained by adding a margin of $d_{h}/\eta$ on all sides of $Q_h$; we also let $Q_0^+$ be obtained from $Q_0$ by adding a margin of $d_1/\eta$ around it. Notice that the distance between $\Gamma(Q_0^+)$ and $\Gamma(G)$ remains at least $d_1/2$. Notice also that for each $1\leq h\leq \rho$, for each pair $Q,\hat Q\in \qset_h$ of level $h$ squares, $d(Q^+,\hat Q^+)\geq d_h/2$.

\begin{figure}[h]
\center
\scalebox{0.28}{\includegraphics{q0-and-g}}
\caption{Square $Q_0$ inside $G$. Original squares $Q$ of $\hset$ are represented by solid lines and the corresponding augmented squares $Q^+$ are represented by dashed lines.
The sources $s_j$ of $\hat \mset$ are represented by red nodes on the top boundary of $G'$, and their copies $s'_j$ are on the top row of $Q_0^+$. The paths of $\pset_0$ are shown in blue.
\label{fig: q0 and g}}
\end{figure}


Let $I'_0$ be the set of the $3 \cdot N(c_0)$ leftmost vertices on the top row of $Q_0^+$.
We map the vertices of $S(\hmset)$ to the vertices of $I'_0$ as follows: if $s$ is the $j$th vertex from the left in $S(\hmset)$, then it is mapped to the $(3j)$th leftmost vertex of $I'_0$, that we denote by $s'$.
For every level $1\leq h\leq \rho$, for every level-$h$ interval $I_h\in \iset_h$ of $R^*$, we can now naturally define a corresponding interval $I'_h$ of $I'_0$ as the smallest interval containing all vertices in $\set{s'_j\mid s_j\in I_h}$. We then let $\iset'_h=\set{I'_h\mid I_h\in \iset_h}$, so that $(\iset'_1,\ldots,\iset'_{\rho})$ can be viewed as a hierarchical partition of $I'_0$.
The parent-child relationship between the new intervals is defined exactly as before. Let $\iset'_0=\set{I'_0}$.


The following observation is immediate (see Figure \ref{fig: q0 and g}):
\begin{observation} \label{obs: paths outside q0+}
  There is an efficient algorithm to compute a set $\pset_0$ of node-disjoint paths, connecting every source $s_j \in \sset(\hat \mset)$ to its corresponding copy $s'_j \in I'_0$, such that the paths in $\pset_0$ are internally disjoint from $Q_0^+$.
\end{observation}

In order to define the routing of all demand pairs in $\hat \mset$, we use special a structure called a \emph{snake}, which we define next.
Recall that,
given a set $\rset$ of consecutive rows of $G$ and a set $\wset$ of consecutive columns of $G$, we denoted by $\Y(\rset,\wset)$ the subgraph of $G$ spanned by the rows in $\rset$ and the columns in $\wset$; we refer to such a graph as a \emph{corridor}.


Let $\Y=\Y(\rset,\wset)$ be any corridor.
Let $R'$ and $R''$ be the first and the last row of $\rset$ respectively, and let $W'$ and $W''$ be the first and the last column of $\wset$ respectively.
Each of the four paths $\Y\cap R',\Y\cap R'',\Y\cap W'$ and $\Y\cap W''$ is called a \emph{boundary edge} of $\Y$, and their union is called the \emph{boundary} of $\Y$. The width of the corridor $\Y$ is $w(\Y)=\min\set{|\rset|,|\wset|}$.
We say that two corridors $\Y,\Y'$ are \emph{internally disjoint}, iff every vertex $v\in \Y\cap \Y'$ belongs to the boundaries of both corridors.
We say that two internally disjoint corridors $\Y,\Y'$ are \emph{neighbors} iff $\Y\cap \Y'\neq \emptyset$.
 
 We are now ready to define snakes. A snake $\yset$ of length $z$ is a sequence $(\Y_1,\Y_2,\ldots,\Y_{z})$ of $z$ corridors that are pairwise internally disjoint, such that for all $1\leq z',z'' \leq z$, $\Y_{z'}$ is a neighbor of $\Y_{z''}$ iff $|z'-z''|=1$. The width of the snake is defined to be the minimum of $\min_{1\leq z'<z}\set{|\Y_{z'}\cap \Y_{z'+1}|}$, and $\min_{1\leq z'\leq z}\set{w(\Y_{z'})}$.
 We say that a node $u \in \yset$ iff $u \in \bigcup_{z'=1}^z \Y_{z'}$.
 Notice that given a snake $\yset$, there is a unique simple cycle $\sigma(\yset)$ in $G$ such that all the nodes $u \in \yset$ lie on or inside $\sigma(\yset)$ and all other nodes of $G$ lie outside it.
We call $\sigma(\yset)$ the \emph{boundary} of $\yset$.
We say that a pair of snakes $\yset_1$ and $\yset_2$ are \emph{internally disjoint} iff there is a boundary edge $\Sigma_1$ of some corridor of $\yset_1$ and a boundary edge $\Sigma_2$ of some corridor of $\yset_2$ such that for every vertex $u$ with $u \in \yset_1$ and $u \in \yset_2$, $u$ must belong to $V(\Sigma_1) \cap V(\Sigma_2)$.
 We use the following simple claim, whose proof can be found, e.g. in~\cite{NDP-hardness}.

 \begin{claim}\label{claim: routing in a snake}
Let $\yset=(\Y_1,\ldots,\Y_{z})$ be a snake of width $w$, and let $A$ and $A'$ be two sets of vertices with $|A|=|A'|\leq w-2$, such that the vertices of $A$ lie on a single boundary edge of $\Y_1$ and the vertices of $A'$ lie on a single boundary edge of $\Y_{z}$. There is an efficient algorithm, that, given the snake $\yset$, and the sets $A$ and $A'$ of vertices as above, computes a set $\qset$ of node-disjoint paths contained in $\bigcup_{z'=1}^{z}\Y_{z'}$, that  connect every vertex of $A$ to a distinct vertex of $A'$. 
 \end{claim}

\begin{definition}
Let $0\leq h\leq \rho$ be a level, let $c_h\in \chi_h$ be a level-$h$ color, and let $\yset$ be a snake.  We say that a snake $\yset$ is a \emph{valid level-$h$ snake for color $c_h$} iff:

\begin{itemize}
\item $\yset\subseteq Q_0^+$;
\item $\yset$ has width at least $3 \cdot N(c_h)$;
\item $\yset$ contains the interval $I' \in \iset_h'$, corresponding to the interval $I\in \iset_h$ that was used in defining color $c_h$, as a part of the top boundary of its first corridor; and
\item for each non-empty level-$h$ square $Q\in \qset_h$, whose level-$h$ color is $c_h$, $Q^+$ is a corridor of $\yset$. 
\end{itemize}
\end{definition}


The following lemma is central to proving Theorem~\ref{thm: snake-like routing}.

\begin{lemma}\label{lemma: building snakes}
There is an efficient algorithm, that constructs, for each level $1\leq h\leq \rho$, for each level-$h$ color $c_h$, a valid level-$h$ snake $\yset(c_h)$ for this color, such that all snakes of the same level are disjoint.
\end{lemma}

We provide the proof of the lemma below, after completing the proof of Theorem~\ref{thm: snake-like routing} using it.
Fix some level-$\rho$ color $c_{\rho}$.
Recall that $\hmset$ contains at most one demand pair $(s,t)$, such that $s$ and $t$ are assigned the level-$\rho$ color $c_{\rho}$.
Recall that $s'\in I'_0$ is the vertex on the top boundary of $Q_0^+$ to which $s$ is mapped.
We route the pair $(s',t)$ inside the valid level-$\rho$ snake $\yset=\yset(c_{\rho})$ given by Lemma~\ref{lemma: building snakes}.
This snake is guaranteed to contain both the level-$\rho$ interval $I'\in \iset'(\rho)$ to which $s'$ belongs, and the non-empty level-$\rho$ square
$Q_{\rho}$ that contains $t$ (as the level-$\rho$ color of $Q_{\rho}$ must be $c_{\rho}$).
We select an arbitrary path $P$ connecting $s'$ to $t$ inside $\yset$.
In order to complete the routing, we combine these paths with the set $\pset_0$ of paths computed in Observation \ref{obs: paths outside q0+}.
As all level-$\rho$ snakes are disjoint, we obtain a valid routing of at least $|\hmset|\geq |\tmset'|/\eta^3 = |\tilde \mset'|/2^{O(\sqrt{\log n})}$ demand pairs. It now remains to prove Lemma~\ref{lemma: building snakes}.
 

 
 \begin{proofof}{Lemma~\ref{lemma: building snakes}}
The proof is by induction on $h$. For level $0$, we construct a single level-$0$ snake $\yset(c_0)$, consisting of a single corridor $Q_0^+$. Clearly, this is a valid level-$0$ snake for color $c_0$.
Assume now that the claim holds for some level $0\leq h<\rho$.
We prove that it holds for level $(h+1)$.

Fix a level-$h$ interval $I_h\in \iset_h$, and its corresponding level-$h$ color $c_h$.
Let $\yset=\yset(c_h)$ be the valid level-$h$ snake for $c_h$, given by the induction hypothesis.
Recall that for each non-empty level-$h$ square $Q$ of color $c_h$, $Q^+$ is a corridor of $\yset$.
The following claim completes the induction step and Lemma \ref{lemma: building snakes} follows.

\begin{claim} \label{clm: construct child snakes master}
 There is an efficient algorithm, that, given a valid level-$h$ snake $\yset(c_h)$ for a level-$h$ color $c_h$, constructs, for every child-color $c_{h+1}$ of $c_h$, a valid level-$(h+1)$ snake $\yset(c_{h+1})$, such that all resulting level-$(h+1)$ snakes are disjoint from each other and are contained in $\yset(c_h)$.
\end{claim}

\begin{proof}
 We will construct a number of \emph{sub-snakes} \footnote{Each of the sub-snake that we construct is a snake as defined earlier. We use the term `sub-snake' to distinguish them from the final snake $\yset(c_{h+1})$, that is obtained by concatenating a number of sub-snakes.}
  for each color $c_{h+1}$, and concatenate them together to construct a snake $\yset(c_{h+1})$ with claimed properties.
  To this end, we will construct sub-snakes of two types: Sub-snakes of type $1$ will be contained in $\yset$, but they will be internally disjoint from all non-empty level-$h$ squares of color $c_h$. Each sub-snake of type $2$ will be contained inside some non-empty level-$h$ square of color $c_h$.
In order to coordinate between these sub-snakes, we use \emph{interfaces} on the top and bottom boundaries of such squares, that we define next.

  For each non-empty level-$h$ square $Q$ of color $c_h$, let $I_Q$ be the shortest sub-path of the top boundary of $Q^+$ that contains the $3 \cdot N(c_h)$ leftmost  vertices of the top boundary of $Q^+$.
  Similarly, let $J_Q$ be the shortest sub-path of the bottom boundary of $Q^+$ that contains the  $3 \cdot N(c_h)$ rightmost vertices of the bottom boundary of $Q^+$. 
  Notice that $I_Q$ and $J_Q$ are well-defined since $3 \cdot N(c_h) \leq 3 \cdot \ceil {d_h/2\eta^3} \leq d_h$.

  %Recall that $\tilde \chi_{h+1}(c_h)$ is the set of all level-$h+1$ descendants of color $c_h$.
  Let $c_h^1, c_h^2, \ldots, c_h^z$ be the child-colors of $c_h$, indexed in the left-to-right order of their corresponding intervals on $R^*$.
 For a non-empty level-$h$ square $Q$,  let $\set{I^i_Q \subseteq I_Q \> | \> i \in \set{1, \ldots, z}}$ be a collection of disjoint sub-paths of $I_Q$ such that the following holds:
  (i) each sub-path $I^i_Q$ contains $3 \cdot N(c_h^i)$ vertices; and
  (ii) for all $1 \leq i < i' \leq z$, $I_Q^i$ appears to the left of $I_Q^{i'}$ on the top boundary of $Q^+$.
  Similarly, let $\set{J^i_Q \subseteq J_Q \> | \> i \in \set{1, \ldots, z}}$ be an analogous collection of disjoint sub-paths of $J_Q$.
  % such that the following holds:
  %(i) each $J^i_Q$ contains $3 \cdot N(C_h^i)$ vertices; and
  %(ii) for $1 \leq i < i' \leq z$, $J_Q^i$ appears on the left of $J_Q^{i'}$ on the bottom boundary of $Q^+$.
  Notice that there is a unique set of such sub-paths, since $\sum_{i=1}^{z} 3 \cdot N(c_h^i) = 3 \cdot N(c_h)$.
  The sub-paths $I^i_Q$ and $J^i_Q$ will act as interfaces  between the sub-snakes corresponding to color $c_h^i$, and will be used to combine them together.
  Having described the interfaces, we now focus on constructing type-$2$ sub-snakes inside each non-empty square of level $h$.
  We will then construct type-$1$ sub-snakes, and finally combine them all together to obtain level-$(h+1)$ snakes as claimed. 

  \begin{definition}
    Fix a non-empty level-$h$ square $Q$ of color $c_h$, and let $c_h^i$ be a child-color of $c_h$. 
    Given a snake $\hat \yset$, we say that $\hat \yset$ is a \emph{valid type-$2$ sub-snake of color $c_h^i$ in square $Q^+$} iff
  \begin{itemize}
    \item $\hat \yset \subseteq Q^+$;
    \item  $\hat \yset$ has width at least $3 \cdot N(c_h^i)$;
    \item $\hat \yset$ contains $I_Q^i$ as the top boundary of its first corridor and $J_Q^i$ as the bottom boundary of its last corridor; and
    \item for each non-empty level-$(h+1)$ child square $\hat Q$ of $Q$ of color $c_h^i$, $\hat Q^+$ is a corridor of $\hat \yset$.
  \end{itemize}
  \end{definition}

  \begin{claim} \label{clm: construct child snakes inside Q}
    There is an efficient algorithm, that, given a non-empty level-$h$ square $Q$ of color $c_h$ constructs, for every child-color $c_h^i$ of $c_h$, a valid type-$2$ sub-snake $\yset_Q(c_h^i)$ of color $c_h^i$ in square $Q^+$, such that the resulting sub-snakes are pairwise disjoint.    
  \end{claim}

  We prove the above claim after completing the proof of Claim \ref{clm: construct child snakes master}, using the claim. We now turn to construct  type-$1$ sub-snakes.
  We starts with the following simple observation.

  \begin{observation}
    Let $\yset = (\Y_1, \Y_2, \ldots, \Y_r)$ be a snake of width $w$.
    Let $\Sigma_1$ be some boundary edge of $\Y_1$ that is contained in the boundary of $\yset$.
    Similarly, let $\Sigma_r \neq \Sigma_1$ be some boundary edge of $\Y_r$ that is contained in the boundary of $\yset$.
    Let $(A_1, A_2, \ldots A_{j})$ be disjoint sub-paths on $\Sigma_1$ and let $(B_1, B_2, \ldots, B_{j})$ be disjoint sub-paths on $\Sigma_r$ such that the sub-paths $(A_1, \ldots, A_j, B_j, B_{j-1}, \ldots, B_1)$ appear in this clockwise order on the boundary of $\yset$ and $\left| \bigcup_{i=1}^j V(A_i) \right|, \left| \bigcup_{i=1}^j V(B_i) \right| \leq w$.
    Then there is an efficient algorithm to construct pairwise disjoint snakes $\yset_1, \ldots, \yset_{j}$ such that for each $1 \leq i \leq j$, (i) $\yset_i$ is contained in $\yset$; 
    (ii) $A_i$ is contained as a part of the boundary of the first corridor of $\yset_i$;
    (iii) $B_i$ is contained as a part of the boundary of the last corridor of $\yset_i$; and
    (iv) the width of the snake $\yset_i$ is at least $\min{(|A_i|, |B_i|)}$.
  \end{observation}

  Recall that we are given a valid level-$h$ snake $\yset$ for a level-$h$ color $c_h$.
  Also, recall that $\yset$ is a sequence of corridors, containing the squares $Q^+$ corresponding to non-empty level-$h$ color $c_h$ squares $Q$ as corridors.
  Let $Q_1, \ldots, Q_r$ be such squares, in the order of their appearance in $\yset$.
  From the above observation, it is now immediate to find pairwise disjoint sub-snakes $\yset^1(c_h^i), \ldots, \yset^r(c_h^i)$ for each child-color $c_h^i$ of $c_h$ such that:
  \begin{itemize}
    \item the top boundary of the first corridor of $\yset^1(c_h^i)$ contains the interval $I'(c_h^i) \in \iset'_{h+1}$ corresponding to the interval $I(c_h^i) \in \iset_{h+1}$ that was used in defining color $c_h^i$;
    \item for each $2 \leq j \leq r$, the top boundary of the first corridor of $\yset^j(c_h^i)$ contains the interval $J_{Q_{j-1}}^i$;
    \item for each $1 \leq j \leq r$, the bottom boundary of the last corridor of $\yset^j(c_h^i)$ contains the interval $I_{Q_j}^i$;
    and
    \item all the sub-snakes are pairwise disjoint, and are internally disjoint from the squares $Q_1, \ldots, Q_r$.
  \end{itemize}

  For each child color $c_h^i$ of $c_h$, we say that the sub-snakes $\yset^1(c_h^i), \ldots, \yset^{r}(c_h^i)$ are sub-snakes of type $1$.
  Now we focus on combining the snakes of type $1$ and type $2$.

  \begin{definition}
    Let $\yset^1 = (\Y^1_1, \ldots, \Y_{\ell_1}^1)$ and $\yset^2 = (\Y^2_1, \ldots, \Y_{\ell_2}^2)$ be a pair of snakes of width $w_1$ and $w_2$ respectively.
    We say that $\yset_1$ and $\yset_2$ are \emph{composable} iff they are internally disjoint and there are boundary edges $\Sigma^1$ of $\Y_{\ell_1}^1$ and $\Sigma^2$ of $\Y_{1}^2$ such that $|V(\Sigma^1) \cap V(\Sigma^2)| \geq \min{(w_1, w_2)}$.
    We denote by $\yset_1 \oplus \yset_2$ the sequence $(\Y^1_1, \ldots, \Y_{\ell_1}^1, \Y^2_1, \ldots, \Y_{\ell_2}^2)$ of corridors.
  \end{definition}

  We begin with a simple observation that follows directly from the definition of snakes.

  \begin{observation}
    Let $\yset_1$ and $\yset_2$ be a pair of composable snakes, each of width at least $w$.
    Then $\hat \yset = \yset_1 \oplus \yset_2$ is also a snake of width at least $w$.      
  \end{observation}

  Notice that for each child-color $c_h^i$ of $c_h$ and for each $1 \leq j \leq r$, the pair of sub-snakes $\yset^j(c_h^i)$ and $\yset_{Q_j}(c_h^i)$ are composable.
  Similarly, for each $1 \leq j < r$, the pair of sub-snakes $\yset_{Q_j}(c_h^i)$ and $\yset^{j+1}(c_h^i)$ are composable.
  Claim \ref{clm: construct child snakes master} now follows by considering the snakes 
  \[ \yset(c_h^i) = \yset^1(c_h^i) \oplus \yset_{Q_1}(c_h^i) \oplus \yset^2(c_h^i) \oplus \ldots \oplus \yset^r(c_h^i) \oplus \yset_{Q_r}(c_h^i)\]
  for all child-colors $c_h^i$ of $c_h$.
  \end{proof}
  \endproofof

  In the remainder of the section, we prove Claim \ref{clm: construct child snakes inside Q}.


\proofof{Claim \ref{clm: construct child snakes inside Q}}

Recall that we are given a non-empty level-$h$ square $Q$ of color $c_h$.
Let $\dset$ be the set of all non-empty level-$(h+1)$ child squares of $Q$.
Recall that given a pair of intervals $I,I'$ of $[\ell']$, we denoted by $Q(I,I')$ the sub-graph induced by all vertices $\set{v(i,j) \> | \> i \in I, j \in I'}$.
We say that a pair of squares $Q_1, Q_2 \in \dset$ are \emph{vertically aligned} iff $Q_1 = Q(I, I_1)$ and $Q_2 = Q(I, I_2)$ for some intervals $I, I_1, I_2$ of $[\ell']$.
Let $\dset_1, \dset_2, \ldots, \dset_r$ be a partition of $\dset$ such that the following holds:
\begin{itemize}
  \item for each $1 \leq i \leq r$, the squares in $\dset_i$ are vertically aligned; and
  \item for each $1 \leq i < i' \leq r$, all squares in $\dset_i$ appear to the left of those in $\dset_{i'}$.
  \end{itemize}

For each $1 \leq i \leq r$, we denote $\dset_i = (Q_i^1, \ldots, Q_i^{k_i})$, where for each $1 \leq j < j' \leq k_i$, the square $Q_i^j$ appears above $Q_i^{j'}$.

Our goal, as before, is to construct a number of child-snakes\footnote{As in the case of sub-snakes, each of the child-snake that we construct, is a snake as defined earlier. We use the term `child-snake' to distinguish them from the final combined sub-snake $\yset_Q(c_h^i)$ that we construct.}
 for each child-color $c_h^i$ of $c_h$, which can be combined together to obtain the desired sub-snake $\yset_Q(c_h^i)$.
To this end, we need interfaces, which we define next.


For each child-square $\hat Q \in \dset$ of $Q$, let $R(\hat Q^+)$ and $R'(\hat Q^+)$ be the rows containing the top and bottom boundaries of $\hat Q^+$ respectively.
Let $\alpha(\hat Q)$ be the sub-path containing all nodes of the top boundary of $\hat Q^+$ along with $3 \cdot N(c_h)$ nodes of $R(\hat Q^+)$ lying immediately to the left and $3 \cdot N(c_h)$ nodes of $R(\hat Q^+)$ lying immediately to the right of the top boundary of $\hat Q^+$.
Similarly, define $\beta(\hat Q)$ analogously for the bottom boundary of $\hat Q^+$.
We say that the vertices in paths $\alpha(\hat Q)$ and $\beta(\hat Q)$ are the \emph{portals} of $\hat Q$.
Let $\set{\alpha_i(\hat Q) \subseteq \alpha(\hat Q) \> | \> i \in \set{1, \ldots, z}}$ be a set of disjoint intervals in the natural left-to-right ordering with following two properties:
(i) there are at least $3 \cdot N(c_i)$ nodes in the interval $\alpha_i(\hat Q)$; and
(ii) if the square $\hat Q$ is assigned level-$(h+1)$ color $c_h^i$, then $\alpha_i(\hat Q)$ is the top boundary of $\hat Q^+$.
We define the intervals $\beta_i(\hat Q) \subseteq \beta(\hat Q)$ corresponding to the bottom boundary of $\hat Q^+$ for each $1 \leq i \leq z$ in a similar fashion.
The sub-paths $\alpha_i(\hat Q)$ and $\beta_i(\hat Q)$ will act as interfaces to connect child-snakes corresponding to color $c_h^i$.
Now, we focus on constructing the child-snakes inside $Q^+$.

Notice that $N_h(c_h) \leq \ceil{d_h/2\eta^3} < d_h/\eta^3 \leq d_{h+1}/18$, since $\eta \geq 3$.
Recall that for each pair $\hat Q, \tilde Q \in \dset$ of distinct level-$(h+1)$ squares contained inside $Q$, $d(\hat Q^+,\tilde Q^+), d(\hat Q^+, \Gamma(Q^+)), d(\tilde Q^+, \Gamma(Q^+)) \geq d_{h+1}/2 > 9 \cdot N(c_h)$.
Hence, portals of any pair of distinct squares are separated by at least $3 \cdot N(c_h)$ nodes from each other.
Exploiting this spacing, it is now immediate to construct the child-snakes of the following five types (see Figure \ref{fig: q and children} for illustration).

\begin{itemize}
  \item The set of child-snakes of type $A$ contains, for each child-color $c_h^i$ of $c_h$, a single snake $\yset^A(c_h^i)$ of width $3 \cdot N(c_h^i)$ with $I_Q^i$ as the top boundary of its first corridor and $\alpha(Q^1_1)$ as the bottom boundary of its last corridor.

  \item The set of child-snakes of type $B$ contains, for each child-color $c_h^i$ of $c_h$, a single snake $\yset^B(c_h^i)$ of width $3 \cdot N(c_h^i)$ with $\beta_i(Q_r^{k_r})$ as the top boundary of its first corridor and $J_Q^i$ as the bottom boundary of its last corridor.
 
  \item The set of child-snakes of type $C$ contains, for each child-color $c_h^i$ of $c_h$,  for each $1 \leq j \leq r$ and $1 \leq j' < k_j$, a snake $\yset_j^{j'}(c_h^i)$ of width $3 \cdot N(c_h^i)$ with $\beta_i(Q_j^{j'})$ as the top boundary of its first corridor and $\alpha(Q_j^{j'+1})$ as the bottom boundary of its last corridor.
  \item The child-snakes of type $D$ consists of, for each child color $c_h^i$ of $c_h$ and $1 \leq j < r$, a snake $\yset_j^{k_j}(c_h^i)$ of width $3 \cdot N(c_h^i)$ with $\beta_i(Q_j^{k_j})$ as the top boundary of its first corridor and $\alpha_i(Q_{j+1}^{1})$ as the bottom boundary of its last corridor.

  \item The child-snakes of type $E$ consists of, for each child-color $c_h^i$ of $c_h$ and square $Q_j^{j'} \in \dset$, a snake $\hat \yset_j^{j'}(c_h^i)$ of width $3 \cdot N(c_h^i)$ with $\alpha_i(Q_j^{j'})$ as the top boundary of its first corridor and $\beta_i(Q_j^{j'})$ as the bottom boundary of its last corridor.
  Moreover, if the level-$(h+1)$ color of $Q_j^{j'}$ is $c_h^i$, then $\hat \yset_j^{j'}(c_h^i)$ is a snake contains the corresponding extended square $Q_j^{j'+}$ as a corridor.
\end{itemize}


Moreover, we also ensure that the child-snakes corresponding to different colors $c_h^i$ are disjoint, and for each child color $c_h^i$ the snakes are composable.
 Claim \ref{clm: construct child snakes inside Q} now follows by considering the snakes 
  \[ \yset_Q(c_h^i) = \yset^A(c_h^i) \oplus \hat \yset_1^1(c_h^i) \oplus \yset_1^1(c_h^i) \oplus \hat \yset_1^2(c_h^i) \oplus \yset_1^2(c_h^i) \oplus \ldots \oplus \yset_{r}^{k_r-1}(c_h^i) \oplus \hat \yset_r^{k_r}(c_h^i) \oplus \yset^B(c^i_{h})\]
  for all child-colors $c^i_h $ of $c_h$.
\end{proofof}


\begin{figure}[h]
\center
\scalebox{0.26}{\includegraphics{snakes-in-q}}
\caption{Squares $Q_1, Q_2, Q_3, Q_4$ are children of level $h$ square $Q$ of color $c_h$.
We label them in this way for simplicity. Here, $Q_1$ and $Q_2$, as well as $Q_3$ and $Q_4$ are vertically aligned.
%Squares $Q_1^+, Q_2^+, Q_3^+, Q_4^+, Q^+$ are their respective extended squares.
The width of the snake responsible to route $N(c_h)$ demand pairs, containing $Q^+$ as a corridor, is $3N(c_h)$.
The figure shows the corridors of snakes corresponding to the child-colors of $c_h$ inside square $Q^+$.
\label{fig: q and children}}
\end{figure}

==> arxiv final/sources-at-distance-d.tex <==
\section{Approximation Algorithm for the Special Case with Sources Close to the Grid Boundary} \label{sec: sources at dist d}
The goal of this section is to prove Theorem~\ref{thm: sources at dist d}. We assume that we are given an instance $(G,\mset)$ of \NDPgrid and an integer $\delta>0$, such that every source vertex is at a distance at most $\delta$ from the grid boundary. Our goal is to design an efficient randomized factor-$(\delta \cdot \approxfactor)$-approximation algorithm for this special case of the problem. We can assume that $\delta<n^{1/4}$, as there is an $\tilde{O}(n^{1/4})$-approximation algorithm for \NDPgrid~\cite{NDP-grids}. For every source vertex $s\in S(\mset)$, let $\tilde s$ be the vertex lying closest to $s$ on $\Gamma(G)$; for every destination vertex $t\in T(\mset)$, let $\tilde t$ be defined similarly. Recall that for each $s\in S(\mset)$, $d(s,\tilde s)\leq \delta$.
For every subset $\mset'\subseteq \mset$ of the demand pairs, we denote $\tilde S(\mset')=\set{\tilde s\mid s\in S(\mset')}$, and similarly $\tilde T(\mset')=\set{\tilde t\mid t\in T(\mset')}$.
 Using the same arguments as in Section~\ref{sec:destinations anywhere}, at the cost of losing an $O(\log n)$-factor in the approximation ratio, we can assume that all vertices of $\tilde S(\mset)$ are contained in a single boundary edge of the grid $G$, that we denote by $\Gamma$, and that  all vertices of $\tilde T(\mset)$ are contained in a single boundary edge of the grid $G$, that we denote by $\Gamma'$, where possibly $\Gamma=\Gamma'$. Moreover, we can assume that there is some integer $d$, such that for all $t\in T(\mset)$, $d\leq d(t,\tilde t)<2d$.

Let $c$ be a sufficiently large constant. Assume first that $d\leq \delta\cdot 2^{c\sqrt{\log n}\log\log n}$. In this case, we can obtain an $(\delta\cdot\approxfactor)$-approximation using the following claim.

\begin{claim} \label{claim: close pairs}
There is an efficient algorithm to compute a factor $(\delta\cdot\approxfactor)$-approximation for the special case where $d \leq \delta\cdot 2^{c\sqrt{\log n}\log\log n}$.
\end{claim}

\begin{proof}
Let $\hat \mset=\set{(\tilde s,\tilde t)\mid (s,t)\in \mset}$ be a new set of demand pairs. Note that all vertices participating in the demand pairs in $\hat \mset$ lie on the boundary of $G$. Therefore, we can efficiently find an optimal solution to the \NDP problem instance $(G,\hat \mset)$ using standard dynamic programming.  Next, we show that $\opt(G,\hat \mset)=\Omega(\opt(G,\mset)/(\delta\cdot\approxfactor))$. For every vertex $v\in S(\mset)\cup T(\mset)$, let $U_v$ be the shortest path connecting $v$ to $\tilde v$.

Let $\pset^*$ be the optimal solution to instance $(G,\mset)$, and let $\mset^*\subseteq \mset$ be the set of the demand pairs routed by $\pset^*$. For each demand pair $(s,t)\in \mset^*$, let $P(s,t)\in \pset^*$ be the path routing it. %For each source vertex $v\in S(\mset')\cup T(\mset')$, let $U_s$ be the shortest path from $v$ to $\tilde v$ in $G$. Note that $U_v$ contains at most $65\delta$ vertices, and we can assume w.l.o.g. that it is a sub-path of a single column or a single row of $G$.

We construct a directed graph $H$, whose vertex set is $V(H)=\set{v(s,t)\mid (s,t)\in \mset^*}$, and there is a directed edge from $v(s,t)$ to $v(s',t')$ iff the path $P(s',t')$ routing the pair $(s',t')$ in the optimal solution $\pset^*$ contains a vertex of $U_s\cup U_t$. It is easy to verify that the out-degree of every vertex of $H$ is at most $d+\delta$, and so there is an independent set $I$ in $H$ containing at least $\Omega(|V(H)|/(d+\delta))=\Omega(\opt(G,\mset)/(\delta\cdot\approxfactor))$ vertices of $I$. 

For each demand pair $(s,t)\in \mset^*$ with $v(s,t)\in I$, let $P'(s,t)$ be the concatenation of $U_s$, $P(s,t)$ and $U_t$. Then $\set{P'(s,t)\mid v(s,t)\in I}$ is a collection of $\Omega(\opt(G,\mset)/(\delta\cdot\approxfactor))$ node-disjoint paths routing demand pairs in $\hmset$. We conclude that  $\opt(G,\hat \mset)=\Omega(\opt(G,\mset)/(\delta\cdot\approxfactor))$. 

Let $\pset'$ be a solution to instance $(G,\hat \mset)$, obtained by the constant-factor approximation algorithm, so $|\pset'|=\Omega(\opt(G,\mset)/(\delta\cdot\approxfactor))$, and let $\hmset'\subseteq \hmset$ be the set of the demand pairs routed. Since all source and all destination  of $\hmset'$ appear on the boundary of $G$, $|\hmset'|=O(\sqrt n)$. Moreover, the demand pairs in $\hmset'$ must be non-crossing: that is, for every pair $(s,t),(s',t')\in \hmset'$, the circular ordering of the corresponding terminals on the boundary of the grid is either $(s,s',t',t)$ or $(s,t,t',s')$. Since we have assumed that $\delta\leq n^{1/4}$  and $d\leq \delta\cdot 2^{c\cdot\sqrt{\log n}\log\log n}$, it is easy to verify that we can route $|\Omega(\hmset')|$ demand pairs from the original set $\mset$, that correspond to the demand pairs in $\hmset'$.

\end{proof}


From now on we assume that $d> \delta\cdot 2^{c\sqrt{\log n}\log\log n}$. 
Next, we define a new set $\tmset$ of demand pairs, as follows: $\tmset=\set{(\tilde s,t)\mid (s,t)\in \mset}$, so all source vertices of the demand pairs in $\tmset$ lie on the boundary edge $\Gamma$ of $G$. Let $\opt'$ be the value of the optimal solution to problem $(G,\tmset)$. The proof of the following claim is  almost identical to the proof of Claim~\ref{claim: close pairs} and is omitted here.

\begin{claim}
$\opt'\geq \Omega( \opt(G,\mset)/\delta)$.
\end{claim}



From now on we focus on instance $(G,\tmset)$ of \restrictedNDP. Recall that for each source vertex $s\in S(\mset)$, we denoted by $U_s$ the shortest path connecting $s$ to $\tilde s$. We say that a path $P$ routing a demand pair $(\tilde s,t)\in \tmset$ is \emph{canonical} iff $U_s\subseteq P$. We say that set $\pset$ of node-disjoint paths routing demand pairs in $\tmset$ is canonical iff every path in $\pset$ is canonical. We will show that we can apply our $\approxfactor$-approximation algorithm to instance $(G,\tmset)$ to obtain a routing in which all paths are canonical. 
For convenience, we assume w.l.o.g. that $\Gamma$ is the top boundary edge of the grid. Therefore, a canonical path connecting a demand pair $(\tilde s,t)\in \tmset$ must follow the column $\col(\tilde s)$ of $G$ until it reaches the vertex $s$.

Assume first that $d>\opt'/\eta$, where $\eta$ is defined as before. Then we obtain a special case of the problem where the destination vertices are sufficiently far from the boundary of the grid, and can use the algorithm from Theorem~\ref{thm: main w destinations far from boundary} to find a $\approxfactor$-approximate solution to instance $(G,\tmset)$.
%Let $\mset^* \subseteq \tmset$ be the set of demand pairs routed.
%If $\delta > |\mset^*|$, then we can route a single demand pair and still obtain $O(\delta \cdot \approxfactor)$-approximate solution.
%From now on, we assume that $\delta \leq |\mset^*|$.
%But from Observation \ref{obs: paths go straight down}, the paths in our solution are canonical.
%
However, we slightly modify the routing to ensure that the paths in our solution are canonical. Recall that the routing itself is recursive. Let $\qset_1$ be the set of all level-$1$ squares, and let $\qset_1'\subseteq\qset_1$ be the set of all non-empty level-$1$ squares. Recall that each square $Q\in \qset_1$ has size $(d_1\times d_1)$, where $d_1\leq \opt'/2^{c^*\sqrt{\log n}\log\log n}$. For each square $Q\in \qset_1'$, we have created an extended square $Q^+$, by adding a margin of size $d_1/\eta$ around $Q$. At the highest level of the recursion, the paths depart from the source vertices of the demand pairs we have chosen to route, and then visit the squares in $\set{Q^+\mid Q\in \qset_1'}$ one-by-one, in a snake-like fashion, entering and leaving each such square $Q^+$ on a pre-selected set of vertices. Recall that we have assumed that $d>\delta\cdot 2^{c\sqrt{\log n}\log\log n}$, and $d>\opt'/\eta$.  Then it is easy to see that the top $d/2\gg \delta$ rows of $G$ are disjoint from the squares of $\qset_1'$, each of which must contain a destination vertex. As the algorithm routes at most $d_1$ paths, this routing can be accomplished via canonical paths. The recursively defined routing inside the level-$1$ squares remains unchanged.


%Notice that at the cost of losing a factor $4$ in the approximation ratio, we can assume that all source vertices of the demand pairs in $\tmset$ lie on a single boundary edge of the grid -- we assume w.l.o.g. that it is the top boundary. Let $\opt$ be the value of the optimal solution to the problem. %Since our goal is to obtain a $\delta\cdot \approxfactor$-approximation, we can assume w.l.o.g. that $\delta<\opt/2^{c\sqrt{\log n}\log\log n}$ for a large enough constant $c$, as otherwise routing a single demand pair is sufficient.

%We consider first the special case of the problem handled by Theorem~\ref{thm: main w destinations far from boundary}, where we are given a lower bound $\opt$ on the value of the optimal solution, and every destination vertex lies at a distance at least $\opt/\eta$ from the boundary of the grid. Once the demand pairs to be routed are selected by the algorithm, a level-$0$ square $Q_0$ is defined. This square excludes the top $d_1\geq \opt/(\eta\cdot 2^{c^*\sqrt{\log n}\log\log n})\geq 2\delta$ rows of the grid. Eventually, the source vertices of the selected demand pairs need to be routed to the pre-selected vertices on the top boundary of the grid $Q_0$. Since at most $d_1$ demand pairs are selected to be routed, it is easy to verify that the top $d_1$ rows of $G$ provide sufficient space to perform this routing, while ensuring that the resulting paths are canonical.

%We now turn to the algorithm for the general case. 

From now on, we assume that $d<\opt'/\eta$, and we now follow the algorithm from Section~\ref{sec:destinations anywhere}.
%Recall that by losing a logarithmic factor in the approximation ratio, we can assume that we are  given some integer $d$, such that for each demand pair $(\tilde s,t)$, $d\leq d(t,\tilde t) <2d$. As before, if $d>\opt/\eta$, then we obtain the special case of the problem that is dealt with by Theorem~\ref{thm: main w destinations far from boundary}, as described above. We assume from now on that $d<\opt/\eta$. 

As before, we consider  three sub-cases. Recall that $\Gamma'$ is the boundary edge of $G$ containing the vertices of $\tilde T(\tmset)$.
In the first sub-case, $\Gamma'$ is the the bottom boundary of the grid. The algorithm constructs a number of square grids of height less than $\ell/2$, whose bottom boundaries are contained in the bottom boundary of the grid $G$. Each such sub-grid defines a modified instance, that is solved separately. Eventually, we need to connect the source vertices of the routed demand pairs to their counterparts in the modified instances. As the top $\ell/2$ rows of $G$ are disjoint from the modified instances, it is easy to see that this can be done via paths that are canonical.

The second sub-case is when $\Gamma'$ is either the left or the right boundary edge of $G$; assume w.l.o.g. that it is the left boundary edge. In this case, we have discarded the demand pairs whose destinations lie in the top $\opt'/16$ rows of the grid $G$. As before, we then define a  collection of modified instances, each of which is defined over a square sub-grid of $G$ of width less than $\ell/2$. The left boundary of each sub-grid is contained in the left boundary of $G$, and each such sub-grid is disjoint from the top $\opt'/16$ rows of $G$. As before, we need to connect the source vertices of the demand pairs routed in the modified sub-instances to their counterparts. In order to do so, we utilize the top $\opt'/16$ rows and the rightmost $\ell/2$ columns of $G$.
This provides sufficient space to perform the routing via canonical paths, as $\delta\ll d<\opt'/\eta$.
%Indeed, if it is not the case, then we can route a single demand pair and still obtain $O(\delta)$-approximation.

The final sub-case is when $\Gamma'=\Gamma$.  This case is in turn partitioned into two sub-cases. The first sub-case is when a large number of the demand pairs routed by the optimal solution belong to the set $\mset^0$: the set of all demand pairs $(s,t)$ with $|\col(s)-\col(t)|\leq 2d$.  In this case, we defined a collection of disjoint sub-grids of $G$, of size $(\Theta(d)\times \Theta(d))$, reducing the problem to a number of disjoint sub-instances that are dealt with using Theorem~\ref{thm: main w destinations far from boundary}. In each such sub-instance, we can ensure that the routing is canonical as before, since the value of the optimal solution in each sub-instance is $O(d)$, and $\delta \ll d$. In the second sub-case, we partition the grid $G$ into a number of sub-instances, where each sub-instance is defined by a pair of consecutive vertical strips of $G$. One of the two strips contains all source vertices, and the other all destination vertices of the resulting sub-instance. We then define a modified instance inside the strip containing the destinations, and route the source vertices to the corresponding sources of the routed modified demand pairs. This routing utilizes the vertical strip containing the sources, and the bottom half of the vertical strip containing the destinations. As before, it is easy to ensure that this routing is canonical.






\iffalse
We note that improving the dependency on $\delta$ to $\sqrt{\delta}$ would enable us to recover the algorithm of Chuzhoy and Kim \cite{NDP-grids} for \NDPgrid up to the same factor. 
We begin with the following lemma that modifies a given set of node-disjoint paths connecting some demand pairs, to avoid certain \emph{forbidden vertices}.

\begin{lemma} \label{lem: bypass forbidden vertices}
	Let $(G, \mset)$ be an instance of \NDPgrid problem.
	For each demand pair $(s_i, t_i) \in \mset$, let $Z_i \subseteq V(G)$ be a set of \emph{forbidden vertices}.
	For a subset $\mset' \subseteq \mset$ of demand pairs, let $\pset'$ be a given set of paths routing them in $G$.
	For each demand pair $(s_i, t_i) \in \mset'$, let $P_i \in \pset'$ be the path routing it.
	We let $\gamma := \max_{(s_i, t_i) \in \mset'}{|Z_i|}$.
	Then there is an efficient algorithm to obtain a subset $\mset'' \subseteq \mset'$ of demand pairs and the subset $\pset'' \subseteq \pset'$ of paths such that
	(i) $\forall (s_i, t_i), (s_j, t_j) \in \mset''$, $Z_i \cap V(P_j) = \emptyset$; and
	(ii) $|\mset''| \geq \Omega(|\mset'|/\gamma)$.
\end{lemma}

\begin{proof}
	We construct a directed graph $H$, whose vertex set is $\set{v(P) \> | \> P \in \pset'}$.
	We add an edge between $v(P_i)$ and $v(P_j)$ iff $Z_i \cap V(P_j) \neq \emptyset$.
	It is immediate to verify that the maximum in-degree of any vertex in $H$ is $\gamma$.
	Therefore, a simple greedy algorithm gives us a set $U \subseteq V(H)$ of $\Omega(|V(H)|/\gamma)$ vertices, such that no two vertices of $U$ are connected by an edge.
	We let $\pset'' = \set{P \> | \> v(P) \in U}$ be the subset of paths we pick and let $\mset''$ be the corresponding subset of demand pairs.
	It is now immediate to verify that the properties (i) and (ii) of the lemma holds.
\end{proof}


\proofof{Theorem \ref{thm: sources at dist d}}
	We will prove the theorem in three steps.
	First, we will construct an instance $\hat I$ of \restrictedNDP by relocating the sources of $\mset$ to some suitably chosen vertex on the grid boundary, such that $\opt(\hat I) = \Omega(\opt(I)/\delta)$.
	Next, we will apply the algorithm of Theorem \ref{thm: main} on $\hat I$ to obtain a set of node-disjoint paths routing $\opt(I)/\approxfactor$ demand pairs.
	We will then exploit it to obtain a set of node-disjoint paths in $I$ to route at least $\opt(I)/(\approxfactor \cdot \delta^2)$ demand pairs.
	
	%\paragraph{Constructing $\hat I$}
	For each source $s \in S(\mset)$, let $\hat s \in \Gamma(G)$ be a vertex minimizing $d(s, \hat s)$ breaking ties arbitrarily.
	We let $\hat \mset = \set{(\hat s, t) \> | \> (s,t) \in \mset}$.
	Our instance is now simply $\hat I = (G, \hat \mset)$.
	For convenience, given any two nodes $(u,v)$ of $G$, we let $L(u,v)$ be a  shortest path connecting $u$ and $v$ in $G$.
	\begin{claim} \label{clm: opt within factor delta}
		$\opt(\hat I) = \Omega(\opt(I)/ \delta)$
	\end{claim}	
	
	
	
	\begin{proof}
		Let $\pset^*$ be the optimum set of node-disjoint paths routing a subset $\mset^* \subseteq \mset$ of $|\opt(I)|$ demand pairs.
		For each source $s \in S(\mset^*)$, we set $Z_s = V(L(s,\hat s))$.
		Notice that for each $s \in S(\mset^*)$, $|Z_s| \leq \delta + 1$.
		From Lemma \ref{lem: bypass forbidden vertices}, we obtain a subset $\tilde \mset \subseteq \mset^*$ of $\Omega(|\mset^*| / \delta)$ demand pairs and a subset $\tilde \pset \subseteq \pset^*$ of node-disjoint paths routing them. 
		For each demand pair $(s,t) \in \tilde \mset$, we augment the path $L(s, \hat s)$ to the corresponding path in $\tilde \pset$.
		Let $\pset'$ be the set of paths thus obtained.
		From the guarantee of Lemma \ref{lem: bypass forbidden vertices}, it is immediate to see that $\pset'$ is a node-disjoint set of paths routing $|\tilde \mset| = \Omega(|\opt(I)|/\delta)$ demand pairs of $\hat \mset$.
	\end{proof}


Notice that $\hat I$ is a instance of \restrictedNDP problem.
From Theorem \ref{thm: main}, we have an efficient algorithm routing $\Omega(|\opt(\hat I)| / \approxfactor)$ demand pairs of $\hat I$.
Let $\tilde \mset$ be a set of such demand pairs and $\tilde \pset$ be a set of node-disjoint paths routing them.
We can now employ the same arguments as in the proof of Claim \ref{clm: opt within factor delta} to obtain a set $\pset'$ of demand pairs routing 
\[\frac{|\tilde \mset|}{\delta} = \Omega \left(\frac{|\opt(\hat I)|}{\approxfactor \cdot \delta} \right)  = \Omega \left(\frac{|\opt(I)|}{\approxfactor \cdot \delta^2} \right)\]
demand pairs, completing the proof.
\endproofof

\fi

==> hard-example.tex <==
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
%-------------------------------------------------------------------------
\label{------------------------------------sec: hard example--------------------------------------}

\section{Negative Example for the Distance Property} \label{sec: hard-example}
We say that an instance $(G,\mset)$ of \NDPgrid is \emph{perfectly routable} iff there is a set $\pset$ of node-disjoint paths in $G$, routing all demand pairs in $\mset$.

Assume now that we are given some instance $(G,\mset)$ of \NDPgrid, where all vertices of $S(\mset)$ lie on the top boundary of the grid $G$, and let $\mset' \subseteq \mset$ be any subset of the demand pairs, whose sources are all distinct.
For any two sources $s, s' \in S(\mset')$, let $N_{\mset'}(s,s')$ be the number of all sources in $S(\mset')$ lying between $s$ and $s'$ on the top boundary of $G$.
Recall that we say that $\mset'$ has the $1$-distance property iff for each $(s,t), (s',t') \in \mset'$, $N_{\mset'}(s,s')  \leq d(t,t')$.
For convenience, in the remainder of this section, we refer to the $1$-distance property simply as the \emph{distance property}.

The goal of this section is to construct a family of perfectly routable instances  $(G,\mset)$ of \NDPgrid, with sources lying on the top boundary of the grid, such that every subset $\mset'\subseteq \mset$ of the demand pairs, if $\mset'$ has the distance property, then $|\mset'|\leq |\mset|/2^{\Omega(\sqrt{\log n})}$, where $n=|V(G)|$.
More precisely, we prove the following theorem.

\begin{theorem} \label{thm: main hard}
For each sufficiently large integer $n$, there is a perfectly routable instance $(G,\mset)$ of \rNDPgrid, where $G$ is an $(n^{\Theta(1)}\times n^{\Theta(1)})$-grid, all source vertices in $S(\mset)$ lie on the top boundary of $G$, and for every subset $\mset' \subseteq \mset$ of the demand pairs that has the distance property, $|\mset'|\leq |\mset| / 2^{\Omega(\sqrt{\log n})}$.
\end{theorem}

We note that in the instances that we construct, the destination vertices may lie close to the grid boundaries; however, adding a padding of $\sqrt n$ columns on either side of the grid, and possibly additional rows at the bottom of the grid, rectifies this problem without affecting the final result.

We use a parameter $g=1.1$. Our construction is iterative. In iteration $i$, we construct a level-$i$ instance $(G_i,\mset_i)$; the instance is perfectly routable and has all vertices of $S(\mset_i)$ lying on the top boundary of $G_i$.  We denote the dimensions of the grid $G_i$ by $\ell_i$ (so $G_i$ is the $(\ell_i\times \ell_i)$-grid), and we denote $|\mset_i|=N_i$. We will ensure that the largest subset of the demand pairs in $\mset_i$ that has the distance property has cardinality at most $N_i/g^i$. We now set the parameters $\ell_i$ and $N_i$. Let $\gamma_i=20g^{2i}$. We then set $N_0=1$, and for all $i\geq 1$, $N_i=2\gamma_{i-1}N_{i-1}$. A simple calculation shows that $N_i=2^{\Theta(i^2)}$. We also set $\ell_i=9N_ig^i=2^{\Theta(i^2)}$. It is now enough to prove the following theorem.



\begin{theorem}\label{thm: iterations}
For every integer $i\geq 0$, there is an instance $(G_i,\mset_i)$ of \rNDPgrid, such that:

\begin{itemize}
\item $G_i$ is the $(\ell_i\times \ell_i)$ grid, $|\mset_i|=N_i$; 
\item all source vertices of $\mset_i$ lie on the top boundary of $G_i$;
\item instance $(G_i,\mset_i)$ is perfectly routable; and
\item for every subset $\mset'_i\subseteq \mset_i$ of demand pairs that has the distance property, $|\mset'_i|\leq N_i/g^i$.
\end{itemize}
\end{theorem}

Indeed, suppose we are given a large enough parameter $n$. We set $\rho=\ceil{\sqrt{\log n}}$, and consider the level-$\rho$ instance $(G_{\rho},\mset_{\rho})$. Then $G_{\rho}$ is the $(\ell_{\rho}\times \ell_{\rho})$ grid, where $\ell_{\rho}=n^{\Theta(1)}$, and the instance $(G_{\rho},\mset_{\rho})$ is perfectly routable, with all source vertices lying on the top row of $G_{\rho}$. Moreover, if $\mset'\subseteq \mset_{\rho}$ has the distance property, then $|\mset'|\leq |\mset_{\rho}|/g^{\rho}=|\mset_{\rho}|/2^{\Omega(\sqrt{\log n})}$. In the remainder of this section we prove Theorem~\ref{thm: iterations}.



\begin{figure}[h]
\scalebox{0.18}{\includegraphics{level0}}
\caption{Level-$0$ instance \label{fig: level0}}
\end{figure}

\begin{figure}[h]
\scalebox{0.4}{\includegraphics{flip}}
\caption{Flipping a level-$i$ instance \label{fig: flip}}
\end{figure}


\iffalse
\begin{figure}[h]
%\centering
\hspace{1cm}
\subfigure[Level-$0$ instance]{\scalebox{0.18}{\includegraphics{level0}}\label{fig: level0}}
\hspace{2cm}
\subfigure[Flipping a level-$i$ instance]{
\scalebox{0.4}{\includegraphics{flip}}\label{fig: flip}}
\caption{
  Illustration to the proof of Theorem~\ref{thm: iterations}.
  \label{fig: routing-spaced}}
\end{figure}
\fi

\iffalse

We set a parameter $g = 0.9$.
For some sufficiently large parameter $\rho$, let $N=2^{\Omega(\rho^2)}$.
We will construct a $\sqrt{N} \times \sqrt{N}$ grid $G$ with a set $\mset$ of $\Omega(\sqrt{N})$ demand pairs.
We will place all the sources on the top boundary and all the destinations on a single row of $G$.
We will ensure that all the demand pairs in $\mset$ can be routed via node-disjoint paths, but on the other hand, no subset of more than $g^\rho \cdot |\mset| = |\mset|/2^{\Omega(\sqrt{\log N})}$ of demand pairs has distance property.


The idea is to construct the instance in a hierarchical fashion, in a sequence of steps, which we call \textit{levels}.
There are $\rho$ levels, in total.
For each $0 \leq i \leq \rho$, the level-$i$ instance $I_i = (G_i, \mset_i)$ is a $\ell_i \times \ell_i$ grid $G_i$ with $|\mset_i| = N_i$ demand pairs.
We say that the instance $I_i$ is \emph{perfect} iff
(i) it is routable;
(ii) all sources $S(\mset_i)$ lie on the top boundary of $G_i$; and
(iii) no subset of $N'_i > g^i N_i$ demand pairs of $\mset_i$ has distance property.
For each level $0 \leq i \leq \rho$, we set a parameter $\gamma_i = 20/g^{2i}$.


\begin{theorem} \label{thm: induct hard}
  For each $0 \leq i \leq \rho$, there is a \textit{perfect} level-$i$ instance $I_i = (G_i, \mset_i)$ with the following properties:
  \begin{itemize}
    \item $N_0 = 1$ and for all other $0 < i \leq \rho$, $N_i = 2 \gamma_{i-1}N_{i-1}$
    \item $\ell_i = 9 \cdot N_i/g^i$
  \end{itemize}
\end{theorem}

Before proving the theorem, let us complete the proof of Theorem \ref{thm: main hard} using it.

\proofof{Theorem \ref{thm: main hard}}
Consider level-$\rho$ instance $I_{\rho}=(G_\rho, \mset_\rho)$.
The number of demand pairs:
\[ N_\rho = N_0 \cdot \prod_{i=1}^{\rho} 2\gamma_{i-1}  \leq \gamma_\rho ^ {O(\rho)} \leq g^{-O(\rho^2)}\]
The size of the grid is $\ell_\rho \times \ell_\rho$ where $\ell_\rho = O(N_\rho / g^\rho) \leq g^{-O(\rho^2)}$.
In other words, $n = g^{-O(\rho^2)}$.
Thus, the final gap we achieve is $N'_\rho/N_\rho < g^\rho = 2^{-\Theta(\rho)} = 2^{-\Omega(\sqrt{\log n})}$.
\endproofof

Notice that in the instance that we construct, the sources are quite close to the grid boundary.
This is not a problem, since we can pad $G_\rho$ by $\ell_\rho$ columns on left and right sides and $2 \ell_\rho$ rows on the bottom.
In the new \emph{routable} instance obtained, all the destination nodes are at distance $\Omega(\ell_\rho)$ from the grid boundaries.
In the remainder of the section, we prove Theorem \ref{thm: induct hard}.

%-------------------------------------
%-------------------------------------
%-------------------------------------
%-------------------------------------
\fi



\proofof{Theorem \ref{thm: iterations}}
The proof is by induction on $i$.
The base case is when $i=0$.
The level-$0$ instance, $(G_0, \mset_0)$, is defined as follows. Notice that from our setting of the parameters, $N_0=1$ and $\ell_0=9$. Graph $G_0$ is the $(9 \times 9)$ grid, and $\mset_0$ consists of a single demand pair $(s_0, t_0)$, with both $s_0$ and $t_0$ lying on the first column of the grid, with $s_0$ lying on its first row and $t_0$ on its $5$th row (see Figure \ref{fig: level0}).
It is immediate to see that this instance has all required properties.
 
We now assume that the theorem holds for some integer $i\geq 0$, and prove it for $(i+1)$. We let $G_{i+1}$ be the $(\ell_{i+1}\times \ell_{i+1})$-grid. In order to define the set $\mset_{i+1}$ of demand pairs, we carefully combine $2\gamma_i$ copies of level-$i$ instances. Each such copy will be mapped to a square sub-grid of $G_{i+1}$, with the different copies being horizontally aligned, and lying roughly midway between the top and the bottom rows of $G_{i+1}$. For convenience, we denote $\gamma_i$ by $\gamma$ from now on.



Let $R^*$ be the top row of the grid $G_{i+1}$, and let $R'$ be the row appearing at distance exactly $\gamma N_i$ from the bottom row of $G_{i+1}$. Let $\rset$ be the set of $\ell_i$ consecutive rows of $G_{i+1}$, such that $R'$ is the last row in $\rset$. Consider the horizontal strip $S$ of $G_{i+1}$ spanned by the rows in $\rset$. Next, we define $2\gamma_i$ square $(\ell_i\times \ell_i)$ sub-grids of $S$, to which the copies of the level-$i$ instances will be mapped. The sub-grids are denoted by $A_1,A_2, \ldots,A_{2\gamma}$. We place these sub-grids side-by-side in this left-to-right order inside $S$, so that the left boundary of $A_1$ is at a  distance at least $\gamma N_i$ from the left boundary of $G_{i+1}$ (see Figure~\ref{fig: leveli}). Since:

\[\ell_{i+1}=9N_{i+1}g^{i+1}=18\gamma N_i g^{i+1} \geq (2\gamma)\cdot \ell_i + \gamma N_i,\]

there is enough horizontal space to find such a placement.

For each $1\leq j\leq 2\gamma$, where $j$ is an even integer, we view $A_j$ as a copy of the level-$i$ instance $(G_i,\mset_i)$. In other words, we map the vertices and the edges of $G_i$ to the vertices and the edges $A_j$ in the natural manner. This mapping defines a set $\nset_j$ of pairs of vertices of $A_j$, that correspond to the demand pairs in $\mset_i$.

Similarly, for each $1\leq j\leq 2\gamma$, where $j$ is an odd integer, we view $A_j$ as a copy of the level-$i$ instance $(G_i,\mset_i)$, except that now the instance is {\bf flipped}: when we map $G_i$ to $A_j$, we reverse the order of its rows (so they now appear from bottom to top), and the order of its columns (so they now appear from right to left); in particular, all source vertices of $S(\mset_i)$ appear on the bottom boundary of $A_j$ (see Figure~\ref{fig: flip}). This mapping again defines a set $\nset_j$ of pairs of vertices of $A_j$, that correspond to the demand pairs in $\mset_i$.

We are now ready to define the set $\mset_{i+1}$ of the demand pairs of our level-$(i+1)$ instance. This set is a union of $2\gamma$ disjoint subsets, $\nset_1',\ldots,\nset_{2\gamma}'$. For each $1\leq j\leq 2\gamma$, set ${\nset}'_j$ of demand pairs contains, for each pair $(s,t)\in \nset_j$, one new demand pair $(s',t')$, whose destination vertex $t'=t$, and the source vertex appears on the top boundary $R^*$ of $G_{i+1}$ (we specify its exact location below).

%Similarly, set $\tilde{\nset}'_j$ of demand pairs contains, for each pair $(s,t)\in \nset'_j$, one new demand pair $(s',t')$, whose destination vertex $t'=t$, and the source vertex appears on $R^*$. 

Finally, we need to specify the locations of the $N_{i+1}=2\gamma N_i$ new source vertices on $R^*$. The sources are mapped to the $2\gamma N_i$ leftmost vertices of $R^*$. We first place the sources of the odd-indexed sets: $S(\nset_{2\gamma-1}'),S(\nset_{2\gamma-3}'),\ldots,S(\nset_3'),S(\nset_1')$ in this left-to-right order; within each set $S(\nset_{2j-1}')$, the sources are placed in the reversed order of their appearance on the bottom boundary of $A_{2j-1}$. 
Next, we place the sources of the even-indexed sets $S(\nset_2'),S(\nset_4'),\ldots,S(\nset_{2\gamma}')$ in this left-to-right order; within each set $\nset_{2j}'$, the sources are placed in exactly the same order as the order of their appearance on the top boundary of $A_{2j}$ (see Figure~\ref{fig: leveli}). 
This completes the description of the level-$(i+1)$ instance $(G_{i+1}, \mset_{i+1})$.
In the remainder of the proof, we show that it has the required properties.






%  Notice that $N_0=1$ and $\ell_0 = 9 = 9 \cdot N_0/g^0$ by our construction.
 % Now we complete the induction step by constructing level-$i+1$ instance $I_{i+1} = (G_{i+1}, \mset_{i+1})$.
 % We will use the \emph{perfect} level-$i$ instance $I_i = (G_i, \mset_i)$ with above mentioned properties guaranteed to exist by the induction hypothesis.

\begin{figure}[h]
\center
\scalebox{0.4}{\includegraphics{leveli}}
\caption{Level-$(i+1)$ instance $(G_{i+1},\mset_{i+1})$.
% TODO The sources of a constituent level-$i$ instance $I$ are denoted by $S(I)$.
\label{fig: leveli}}
\end{figure}


\iffalse
\paragraph{Level-$i+1$ Instance.}
Consider a $\ell_{i+1} \times \ell_{i+1}$ grid $G_{i+1}$.
Intuitively, we will consider $2\gamma_i$ copies of level-$i$ instance $I_i$, place their sources on the top row of $G_{i+1}$ and \textit{interlace} their destinations in $G_{i+1}$ (see: Figure \ref{fig: leveli}).
Let $(A^1, \cdots, A^{\gamma_i})$, $(B^1, \cdots, B^{\gamma_i})$ be fresh copies of level-$i$ instance $I_{i}$.
We call $A^1, \cdots, A^{\gamma_i}$ as \textit{blue} instances and $B^1, \cdots, B^{\gamma_i}$ as \textit{red} instances.
%Let $s(1), s(2), \cdots, s({N_i})$ be $N_i$ left-most vertices on the top row of $G_i$.
%For each $1 \leq j \leq \eta$ and $1 \leq k \leq N_{i-1}$, we map $k^{th}$ source node from left of the instance $I^j$ to the node $s(k + (j-1) \cdot N_{i-1})$.

Let $R$ be the top row of $G_{i+1}$ and $v(1), v(2). \ldots, v(\ell_{i+1})$ be the nodes of $R$ in the natural left-to-right order.
We map leftmost $\gamma_i N_i$ nodes on $R$ to the sources of \textit{blue} instances in \textbf{right-to-left} order (see: Figure \ref{fig: leveli}).
Formally, let $s_A(j,1), \ldots, s_A(j,N_i)$ be the sources $S(A^j)$ in left-to-right order.
For each $1 \leq k \leq N_i$, we map the source $s_A(j,k)$ to the node $v((j-1)N_i + k)$ on $R$ that we denote by $s'_A(j,k)$.
Similarly, we map next $\gamma_i N_i$ nodes of $R$ to the sources of \textit{red} instances in \textbf{left-to-right} order.
Formally, let $s_B(j,1), \ldots, s_B(j,N_i)$ be the sources $S(B^j)$ in left-to-right order.
For each $1 \leq k \leq N_i$, we map the source $s_B(j,k)$ to the node $v(\gamma_iN_i + (j-1)N_i + k)$ on $R$ that we denote by $s'_B(j,k)$.
Note that the placement of sources is well defined since $\ell_{i+1} \geq N_{i+1}$.
This completes the mapping of sources on the top row $R$ of $G_{i+1}$.


Our idea of placing the destination nodes motivates yet another definition: \textit{flipped} instances.
For a grid $G_i$, the flipped grid $G_{-i}$ is obtained by toggling the order of rows and columns in $G_i$ (see: Figure \ref{fig: flip}).
For an instance $A^j = (G_i, \mset_i)$, the corresponding flipped instance is given by $A^{-j} = (G_{-i}, \mset_i)$. 
Notice that each of the flipped instance $A^{-j}$ is also a perfect instance inheriting the same properties as $A^j$.


For $1 \leq j \leq \gamma_i$, we put the grids corresponding to \textit{blue} and \textit{red} instances $A^{-j}$ and $B^j$ side-by-side in alternating fashion, in their natural left-to-right order far away from top, left and bottom grid boundaries (see: Figure \ref{fig: leveli}).
We also ensure that all the destinations are mapped to the same row of $G_{i+1}$.
For each demand pair $(s_A(j,k), t_A(j,k))$ of $A^{-j}$, we add a unique demand pair $(s'_A(j,k), t_A(j,k))$ to $\mset_{i+1}$.
Similarly, for each demand pair $(s_B(j,k), t_B(j,k))$ of $B^{j}$, we also add a unique demand pair $(s'_B(j,k), t_B(j,k))$ to $\mset_{i+1}$.
%------------------------
%------------------------
%------------------------
%------------------------
\fi


It is immediate from our construction that $G_{i+1}$ is the $(\ell_{i+1}\times \ell_{i+1})$-grid, that $|\mset_{i+1}|=2\gamma_i N_i=N_{i+1}$, and that all source vertices of  $\mset_{i+1}$ lie on the top boundary of $G_{i+1}$. It now remains to show that instance $(G_{i+1},\mset_{i+1})$ is perfectly routable, and
that every subset $\hmset\subseteq \mset_{i+1}$ of demand pairs that has the distance property has cardinality at most $N_{i+1}/g^{i+1}$.
We prove this in the following two claims.

%Note that when we put these instances, we only map the destinations, as sources are already mapped on the first row of $G_{i+1}$.
%We note that the distance of $\gamma_i N_i$ from the left and bottom boundary; and $t_i$ from the top and right boundary is sufficient.
%Notice that the size of grid $\ell_{i+1} \times \ell_{i+1}$, where $\ell_{i+1} = 9 \cdot N_{i+1}/g_{i+1} \geq \gamma_i N_i + 2 \gamma_i \ell_i$ is sufficient to route every demand pair of $I_i$ by node-disjoint paths.

\begin{claim} \label{clm: routable}
 Instance $(G_{i+1},\mset_{i+1})$ is perfectly routable.
\end{claim}
\begin{proof}
  From the induction hypothesis, for each $1\leq j\leq 2\gamma$, there is a set $\pset_j$ of node-disjoint paths contained in $A_j$, that route all demand pairs in $\nset_j$. In order to complete the proof, it is enough to show that there is a set $\pset^*$ of node-disjoint paths, that are internally disjoint from $\bigcup_{j=1}^{2\gamma}A_j$, such that for each $1\leq j\leq 2\gamma$, for each pair $(s,t)\in \nset_j$, some path $P(s,t)\in\pset^*$ connects $s$ to its corresponding new source vertex $s'$.  
  %Notice that $\ell_{i+1} = 9 \cdot N_{i+1}/g^{i+1} \geq \gamma_i N_i + 2 \gamma_i \ell_i$.
 It is straightforward to construct the required set $\pset^*$ of paths, by utilizing the $\gamma N_i$ columns to the left of $A_1$ and the $\gamma N_i$ rows lying above and below the strip $S$ (see Figure \ref{fig: leveli}). 
\end{proof}

The next claim will finish the proof of Theorem~\ref{thm: iterations}.


\begin{claim} \label{clm: dist prop}
Let $\hmset\subseteq\mset_{i+1}$ be any subset of demand pairs that has the distance property. Then $|\hmset|\leq N_{i+1}/g^{i+1}$.
\end{claim}
\begin{proof}
Assume for contradiction that $|\hmset|> N_{i+1}/g^{i+1}$. For each $1\leq j\leq 2\gamma$, let $\hmset'_j=\nset'_j\cap \hmset$, and let $\hmset_j\subseteq \nset_j$ contain all demand pairs $(s,t)$ for which the corresponding new demand pair $(s',t')\in \hmset_j$. Notice that all demand pairs in $\hmset_j$ must also have the distance property inside the level-$i$ instance defined by $A_j$, and so, from the induction hypothesis, $|\hmset'_j|=|\hmset_j|\leq  N_i/g^i$. We say that index $1\leq j\leq 2\gamma$ is \emph{interesting} iff $\hmset'_j\neq \emptyset$. From the above discussion, the number of interesting indices is at least $\frac{N_{i+1}}{g^{i+1}}/\frac{N_i}{g^i} = \frac{N_{i+1}}{g\cdot N_i}=\frac{2\gamma}{g}>1.8\gamma$. 
We claim that there is an index $j> 0.8\gamma$, such that both $2j-1$ and $2j$ are interesting. Indeed, assume otherwise. Then the number of interesting indices is at most $1.6\gamma+0.2\gamma\leq 1.8\gamma$, a contradiction.
Let $j^*>0.8\gamma$ be an index, such that both $2j^*-1$ and $2j^*$ are interesting.
 Let $(s_1,t_1)\in \hmset'_{2j^*-1}$, and let $(s_2,t_2)\in \hmset'_{2j^*}$ be any demand pairs. From our construction, the two grids $A_{2j^*-1}$ and $A_{2j^*}$ are consecutive, and so $d(t_1,t_2) < 3 \ell_i = 27 N_i g^i$. We next show that $N_{\hmset}(s_1,s_2)>27N_ig^i$, contradicting the distance property of $\hmset$. The following claim will then finish the proof.
 
 
\begin{claim}
 $N_{\hmset}(s_1,s_2) > 27N_ig^i$
\end{claim}
\begin{proof}
Notice that if $(s,t)\in \hmset$ is a demand pair with $s$ lying to the left of $s_1$ on $R^*$, then $(s,t)\in \hmset'_{2j-1}$, where $j\geq j^*> 0.8\gamma$. Similarly, if   $(s,t)\in \hmset$ is a demand pair with $s$ lying to the right of $s_2$ on $R^*$, then $(s,t)\in \hmset'_{2j}$, where $j\geq j^*> 0.8\gamma$. Recall that for each $j$, 
  $|\hmset'_j|\leq  N_i/g^i$, and so overall the number of the demand pairs $(s,t)\in \hmset$ with $s$ lying to the left of $s_1$ or to the right of $s_2$ is bounded by $0.4\gamma\cdot N_i/g^i$ (this number includes the pairs $(s_1,t_1)$ and $(s_2,t_2)$). The remaining demand pairs must lie between $s_1$ and $s_2$ and therefore contribute to $N_{\hmset}(s_1,s_2)$. We then get that:
  
\[\begin{split}
N_{\hmset}(s_1,s_2)&\geq |\hmset|-\frac{0.4\gamma\cdot N_i}{g^i}\\
&\geq \frac{N_{i+1}}{g^{i+1}}-\frac{0.4\gamma\cdot N_i}{g^i}\\
&=\frac{2\gamma N_i}{1.1g^{i}}-\frac{0.4\gamma\cdot N_i}{g^i}\\
&\geq 1.4\frac{\gamma N_i}{g^i} \\
&=28 N_ig^i.\end{split}\]
  
    %Recall that $j \geq 0.8 \gamma_i$.
%    Let $\cset = \set{A^{-\gamma_i}, \ldots, A^{-j}, B^{j}, \ldots, B^{\gamma_i}}$ be a set of level-$i$ instances.
%    Notice that if a source $s \in S(\mset'_{i+1})$ appears either to the left of $s'$ or to the right of $s''$ on $R$, then $s$ belongs to some instance in $\cset$.
%    From level-$i$ analysis, at most $g^iN_i$ sources of $\mset'_{i+1}$ may belong to any such instance.
%    Thus, 
%    \[N_{\mset'_{i+1}}(s',s'') \geq |\mset'_{i+1}| -  |\cset| g^i N_i \]
%    Since $j \geq 0.8 \cdot \gamma_i$, $|\cset| \leq 2(\gamma_i - j)+2 \leq 0.5 \cdot \gamma_i$.
%    Recall that $|\mset'_{i+1}| > g^{i+1}N_{i+1}$, $\gamma_i = 20/g^{2i}$ and $N_{i+1} = 2 \gamma_i N_i$.
%    Substituting these values, we obtain the claimed bound.
  \end{proof}
\end{proof}
%
%From Claim \ref{clm: routable} and Claim \ref{clm: dist prop}, we conclude that $I_{i+1}$ is a \emph{perfect} instance, completing the induction step.
%
%
\endproofof



